Efficient Real Time Recurrent Learning through combined activity and parameter sparsity

Backpropagation through time (BPTT) is the standard algorithm for training recurrent neural networks (RNNs), which requires separate simulation phases for the forward and backward passes for inference and learning, respectively. Moreover, BPTT requires storing the complete history of network states between phases, with memory consumption growing proportional to the input sequence length. This makes BPTT unsuited for online learning and presents a challenge for implementation on low-resource real-time systems. Real-Time Recurrent Learning (RTRL) allows online learning, and the growth of required memory is independent of sequence length. However, RTRL suffers from exceptionally high computational costs that grow proportional to the fourth power of the state size, making RTRL computationally intractable for all but the smallest of networks. In this work, we show that recurrent networks exhibiting high activity sparsity can reduce the computational cost of RTRL. Moreover, combining activity and parameter sparsity can lead to significant enough savings in computational and memory costs to make RTRL practical. Unlike previous work, this improvement in the efficiency of RTRL can be achieved without using any approximations for the learning process.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}


==> tags <==
!_TAG_EXTRA_DESCRIPTION	anonymous	/Include tags for non-named objects like lambda/
!_TAG_EXTRA_DESCRIPTION	fileScope	/Include tags of file scope/
!_TAG_EXTRA_DESCRIPTION	pseudo	/Include pseudo tags/
!_TAG_EXTRA_DESCRIPTION	subparser	/Include tags generated by subparsers/
!_TAG_FIELD_DESCRIPTION	epoch	/the last modified time of the input file (only for F\/file kind tag)/
!_TAG_FIELD_DESCRIPTION	file	/File-restricted scoping/
!_TAG_FIELD_DESCRIPTION	input	/input file/
!_TAG_FIELD_DESCRIPTION	name	/tag name/
!_TAG_FIELD_DESCRIPTION	pattern	/pattern/
!_TAG_FIELD_DESCRIPTION	typeref	/Type and name of a variable or typedef/
!_TAG_FIELD_DESCRIPTION!XML	uri	/uri associated with name prefix/
!_TAG_FILE_FORMAT	2	/extended format; --format=1 will not append ;" to lines/
!_TAG_FILE_SORTED	1	/0=unsorted, 1=sorted, 2=foldcase/
!_TAG_KIND_DESCRIPTION!BibTeX	B,booklet	/booklet/
!_TAG_KIND_DESCRIPTION!BibTeX	I,incollection	/incollection/
!_TAG_KIND_DESCRIPTION!BibTeX	M,mastersthesis	/mastersthesis/
!_TAG_KIND_DESCRIPTION!BibTeX	P,proceedings	/proceedings/
!_TAG_KIND_DESCRIPTION!BibTeX	a,article	/article/
!_TAG_KIND_DESCRIPTION!BibTeX	b,book	/book/
!_TAG_KIND_DESCRIPTION!BibTeX	c,conference	/conference/
!_TAG_KIND_DESCRIPTION!BibTeX	i,inbook	/inbook/
!_TAG_KIND_DESCRIPTION!BibTeX	j,inproceedings	/inproceedings/
!_TAG_KIND_DESCRIPTION!BibTeX	m,manual	/manual/
!_TAG_KIND_DESCRIPTION!BibTeX	n,misc	/misc/
!_TAG_KIND_DESCRIPTION!BibTeX	p,phdthesis	/phdthesis/
!_TAG_KIND_DESCRIPTION!BibTeX	s,string	/string/
!_TAG_KIND_DESCRIPTION!BibTeX	t,techreport	/techreport/
!_TAG_KIND_DESCRIPTION!BibTeX	u,unpublished	/unpublished/
!_TAG_KIND_DESCRIPTION!SVG	d,def	/ids in defs tags/
!_TAG_KIND_DESCRIPTION!Tex	B,bibitem	/bibliography items/
!_TAG_KIND_DESCRIPTION!Tex	C,command	/command created with \\newcommand/
!_TAG_KIND_DESCRIPTION!Tex	G,subparagraph	/subparagraphs/
!_TAG_KIND_DESCRIPTION!Tex	N,counter	/counter created with \\newcounter/
!_TAG_KIND_DESCRIPTION!Tex	P,paragraph	/paragraphs/
!_TAG_KIND_DESCRIPTION!Tex	b,subsubsection	/subsubsections/
!_TAG_KIND_DESCRIPTION!Tex	c,chapter	/chapters/
!_TAG_KIND_DESCRIPTION!Tex	e,environment	/environment created with \\newenvironment/
!_TAG_KIND_DESCRIPTION!Tex	i,xinput	/external input files/
!_TAG_KIND_DESCRIPTION!Tex	l,label	/labels/
!_TAG_KIND_DESCRIPTION!Tex	o,operator	/math operator created with \\DeclareMathOperator/
!_TAG_KIND_DESCRIPTION!Tex	p,part	/parts/
!_TAG_KIND_DESCRIPTION!Tex	s,section	/sections/
!_TAG_KIND_DESCRIPTION!Tex	t,theorem	/theorem created with \\newtheorem/
!_TAG_KIND_DESCRIPTION!Tex	u,subsection	/subsections/
!_TAG_KIND_DESCRIPTION!XML	i,id	/id attributes/
!_TAG_KIND_DESCRIPTION!XML	n,nsprefix	/namespace prefixes/
!_TAG_KIND_DESCRIPTION!XML	r,root	/root elements/
!_TAG_OUTPUT_EXCMD	mixed	/number, pattern, mixed, or combineV2/
!_TAG_OUTPUT_FILESEP	slash	/slash or backslash/
!_TAG_OUTPUT_MODE	u-ctags	/u-ctags or e-ctags/
!_TAG_PATTERN_LENGTH_LIMIT	96	/0 for no limit/
!_TAG_PROC_CWD	/Users/anand/source/abs/A13-Sparse-RTRL/	//
!_TAG_PROGRAM_AUTHOR	Universal Ctags Team	//
!_TAG_PROGRAM_NAME	Universal Ctags	/Derived from Exuberant Ctags/
!_TAG_PROGRAM_URL	https://ctags.io/	/official site/
!_TAG_PROGRAM_VERSION	5.9.0	//
!_TAG_ROLE_DESCRIPTION!Tex!xinput	bibliography	/bibliography (.bib) file/
!_TAG_ROLE_DESCRIPTION!Tex!xinput	included	/external input file specified with \\include/
!_TAG_ROLE_DESCRIPTION!Tex!xinput	input	/external input file specified with \\input/
ASGD	references.bib	/^@article{ASGD,$/;"	a
Adam2015	references.bib	/^@inproceedings{Adam2015,$/;"	j
Arrow2Mend	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-2	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-2	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-2-0	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-2-0	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-2-3	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-2-3	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-2-3-0	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-2-3-0	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-2-3-0-0	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-2-3-0-0	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-2-3-0-6	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-2-3-0-6	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-2-3-0-8	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-2-3-0-8	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-2-3-00	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-2-3-00	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-2-3-05	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-2-3-05	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-2-3-3	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-2-3-3	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-2-5	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-2-5	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-2-7	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-2-7	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-4	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-4	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-4-5	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-4-5	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-4-5-9	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-4-5-9	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-7	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-7	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-2	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-2	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-2-1	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-2-1	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-2-1-5	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-2-1-5	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-0	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-0	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-0-0	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-0-0	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-0-0-4	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-0-0-4	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-0-0-5	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-0-0-5	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-0-0-6	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-0-0-6	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-0-0-7	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-0-0-7	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-0-0-75	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-0-0-75	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-0-0-75-7	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-0-0-75-7	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-0-0-75-8	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-0-0-75-8	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-0-0-75-8-9	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-0-0-75-8-9	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-0-03	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-0-03	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-0-03-0	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-0-03-0	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-0-03-1	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-0-03-1	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-0-03-4	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-0-03-4	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-0-03-4-1	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-0-03-4-1	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-0-03-6	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-0-03-6	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-0-03-65	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-0-03-65	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-0-6	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-0-6	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-0-8	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-0-8	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-0-9	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-0-9	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-04	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-04	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-4	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-4	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-4-1	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-4-1	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-4-12	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-4-12	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-4-12-3	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-4-12-3	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-4-12-3-7	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-4-12-3-7	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-4-12-8	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-4-12-8	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-4-3	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-4-3	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-4-5	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-4-5	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-4-7	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-4-7	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-6	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-6	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-6-5	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-6-5	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-6-52	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-6-52	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-6-52-8	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-6-52-8	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-6-8	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-6-8	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-60	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-60	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-67	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-67	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-67-3	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-67-3	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-67-31	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-67-31	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-67-5	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-67-5	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-67-6	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-67-6	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-67-9	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-67-9	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-67-9-8	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-67-9-8	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-67-9-8-5	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-67-9-8-5	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-67-9-8-5-6	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-67-9-8-5-6	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-67-9-8-7	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-67-9-8-7	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-67-9-8-7-0	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-67-9-8-7-0	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-67-9-8-7-0-3	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-67-9-8-7-0-3	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-67-9-8-7-0-3-4	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-67-9-8-7-0-3-4	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-67-9-8-7-6	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-67-9-8-7-6	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-67-9-8-7-6-5	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-67-9-8-7-6-5	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-67-9-8-7-6-5-9	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-67-9-8-7-6-5-9	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-67-9-8-7-9	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-67-9-8-7-9	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-3-67-9-8-7-9-6	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-3-67-9-8-7-9-6	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-30	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-30	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-30-9	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-30-9	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-30-9-3	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-30-9-3	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-30-9-3-2	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-30-9-3-2	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-30-9-3-2-2	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-30-9-3-2-2	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-30-9-3-2-3	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-30-9-3-2-3	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-30-9-3-2-3-1	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-30-9-3-2-3-1	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-30-9-3-2-3-2	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-30-9-3-2-3-2	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-30-9-3-2-3-4	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-30-9-3-2-3-4	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-30-9-3-2-3-44	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-30-9-3-2-3-44	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-30-9-3-2-3-44-2	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-30-9-3-2-3-44-2	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-30-9-3-2-3-44-2-5	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-30-9-3-2-3-44-2-5	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-30-9-3-2-3-44-2-5-0	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-30-9-3-2-3-44-2-5-0	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-30-9-3-2-3-44-2-8	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-30-9-3-2-3-44-2-8	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-30-9-3-2-3-44-2-9	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-30-9-3-2-3-44-2-9	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-30-9-3-2-3-44-7	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-30-9-3-2-3-44-7	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-30-9-3-2-3-44-9	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-30-9-3-2-3-44-9	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-30-9-3-2-3-7	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-30-9-3-2-3-7	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-30-9-3-2-31	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-30-9-3-2-31	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-30-9-3-2-4	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-30-9-3-2-4	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-30-9-3-2-47	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-30-9-3-2-47	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-30-9-3-2-47-3	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-30-9-3-2-47-3	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-30-9-3-2-47-3-1	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-30-9-3-2-47-3-1	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-30-9-3-2-47-3-8	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-30-9-3-2-47-3-8	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-30-9-3-2-47-6	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-30-9-3-2-47-6	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-30-9-3-2-47-6-0	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-30-9-3-2-47-6-0	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-30-9-3-2-47-6-0-3	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-30-9-3-2-47-6-0-3	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-30-9-3-2-47-6-0-4	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-30-9-3-2-47-6-0-4	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-30-9-3-2-47-6-0-4-6	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-30-9-3-2-47-6-0-4-6	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-30-9-3-2-47-6-0-4-8	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-30-9-3-2-47-6-0-4-8	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-30-9-3-2-47-6-0-4-9	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-30-9-3-2-47-6-0-4-9	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-30-9-3-2-47-6-0-4-9-0	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-30-9-3-2-47-6-0-4-9-0	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-30-9-3-2-47-6-0-7	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-30-9-3-2-47-6-0-7	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-30-9-3-2-47-6-2	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-30-9-3-2-47-6-2	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-30-9-3-2-47-6-4	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-30-9-3-2-47-6-4	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-30-9-3-2-47-6-7	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-30-9-3-2-47-6-7	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-30-9-3-2-47-6-8	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-30-9-3-2-47-6-8	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-30-9-3-2-47-69	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-30-9-3-2-47-69	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-30-9-3-2-47-7	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-30-9-3-2-47-7	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-30-9-3-2-47-77	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-30-9-3-2-47-77	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-30-9-3-2-6	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-30-9-3-2-6	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-30-9-3-2-6-0	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-30-9-3-2-6-0	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-30-9-3-2-6-4	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-30-9-3-2-6-4	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-30-9-3-2-6-6	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-30-9-3-2-6-6	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-30-9-3-2-63	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-30-9-3-2-63	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-30-9-3-2-64	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-30-9-3-2-64	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-30-9-3-2-64-1	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-30-9-3-2-64-1	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-30-9-3-2-64-3	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-30-9-3-2-64-3	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-30-9-3-2-8	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-30-9-3-2-8	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-30-9-3-2-8-2	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-30-9-3-2-8-2	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-30-9-3-2-8-7	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-30-9-3-2-8-7	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-30-9-3-2-8-9	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-30-9-3-2-8-9	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-30-9-3-5	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-30-9-3-5	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-1	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-1	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-4	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-4	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-4-0	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-4-0	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-4-6	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-4-6	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-6	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-6	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-7	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-7	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-7-2	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-7-2	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-7-2-4	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-7-2-4	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-7-3	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-7-3	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-7-3-0	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-7-3-0	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-7-3-4	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-7-3-4	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-7-3-5	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-7-3-5	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-7-3-52	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-7-3-52	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-7-3-52-1	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-7-3-52-1	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-7-3-52-6	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-7-3-52-6	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-7-3-52-6-3	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-7-3-52-6-3	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-7-3-52-6-6	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-7-3-52-6-6	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-7-3-52-6-6-6	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-7-3-52-6-6-6	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-7-3-59	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-7-3-59	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-7-3-59-6	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-7-3-59-6	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-7-3-59-6-4	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-7-3-59-6-4	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-7-3-59-8	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-7-3-59-8	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-7-3-8	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-7-3-8	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-7-3-8-0	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-7-3-8-0	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-7-3-8-7	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-7-3-8-7	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-7-3-8-8	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-7-3-8-8	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-7-3-82	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-7-3-82	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-7-3-9	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-7-3-9	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-7-32	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-7-32	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-7-4	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-7-4	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-7-4-0	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-7-4-0	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-7-4-1	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-7-4-1	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-7-4-1-1	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-7-4-1-1	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-7-4-1-1-1	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-7-4-1-1-1	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-7-4-1-1-2	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-7-4-1-1-2	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-7-4-1-1-2-4	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-7-4-1-1-2-4	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-7-4-1-4	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-7-4-1-4	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-7-4-8	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-7-4-8	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-7-8	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-7-8	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-9	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-9	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-9-2	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-9-2	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-9-2-0	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-9-2-0	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-9-2-0-5	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-9-2-0-5	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-9-2-0-7	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-9-2-0-7	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-9-2-03	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-9-2-03	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-9-2-2	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-9-2-2	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-9-2-3	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-9-2-3	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-9-2-4	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-9-2-4	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-9-3	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-9-3	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-9-3-0	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-9-3-0	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-9-3-0-6	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-9-3-0-6	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-9-6	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-9-6	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-9-8	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-9-8	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-8-5-1-7-9-9-9	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-8-5-1-7-9-9-9	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
Arrow2Mend-88	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	d
Arrow2Mend-88	figures/pseudo-derivative.svg	/^       inkscape:isstock="true">$/;"	i
DejaVuSans-20	figures/combined-sparsity-plots.svg	/^					<path id="DejaVuSans-20" d="M-292.7-4498.2"\/>$/;"	i
DejaVuSans-20_00000000933122482684904760000013828614274790569884_	figures/combined-sparsity-plots.svg	/^					<path id="DejaVuSans-20_00000000933122482684904760000013828614274790569884_" d="M1066.8,726/;"	i
DejaVuSans-20_00000003796856781613302640000010362891249348088988_	figures/combined-sparsity-plots.svg	/^					<path id="DejaVuSans-20_00000003796856781613302640000010362891249348088988_" d="M-114.7,316/;"	i
DejaVuSans-20_00000026869032335421174310000000325053025422993798_	figures/combined-sparsity-plots.svg	/^					<path id="DejaVuSans-20_00000026869032335421174310000000325053025422993798_" d="M-471,316.2/;"	i
DejaVuSans-20_00000035518405579965693020000017031614133456917949_	figures/combined-sparsity-plots.svg	/^					<path id="DejaVuSans-20_00000035518405579965693020000017031614133456917949_" d="M-114.7,316/;"	i
DejaVuSans-20_00000040563361992285678520000002497562525848362937_	figures/combined-sparsity-plots.svg	/^					<path id="DejaVuSans-20_00000040563361992285678520000002497562525848362937_" d="M709.1,726./;"	i
DejaVuSans-20_00000044868963830428098560000012115509787269955733_	figures/combined-sparsity-plots.svg	/^					<path id="DejaVuSans-20_00000044868963830428098560000012115509787269955733_" d="M1949.8,726/;"	i
DejaVuSans-20_00000047030800753492638960000010260349855201616793_	figures/combined-sparsity-plots.svg	/^					<path id="DejaVuSans-20_00000047030800753492638960000010260349855201616793_" d="M-285.2,340/;"	i
DejaVuSans-20_00000047046513215130848150000000176326957908490394_	figures/combined-sparsity-plots.svg	/^					<path id="DejaVuSans-20_00000047046513215130848150000000176326957908490394_" d="M171.3-4498/;"	i
DejaVuSans-20_00000049931395413548677450000017477878126748854457_	figures/combined-sparsity-plots.svg	/^					<path id="DejaVuSans-20_00000049931395413548677450000017477878126748854457_" d="M-114.7,316/;"	i
DejaVuSans-20_00000053521068199056466570000002379060559751162297_	figures/combined-sparsity-plots.svg	/^					<path id="DejaVuSans-20_00000053521068199056466570000002379060559751162297_" d="M-114.7,316/;"	i
DejaVuSans-20_00000060711316759976672910000018080627987372793521_	figures/combined-sparsity-plots.svg	/^					<path id="DejaVuSans-20_00000060711316759976672910000018080627987372793521_" d="M1494.9,726/;"	i
DejaVuSans-20_00000063603659267038216190000004543297147019609277_	figures/combined-sparsity-plots.svg	/^					<path id="DejaVuSans-20_00000063603659267038216190000004543297147019609277_" d="M-471,316.2/;"	i
DejaVuSans-20_00000067200150965252031850000005593972709329515909_	figures/combined-sparsity-plots.svg	/^					<path id="DejaVuSans-20_00000067200150965252031850000005593972709329515909_" d="M-471,316.2/;"	i
DejaVuSans-20_00000072972201683617523530000003148106503635058105_	figures/combined-sparsity-plots.svg	/^					<path id="DejaVuSans-20_00000072972201683617523530000003148106503635058105_" d="M-471,316.2/;"	i
DejaVuSans-20_00000075862840085705395880000013042648043673935783_	figures/combined-sparsity-plots.svg	/^					<path id="DejaVuSans-20_00000075862840085705395880000013042648043673935783_" d="M-114.7,316/;"	i
DejaVuSans-20_00000084519305779982174710000003291228013811479481_	figures/combined-sparsity-plots.svg	/^					<path id="DejaVuSans-20_00000084519305779982174710000003291228013811479481_" d="M-178.3,316/;"	i
DejaVuSans-20_00000087385210601679732710000012708667263313734548_	figures/combined-sparsity-plots.svg	/^					<path id="DejaVuSans-20_00000087385210601679732710000012708667263313734548_" d="M-471,316.2/;"	i
DejaVuSans-20_00000096766201910672934810000013788179203198611877_	figures/combined-sparsity-plots.svg	/^					<path id="DejaVuSans-20_00000096766201910672934810000013788179203198611877_" d="M-471,316.2/;"	i
DejaVuSans-20_00000105389556466709053190000005179215705326844573_	figures/combined-sparsity-plots.svg	/^					<path id="DejaVuSans-20_00000105389556466709053190000005179215705326844573_" d="M-114.7,316/;"	i
DejaVuSans-20_00000110469299586373801690000003006642779072324753_	figures/combined-sparsity-plots.svg	/^					<path id="DejaVuSans-20_00000110469299586373801690000003006642779072324753_" d="M-471,316.2/;"	i
DejaVuSans-20_00000136373666080323960300000008849441996888113588_	figures/combined-sparsity-plots.svg	/^					<path id="DejaVuSans-20_00000136373666080323960300000008849441996888113588_" d="M-114.7,316/;"	i
DejaVuSans-20_00000146458596222550498210000001623747656782912676_	figures/combined-sparsity-plots.svg	/^					<path id="DejaVuSans-20_00000146458596222550498210000001623747656782912676_" d="M618.7,726./;"	i
DejaVuSans-20_00000151508181175725285020000013384640725564432014_	figures/combined-sparsity-plots.svg	/^					<path id="DejaVuSans-20_00000151508181175725285020000013384640725564432014_" d="M-534.7,316/;"	i
DejaVuSans-20_00000158727506074135514030000000851943848061047936_	figures/combined-sparsity-plots.svg	/^					<path id="DejaVuSans-20_00000158727506074135514030000000851943848061047936_" d="M1046.8,726/;"	i
DejaVuSans-20_00000163791349380397269610000012777860209505395380_	figures/combined-sparsity-plots.svg	/^					<path id="DejaVuSans-20_00000163791349380397269610000012777860209505395380_" d="M-471,316.2/;"	i
DejaVuSans-20_00000166654823392998456270000014493217893761206204_	figures/combined-sparsity-plots.svg	/^					<path id="DejaVuSans-20_00000166654823392998456270000014493217893761206204_" d="M-471,316.2/;"	i
DejaVuSans-20_00000167386854502508597900000000986039233613834150_	figures/combined-sparsity-plots.svg	/^					<path id="DejaVuSans-20_00000167386854502508597900000000986039233613834150_" d="M-114.7,316/;"	i
DejaVuSans-20_00000171684539710491218540000016455549699183742848_	figures/combined-sparsity-plots.svg	/^					<path id="DejaVuSans-20_00000171684539710491218540000016455549699183742848_" d="M178.8,340./;"	i
DejaVuSans-20_00000171707509780121841060000008441670706628952492_	figures/combined-sparsity-plots.svg	/^					<path id="DejaVuSans-20_00000171707509780121841060000008441670706628952492_" d="M-114.7,316/;"	i
DejaVuSans-20_00000176011407766807618400000012566301898726702013_	figures/combined-sparsity-plots.svg	/^					<path id="DejaVuSans-20_00000176011407766807618400000012566301898726702013_" d="M1501.7,726/;"	i
DejaVuSans-25	figures/combined-sparsity-plots.svg	/^						C-553,388.6-548.9,390.4-543.8,390.4z"\/>$/;"	i
DejaVuSans-25_00000011746982749686438720000016788902290563881367_	figures/combined-sparsity-plots.svg	/^						s-9.3,1.8-12.3,5.3c-3,3.6-4.5,8.4-4.5,14.5s1.5,10.9,4.5,14.5C-553,388.6-548.9,390.4-543.8,/;"	i
DejaVuSans-25_00000039109616884296073630000001125534794453467280_	figures/combined-sparsity-plots.svg	/^						"\/>$/;"	i
DejaVuSans-25_00000046326327300520746410000006233352779577165235_	figures/combined-sparsity-plots.svg	/^						s-9.3,1.8-12.3,5.3c-3,3.6-4.5,8.4-4.5,14.5s1.5,10.9,4.5,14.5C-553,388.6-548.9,390.4-543.8,/;"	i
DejaVuSans-25_00000060004923906444056390000013392017819144808842_	figures/combined-sparsity-plots.svg	/^						s-9.3,1.8-12.3,5.3c-3,3.6-4.5,8.4-4.5,14.5s1.5,10.9,4.5,14.5C-553,388.6-548.9,390.4-543.8,/;"	i
DejaVuSans-25_00000062906290926742504260000006450637483668136835_	figures/combined-sparsity-plots.svg	/^						s-9.3,1.8-12.3,5.3c-3,3.6-4.5,8.4-4.5,14.5s1.5,10.9,4.5,14.5C-553,388.6-548.9,390.4-543.8,/;"	i
DejaVuSans-25_00000072251611031702321960000018136233830108679070_	figures/combined-sparsity-plots.svg	/^						s-9.3,1.8-12.3,5.3c-3,3.6-4.5,8.4-4.5,14.5s1.5,10.9,4.5,14.5C-553,388.6-548.9,390.4-543.8,/;"	i
DejaVuSans-25_00000105412716874704699750000017307487032142071947_	figures/combined-sparsity-plots.svg	/^						s-9.3,1.8-12.3,5.3c-3,3.6-4.5,8.4-4.5,14.5s1.5,10.9,4.5,14.5C-553,388.6-548.9,390.4-543.8,/;"	i
DejaVuSans-25_00000141452487440466379710000014665599244653760677_	figures/combined-sparsity-plots.svg	/^						s-9.3,1.8-12.3,5.3c-3,3.6-4.5,8.4-4.5,14.5s1.5,10.9,4.5,14.5C-553,388.6-548.9,390.4-543.8,/;"	i
DejaVuSans-25_00000162349241254369505800000002652144640784665762_	figures/combined-sparsity-plots.svg	/^						s-9.3,1.8-12.3,5.3c-3,3.6-4.5,8.4-4.5,14.5s1.5,10.9,4.5,14.5C-553,388.6-548.9,390.4-543.8,/;"	i
DejaVuSans-28_00000005967975450675089700000007456515771768727716_	figures/combined-sparsity-plots.svg	/^						c-2.4,7.4-3.6,14.7-3.6,22s1.2,14.6,3.6,21.9c2.4,7.4,6.1,14.9,11,22.6L1109.6,802.2L1109.6,8/;"	i
DejaVuSans-28_00000152242452745567282500000003267269704338175667_	figures/combined-sparsity-plots.svg	/^						c-2.4,7.4-3.6,14.7-3.6,22s1.2,14.6,3.6,21.9c2.4,7.4,6.1,14.9,11,22.6L1557.7,802.2L1557.7,8/;"	i
DejaVuSans-29_00000153703406245816011120000007570367017318592951_	figures/combined-sparsity-plots.svg	/^						s-1.1,14.9-3.2,22.3C1664.8,787.4,1661.6,794.8,1657.2,802.2z"\/>$/;"	i
DejaVuSans-29_00000174577534312697788690000005966734626504842904_	figures/combined-sparsity-plots.svg	/^						s-1.1,14.9-3.2,22.3C2112.9,787.4,2109.6,794.8,2105.3,802.2z"\/>$/;"	i
DejaVuSans-2e_00000005248122890058027840000006740331159876860298_	figures/combined-sparsity-plots.svg	/^						<path id="DejaVuSans-2e_00000005248122890058027840000006740331159876860298_" d="M-652.1,36/;"	i
DejaVuSans-2e_00000011012501868090512190000004571999484880874399_	figures/combined-sparsity-plots.svg	/^						<path id="DejaVuSans-2e_00000011012501868090512190000004571999484880874399_" d="M-652.1,26/;"	i
DejaVuSans-2e_00000018215440193500462220000006522326438756401333_	figures/combined-sparsity-plots.svg	/^							\/>$/;"	i
DejaVuSans-2e_00000024717162136650628310000005120562387585398179_	figures/combined-sparsity-plots.svg	/^						<path id="DejaVuSans-2e_00000024717162136650628310000005120562387585398179_" d="M-652.1,26/;"	i
DejaVuSans-2e_00000029731481506297607420000000900790921774186423_	figures/combined-sparsity-plots.svg	/^							\/>$/;"	i
DejaVuSans-2e_00000042007522202839979850000002562488174219114925_	figures/combined-sparsity-plots.svg	/^							\/>$/;"	i
DejaVuSans-2e_00000046315318523671917880000013246145933027070337_	figures/combined-sparsity-plots.svg	/^							\/>$/;"	i
DejaVuSans-2e_00000050626129518775418580000002151766316090692234_	figures/combined-sparsity-plots.svg	/^						<path id="DejaVuSans-2e_00000050626129518775418580000002151766316090692234_" d="M-652.1,35/;"	i
DejaVuSans-2e_00000051344384614713725600000014066533418081663648_	figures/combined-sparsity-plots.svg	/^						<path id="DejaVuSans-2e_00000051344384614713725600000014066533418081663648_" d="M-652.1,36/;"	i
DejaVuSans-2e_00000054253949413983587030000001464972681892323480_	figures/combined-sparsity-plots.svg	/^							\/>$/;"	i
DejaVuSans-2e_00000067235200565485227040000011138053698865846663_	figures/combined-sparsity-plots.svg	/^						<path id="DejaVuSans-2e_00000067235200565485227040000011138053698865846663_" d="M-652.1,26/;"	i
DejaVuSans-2e_00000070830675555413806050000013640327629327518112_	figures/combined-sparsity-plots.svg	/^						<path id="DejaVuSans-2e_00000070830675555413806050000013640327629327518112_" d="M-652.1,26/;"	i
DejaVuSans-2e_00000075163027847059296810000007825732182267906464_	figures/combined-sparsity-plots.svg	/^							\/>$/;"	i
DejaVuSans-2e_00000093139737727747568540000006617376359757509769_	figures/combined-sparsity-plots.svg	/^						<path id="DejaVuSans-2e_00000093139737727747568540000006617376359757509769_" d="M-652.1,26/;"	i
DejaVuSans-2e_00000102532238522905335020000018313647037996122046_	figures/combined-sparsity-plots.svg	/^						<path id="DejaVuSans-2e_00000102532238522905335020000018313647037996122046_" d="M-652.1,26/;"	i
DejaVuSans-2e_00000111158155730428788880000014135356375583205249_	figures/combined-sparsity-plots.svg	/^						<path id="DejaVuSans-2e_00000111158155730428788880000014135356375583205249_" d="M-652.1,35/;"	i
DejaVuSans-2e_00000124126431696580612610000001361361031353365899_	figures/combined-sparsity-plots.svg	/^							\/>$/;"	i
DejaVuSans-2e_00000124858160598920511490000008950297130052454786_	figures/combined-sparsity-plots.svg	/^						<path id="DejaVuSans-2e_00000124858160598920511490000008950297130052454786_" d="M-652.1,35/;"	i
DejaVuSans-2e_00000129204539062144876540000000358622699789344643_	figures/combined-sparsity-plots.svg	/^						<path id="DejaVuSans-2e_00000129204539062144876540000000358622699789344643_" d="M-652.1,26/;"	i
DejaVuSans-2e_00000129915099267347312140000014508330793443911855_	figures/combined-sparsity-plots.svg	/^							\/>$/;"	i
DejaVuSans-2e_00000135664922500776088550000009602418613022075533_	figures/combined-sparsity-plots.svg	/^						<path id="DejaVuSans-2e_00000135664922500776088550000009602418613022075533_" d="M-652.1,26/;"	i
DejaVuSans-2e_00000138531978512497701630000018190460986444747912_	figures/combined-sparsity-plots.svg	/^						<path id="DejaVuSans-2e_00000138531978512497701630000018190460986444747912_" d="M-652.1,35/;"	i
DejaVuSans-2e_00000145021926615557705480000014811254296533993639_	figures/combined-sparsity-plots.svg	/^						<path id="DejaVuSans-2e_00000145021926615557705480000014811254296533993639_" d="M-652.1,36/;"	i
DejaVuSans-2e_00000149348665938933622420000008479291369355915677_	figures/combined-sparsity-plots.svg	/^						<path id="DejaVuSans-2e_00000149348665938933622420000008479291369355915677_" d="M-652.1,36/;"	i
DejaVuSans-2e_00000150066109426128174680000002131574691739141035_	figures/combined-sparsity-plots.svg	/^						<path id="DejaVuSans-2e_00000150066109426128174680000002131574691739141035_" d="M-652.1,26/;"	i
DejaVuSans-2e_00000154423043244526075900000012737097209132460176_	figures/combined-sparsity-plots.svg	/^						<path id="DejaVuSans-2e_00000154423043244526075900000012737097209132460176_" d="M-652.1,26/;"	i
DejaVuSans-2e_00000177455188434414377940000014981514475613259186_	figures/combined-sparsity-plots.svg	/^						<path id="DejaVuSans-2e_00000177455188434414377940000014981514475613259186_" d="M-652.1,26/;"	i
DejaVuSans-2e_00000180338932761597252230000017558556999117734330_	figures/combined-sparsity-plots.svg	/^						<path id="DejaVuSans-2e_00000180338932761597252230000017558556999117734330_" d="M-652.1,26/;"	i
DejaVuSans-30_00000002376248948796544300000009235469614677921968_	figures/combined-sparsity-plots.svg	/^							C-613.6,421.1-607.3,424.4-599.2,424.4z"\/>$/;"	i
DejaVuSans-30_00000003785447762031392150000000727379008272454311_	figures/combined-sparsity-plots.svg	/^							C-652.8-4427.2-646.6-4423.9-638.4-4423.9z"\/>$/;"	i
DejaVuSans-30_00000004515253617481624350000001378090742797676205_	figures/combined-sparsity-plots.svg	/^							C-581.7,411.1-575.5,414.4-567.3,414.4z"\/>$/;"	i
DejaVuSans-30_00000004524317319369171930000007207129462578071224_	figures/combined-sparsity-plots.svg	/^							C-616.1-4430.6-609.9-4427.3-601.7-4427.3z"\/>$/;"	i
DejaVuSans-30_00000004525712345360512040000006522770785054164102_	figures/combined-sparsity-plots.svg	/^						C-612.3,387.2-606.1,390.4-597.9,390.4z"\/>$/;"	i
DejaVuSans-30_00000005964405957135689610000005691512925626168973_	figures/combined-sparsity-plots.svg	/^							C-584.3-4430.6-578.1-4427.3-569.9-4427.3z"\/>$/;"	i
DejaVuSans-30_00000005975700635128368810000012668534937044094598_	figures/combined-sparsity-plots.svg	/^							S-583-4423.9-574.8-4423.9z"\/>$/;"	i
DejaVuSans-30_00000012444685763251590530000006141356828913695660_	figures/combined-sparsity-plots.svg	/^							s-10.6-9.7-18.7-9.7c-8.2,0-14.4,3.2-18.7,9.7s-6.5,15.8-6.5,28.1c0,12.3,2.2,21.7,6.5,28.1S/;"	i
DejaVuSans-30_00000016046758952901358320000004532948365418984360_	figures/combined-sparsity-plots.svg	/^							C-709,321.1-702.8,324.4-694.6,324.4z"\/>$/;"	i
DejaVuSans-30_00000018228595375457357810000018402983690780835204_	figures/combined-sparsity-plots.svg	/^							C-645.4,411.1-639.1,414.4-631,414.4z"\/>$/;"	i
DejaVuSans-30_00000019655472945591878180000005996945962772876184_	figures/combined-sparsity-plots.svg	/^							C-709,411.1-702.8,414.4-694.6,414.4z"\/>$/;"	i
DejaVuSans-30_00000021083477605737115860000016261571068301194429_	figures/combined-sparsity-plots.svg	/^							C-581.7,321.1-575.5,324.4-567.3,324.4z"\/>$/;"	i
DejaVuSans-30_00000022559632636071645940000012901055904583281032_	figures/combined-sparsity-plots.svg	/^							C-645.4,321.1-639.1,324.4-631,324.4z"\/>$/;"	i
DejaVuSans-30_00000023277236429799593440000010102166379690220952_	figures/combined-sparsity-plots.svg	/^							S-583-4423.9-574.8-4423.9z"\/>$/;"	i
DejaVuSans-30_00000028282665526829575130000017022182031985866888_	figures/combined-sparsity-plots.svg	/^							C-584.3-4430.6-578.1-4427.3-569.9-4427.3z"\/>$/;"	i
DejaVuSans-30_00000029025553431134186230000014496020482037455232_	figures/combined-sparsity-plots.svg	/^							s-10.6-9.7-18.7-9.7c-8.2,0-14.4,3.2-18.7,9.7s-6.5,15.8-6.5,28.1c0,12.3,2.2,21.7,6.5,28.1S/;"	i
DejaVuSans-30_00000029039857562496777250000000599676036505405831_	figures/combined-sparsity-plots.svg	/^							s-10.6-9.7-18.7-9.7c-8.2,0-14.4,3.2-18.7,9.7s-6.5,15.8-6.5,28.1c0,12.3,2.2,21.7,6.5,28.1S/;"	i
DejaVuSans-30_00000029750333870484924650000011704616615096834177_	figures/combined-sparsity-plots.svg	/^							C-581.7,321.1-575.5,324.4-567.3,324.4z"\/>$/;"	i
DejaVuSans-30_00000029759327791112641150000013042589633837898648_	figures/combined-sparsity-plots.svg	/^							s-10.6-9.7-18.7-9.7c-8.2,0-14.4,3.2-18.7,9.7s-6.5,15.8-6.5,28.1c0,12.3,2.2,21.7,6.5,28.1S/;"	i
DejaVuSans-30_00000033357577772361811650000000932268821121753755_	figures/combined-sparsity-plots.svg	/^							C-518.1,321.1-511.9,324.4-503.7,324.4z"\/>$/;"	i
DejaVuSans-30_00000034063494508121330000000009668461870458568875_	figures/combined-sparsity-plots.svg	/^						C-516.8,2363.8-510.6,2367.1-502.4,2367.1z"\/>$/;"	i
DejaVuSans-30_00000034067370764261387080000005284178778790544779_	figures/combined-sparsity-plots.svg	/^							C-652.8-4427.2-646.6-4423.9-638.4-4423.9z"\/>$/;"	i
DejaVuSans-30_00000035503189656106778410000016605213528309604789_	figures/combined-sparsity-plots.svg	/^							C-709,411.1-702.8,414.4-694.6,414.4z"\/>$/;"	i
DejaVuSans-30_00000036966438665421758190000004998179586887449473_	figures/combined-sparsity-plots.svg	/^							C-645.4,411.1-639.1,414.4-631,414.4z"\/>$/;"	i
DejaVuSans-30_00000039839557644147079610000013726594823275252408_	figures/combined-sparsity-plots.svg	/^							C-518.1,321.1-511.9,324.4-503.7,324.4z"\/>$/;"	i
DejaVuSans-30_00000042007678270082986510000002144418017868062632_	figures/combined-sparsity-plots.svg	/^							S-641.7-4427.3-633.5-4427.3z"\/>$/;"	i
DejaVuSans-30_00000045579654104233649790000005965404091549085073_	figures/combined-sparsity-plots.svg	/^						C-580.4,2363.8-574.2,2367.1-566,2367.1z"\/>$/;"	i
DejaVuSans-30_00000045586271030470905230000005868229350516981130_	figures/combined-sparsity-plots.svg	/^							C-581.7,321.1-575.5,324.4-567.3,324.4z"\/>$/;"	i
DejaVuSans-30_00000045608560271419017640000013523618641904409259_	figures/combined-sparsity-plots.svg	/^						C-707.7,2363.8-701.5,2367.1-693.3,2367.1z"\/>$/;"	i
DejaVuSans-30_00000046302576918194038540000014073381359677053061_	figures/combined-sparsity-plots.svg	/^						C-612.3,387.2-606.1,390.4-597.9,390.4z"\/>$/;"	i
DejaVuSans-30_00000047754565307488081600000013468651999027538589_	figures/combined-sparsity-plots.svg	/^							C-581.7,321.1-575.5,324.4-567.3,324.4z"\/>$/;"	i
DejaVuSans-30_00000051346376381417743540000012028844152747552649_	figures/combined-sparsity-plots.svg	/^						C-644.1,2363.8-637.8,2367.1-629.7,2367.1z"\/>$/;"	i
DejaVuSans-30_00000051382061687270417340000010632065695119734414_	figures/combined-sparsity-plots.svg	/^							s-10.6-9.7-18.7-9.7c-8.2,0-14.4,3.2-18.7,9.7s-6.5,15.8-6.5,28.1c0,12.3,2.2,21.7,6.5,28.1S/;"	i
DejaVuSans-30_00000052080918089131199260000000746737154185866676_	figures/combined-sparsity-plots.svg	/^						C-612.3,387.2-606.1,390.4-597.9,390.4z"\/>$/;"	i
DejaVuSans-30_00000053538466432957788410000013080946036071960449_	figures/combined-sparsity-plots.svg	/^							C-645.4,411.1-639.1,414.4-631,414.4z"\/>$/;"	i
DejaVuSans-30_00000054254313552611437110000017875336989832244905_	figures/combined-sparsity-plots.svg	/^							C-518.1,321.1-511.9,324.4-503.7,324.4z"\/>$/;"	i
DejaVuSans-30_00000055685859524875050820000000505633290830974384_	figures/combined-sparsity-plots.svg	/^						C-580.4,2363.8-574.2,2367.1-566,2367.1z"\/>$/;"	i
DejaVuSans-30_00000057110723591222256570000002940595688108223409_	figures/combined-sparsity-plots.svg	/^							C-709,321.1-702.8,324.4-694.6,324.4z"\/>$/;"	i
DejaVuSans-30_00000057835754479811406400000009818998064689305774_	figures/combined-sparsity-plots.svg	/^							C-581.7,321.1-575.5,324.4-567.3,324.4z"\/>$/;"	i
DejaVuSans-30_00000057836779582744843780000007448880551526733496_	figures/combined-sparsity-plots.svg	/^							C-581.7,411.1-575.5,414.4-567.3,414.4z"\/>$/;"	i
DejaVuSans-30_00000062175870518631948210000004324614900246197131_	figures/combined-sparsity-plots.svg	/^						C-675.9,387.2-669.7,390.4-661.5,390.4z"\/>$/;"	i
DejaVuSans-30_00000062186301458136282720000017172946273450643863_	figures/combined-sparsity-plots.svg	/^							s-10.6-9.7-18.7-9.7c-8.2,0-14.4,3.2-18.7,9.7s-6.5,15.8-6.5,28.1c0,12.3,2.2,21.7,6.5,28.1S/;"	i
DejaVuSans-30_00000063602495581979919520000010127012126074450826_	figures/combined-sparsity-plots.svg	/^							C-581.7,321.1-575.5,324.4-567.3,324.4z"\/>$/;"	i
DejaVuSans-30_00000063613675345627678350000015565254413634879375_	figures/combined-sparsity-plots.svg	/^							S-583-4423.9-574.8-4423.9z"\/>$/;"	i
DejaVuSans-30_00000063616499424227362490000010904013366152211867_	figures/combined-sparsity-plots.svg	/^							C-613.6,321.1-607.3,324.4-599.2,324.4z"\/>$/;"	i
DejaVuSans-30_00000068643275532080115890000015080081654585429379_	figures/combined-sparsity-plots.svg	/^							C-518.1,321.1-511.9,324.4-503.7,324.4z"\/>$/;"	i
DejaVuSans-30_00000068650899037864751730000017143112508560794258_	figures/combined-sparsity-plots.svg	/^							C-518.1,321.1-511.9,324.4-503.7,324.4z"\/>$/;"	i
DejaVuSans-30_00000069363170427088266600000013900800351737992325_	figures/combined-sparsity-plots.svg	/^							C-709,411.1-702.8,414.4-694.6,414.4z"\/>$/;"	i
DejaVuSans-30_00000070082698613743551990000015776512573932713112_	figures/combined-sparsity-plots.svg	/^							C-709,321.1-702.8,324.4-694.6,324.4z"\/>$/;"	i
DejaVuSans-30_00000070111324442959534880000016357368129023540620_	figures/combined-sparsity-plots.svg	/^							C-645.4,411.1-639.1,414.4-631,414.4z"\/>$/;"	i
DejaVuSans-30_00000072272899114426986320000016501523156382677894_	figures/combined-sparsity-plots.svg	/^							S-583-4423.9-574.8-4423.9z"\/>$/;"	i
DejaVuSans-30_00000072980398008518693320000004735979791724951699_	figures/combined-sparsity-plots.svg	/^						C-612.3,387.2-606.1,390.4-597.9,390.4z"\/>$/;"	i
DejaVuSans-30_00000075130552306842209260000015705675652331380629_	figures/combined-sparsity-plots.svg	/^							C-709,321.1-702.8,324.4-694.6,324.4z"\/>$/;"	i
DejaVuSans-30_00000077287604234468892010000013684438432495044740_	figures/combined-sparsity-plots.svg	/^							C-581.7,411.1-575.5,414.4-567.3,414.4z"\/>$/;"	i
DejaVuSans-30_00000078740195848094012800000010107672877020122002_	figures/combined-sparsity-plots.svg	/^						C-516.8,2363.8-510.6,2367.1-502.4,2367.1z"\/>$/;"	i
DejaVuSans-30_00000078755174886367272680000004185627451921380791_	figures/combined-sparsity-plots.svg	/^							C-621.1-4427.2-614.8-4423.9-606.6-4423.9z"\/>$/;"	i
DejaVuSans-30_00000079461916766423933950000016237062816912927154_	figures/combined-sparsity-plots.svg	/^							C-709,421.1-702.8,424.4-694.6,424.4z"\/>$/;"	i
DejaVuSans-30_00000080189268371180191230000004890166477996133035_	figures/combined-sparsity-plots.svg	/^							C-709,321.1-702.8,324.4-694.6,324.4z"\/>$/;"	i
DejaVuSans-30_00000080194574580869119470000005690303376508175037_	figures/combined-sparsity-plots.svg	/^							C-584.3-4430.6-578.1-4427.3-569.9-4427.3z"\/>$/;"	i
DejaVuSans-30_00000081613161810639031550000014863922625495882423_	figures/combined-sparsity-plots.svg	/^							s-10.6-9.7-18.7-9.7c-8.2,0-14.4,3.2-18.7,9.7s-6.5,15.8-6.5,28.1c0,12.3,2.2,21.7,6.5,28.1S/;"	i
DejaVuSans-30_00000082329165922565066990000002976474582646048647_	figures/combined-sparsity-plots.svg	/^							C-584.3-4430.6-578.1-4427.3-569.9-4427.3z"\/>$/;"	i
DejaVuSans-30_00000082330856946855300740000013647921006187272869_	figures/combined-sparsity-plots.svg	/^							C-709,411.1-702.8,414.4-694.6,414.4z"\/>$/;"	i
DejaVuSans-30_00000082358389015290685950000003945577382042221238_	figures/combined-sparsity-plots.svg	/^						C-612.3,387.2-606.1,390.4-597.9,390.4z"\/>$/;"	i
DejaVuSans-30_00000087389183472482532650000015659298942834992571_	figures/combined-sparsity-plots.svg	/^						C1999,797.4,2005.2,800.6,2013.4,800.6z"\/>$/;"	i
DejaVuSans-30_00000089569065717059841560000015087623191526822825_	figures/combined-sparsity-plots.svg	/^							C-581.7,411.1-575.5,414.4-567.3,414.4z"\/>$/;"	i
DejaVuSans-30_00000090260040733519012790000008230725317372720541_	figures/combined-sparsity-plots.svg	/^							C-709,321.1-702.8,324.4-694.6,324.4z"\/>$/;"	i
DejaVuSans-30_00000093171508517274376680000004762202206668037008_	figures/combined-sparsity-plots.svg	/^							C-709,321.1-702.8,324.4-694.6,324.4z"\/>$/;"	i
DejaVuSans-30_00000093856896554565382030000005976255460139047565_	figures/combined-sparsity-plots.svg	/^							S-583-4423.9-574.8-4423.9z"\/>$/;"	i
DejaVuSans-30_00000094587370847446450640000012326719988363352989_	figures/combined-sparsity-plots.svg	/^							C-709,321.1-702.8,324.4-694.6,324.4z"\/>$/;"	i
DejaVuSans-30_00000095322354444910436070000015404088441930100122_	figures/combined-sparsity-plots.svg	/^							C-652.8-4427.2-646.6-4423.9-638.4-4423.9z"\/>$/;"	i
DejaVuSans-30_00000095331404460653879830000000702127527761855413_	figures/combined-sparsity-plots.svg	/^							s-10.6-9.7-18.7-9.7c-8.2,0-14.4,3.2-18.7,9.7s-6.5,15.8-6.5,28.1c0,12.3,2.2,21.7,6.5,28.1S/;"	i
DejaVuSans-30_00000102524410656094391220000002395355796097207437_	figures/combined-sparsity-plots.svg	/^							C-581.7,321.1-575.5,324.4-567.3,324.4z"\/>$/;"	i
DejaVuSans-30_00000104667392742573966430000000270341149413454223_	figures/combined-sparsity-plots.svg	/^							C-709,421.1-702.8,424.4-694.6,424.4z"\/>$/;"	i
DejaVuSans-30_00000104679610825933391850000007453640348154700975_	figures/combined-sparsity-plots.svg	/^							S-641.7-4427.3-633.5-4427.3z"\/>$/;"	i
DejaVuSans-30_00000105401987511141613580000001923835882744264848_	figures/combined-sparsity-plots.svg	/^						C-612.3,387.2-606.1,390.4-597.9,390.4z"\/>$/;"	i
DejaVuSans-30_00000106113375609285281240000005558998999450749585_	figures/combined-sparsity-plots.svg	/^							C-709,421.1-702.8,424.4-694.6,424.4z"\/>$/;"	i
DejaVuSans-30_00000106133379901406417320000006012338357617033137_	figures/combined-sparsity-plots.svg	/^							C-652.8-4427.2-646.6-4423.9-638.4-4423.9z"\/>$/;"	i
DejaVuSans-30_00000109725597455011496020000017304962269500174475_	figures/combined-sparsity-plots.svg	/^							s-10.6-9.7-18.7-9.7c-8.2,0-14.4,3.2-18.7,9.7s-6.5,15.8-6.5,28.1c0,12.3,2.2,21.7,6.5,28.1S/;"	i
DejaVuSans-30_00000109744555593562359420000015952157289367112868_	figures/combined-sparsity-plots.svg	/^						C-516.8,2363.8-510.6,2367.1-502.4,2367.1z"\/>$/;"	i
DejaVuSans-30_00000112620889408619142780000005389112921340583843_	figures/combined-sparsity-plots.svg	/^							s-10.6-9.7-18.7-9.7c-8.2,0-14.4,3.2-18.7,9.7s-6.5,15.8-6.5,28.1c0,12.3,2.2,21.7,6.5,28.1S/;"	i
DejaVuSans-30_00000119112333827515713410000002888577532346449291_	figures/combined-sparsity-plots.svg	/^							C-518.1,321.1-511.9,324.4-503.7,324.4z"\/>$/;"	i
DejaVuSans-30_00000121249155931767717530000006489433910624389565_	figures/combined-sparsity-plots.svg	/^							C-709,321.1-702.8,324.4-694.6,324.4z"\/>$/;"	i
DejaVuSans-30_00000121263109040093214640000005038839713810950555_	figures/combined-sparsity-plots.svg	/^							C-581.7,321.1-575.5,324.4-567.3,324.4z"\/>$/;"	i
DejaVuSans-30_00000124121881618074985180000016015022359797154181_	figures/combined-sparsity-plots.svg	/^							C-613.6,411.1-607.3,414.4-599.2,414.4z"\/>$/;"	i
DejaVuSans-30_00000127021894199198301460000005207189987760300457_	figures/combined-sparsity-plots.svg	/^							s-10.6-9.7-18.7-9.7c-8.2,0-14.4,3.2-18.7,9.7s-6.5,15.8-6.5,28.1c0,12.3,2.2,21.7,6.5,28.1S/;"	i
DejaVuSans-30_00000132771170768231311560000010003743897715817352_	figures/combined-sparsity-plots.svg	/^							C-613.6,321.1-607.3,324.4-599.2,324.4z"\/>$/;"	i
DejaVuSans-30_00000134231068736742385200000003675110742578488990_	figures/combined-sparsity-plots.svg	/^							S-583-4423.9-574.8-4423.9z"\/>$/;"	i
DejaVuSans-30_00000134241770547612408450000016028906263711517601_	figures/combined-sparsity-plots.svg	/^						C-580.4,2363.8-574.2,2367.1-566,2367.1z"\/>$/;"	i
DejaVuSans-30_00000134247390813898753780000015632495947402105998_	figures/combined-sparsity-plots.svg	/^						C-612.3,387.2-606.1,390.4-597.9,390.4z"\/>$/;"	i
DejaVuSans-30_00000137094097612068936780000006787692290821019021_	figures/combined-sparsity-plots.svg	/^						C-580.4,2363.8-574.2,2367.1-566,2367.1z"\/>$/;"	i
DejaVuSans-30_00000140712811997847124560000007332287301085733024_	figures/combined-sparsity-plots.svg	/^							C-645.4,321.1-639.1,324.4-631,324.4z"\/>$/;"	i
DejaVuSans-30_00000141440325763418643650000016262554671018419376_	figures/combined-sparsity-plots.svg	/^							s-10.6-9.7-18.7-9.7c-8.2,0-14.4,3.2-18.7,9.7s-6.5,15.8-6.5,28.1c0,12.3,2.2,21.7,6.5,28.1S/;"	i
DejaVuSans-30_00000144304676461565130910000011590710045669837203_	figures/combined-sparsity-plots.svg	/^							C-581.7,411.1-575.5,414.4-567.3,414.4z"\/>$/;"	i
DejaVuSans-30_00000149378742229938633300000000782663985131392440_	figures/combined-sparsity-plots.svg	/^							C-581.7,321.1-575.5,324.4-567.3,324.4z"\/>$/;"	i
DejaVuSans-30_00000150068455576241214550000014618636248990218429_	figures/combined-sparsity-plots.svg	/^							C-581.7,411.1-575.5,414.4-567.3,414.4z"\/>$/;"	i
DejaVuSans-30_00000150069771367430078690000000632005985028913802_	figures/combined-sparsity-plots.svg	/^							C-584.3-4430.6-578.1-4427.3-569.9-4427.3z"\/>$/;"	i
DejaVuSans-30_00000150096159832823139060000017251266589581226406_	figures/combined-sparsity-plots.svg	/^							C-645.4,321.1-639.1,324.4-631,324.4z"\/>$/;"	i
DejaVuSans-30_00000150815481165011756080000006815490800544037042_	figures/combined-sparsity-plots.svg	/^							C-709,321.1-702.8,324.4-694.6,324.4z"\/>$/;"	i
DejaVuSans-30_00000150821532624652496540000014082167818893601204_	figures/combined-sparsity-plots.svg	/^							C-652.8-4427.2-646.6-4423.9-638.4-4423.9z"\/>$/;"	i
DejaVuSans-30_00000152223112152942072550000010122112007522336428_	figures/combined-sparsity-plots.svg	/^							C-518.1,321.1-511.9,324.4-503.7,324.4z"\/>$/;"	i
DejaVuSans-30_00000154425648710698620720000013964126062818772878_	figures/combined-sparsity-plots.svg	/^							C-709,321.1-702.8,324.4-694.6,324.4z"\/>$/;"	i
DejaVuSans-30_00000155135357366078571610000015346321163859448996_	figures/combined-sparsity-plots.svg	/^						C-580.4,2363.8-574.2,2367.1-566,2367.1z"\/>$/;"	i
DejaVuSans-30_00000159437410161574994930000016985636268303985828_	figures/combined-sparsity-plots.svg	/^							C-645.4,411.1-639.1,414.4-631,414.4z"\/>$/;"	i
DejaVuSans-30_00000160158507955230057300000007701025416253858474_	figures/combined-sparsity-plots.svg	/^							C-709,411.1-702.8,414.4-694.6,414.4z"\/>$/;"	i
DejaVuSans-30_00000160164269605949551060000000025858812335528887_	figures/combined-sparsity-plots.svg	/^						C-516.8,2363.8-510.6,2367.1-502.4,2367.1z"\/>$/;"	i
DejaVuSans-30_00000162341587380430046530000002007638963480640393_	figures/combined-sparsity-plots.svg	/^						C1550.9,797.4,1557.1,800.6,1565.3,800.6z"\/>$/;"	i
DejaVuSans-30_00000163770078405227036540000013889307173773259699_	figures/combined-sparsity-plots.svg	/^						C-644.1,2363.8-637.8,2367.1-629.7,2367.1z"\/>$/;"	i
DejaVuSans-30_00000164479283626744396660000018074720221630279600_	figures/combined-sparsity-plots.svg	/^							C-581.7,321.1-575.5,324.4-567.3,324.4z"\/>$/;"	i
DejaVuSans-30_00000164499831800981697320000005143723755566708619_	figures/combined-sparsity-plots.svg	/^							C-652.8-4427.2-646.6-4423.9-638.4-4423.9z"\/>$/;"	i
DejaVuSans-30_00000168812890259019267520000003980394270934997694_	figures/combined-sparsity-plots.svg	/^						C-612.3,387.2-606.1,390.4-597.9,390.4z"\/>$/;"	i
DejaVuSans-30_00000170237493115250844730000015985335609536005794_	figures/combined-sparsity-plots.svg	/^							C-645.4,411.1-639.1,414.4-631,414.4z"\/>$/;"	i
DejaVuSans-30_00000170262333167917832790000001637869691618956989_	figures/combined-sparsity-plots.svg	/^						C-612.3,387.2-606.1,390.4-597.9,390.4z"\/>$/;"	i
DejaVuSans-30_00000170984147838135323450000006973505681438748074_	figures/combined-sparsity-plots.svg	/^							C-709,421.1-702.8,424.4-694.6,424.4z"\/>$/;"	i
DejaVuSans-30_00000173158222125975696290000004049684580808147622_	figures/combined-sparsity-plots.svg	/^							C-518.1,321.1-511.9,324.4-503.7,324.4z"\/>$/;"	i
DejaVuSans-30_00000174589446743290534260000004174868099268597935_	figures/combined-sparsity-plots.svg	/^							s-10.6-9.7-18.7-9.7c-8.2,0-14.4,3.2-18.7,9.7s-6.5,15.8-6.5,28.1c0,12.3,2.2,21.7,6.5,28.1S/;"	i
DejaVuSans-30_00000178166599255483692170000012996097545543053500_	figures/combined-sparsity-plots.svg	/^							s-10.6-9.7-18.7-9.7c-8.2,0-14.4,3.2-18.7,9.7s-6.5,15.8-6.5,28.1c0,12.3,2.2,21.7,6.5,28.1S/;"	i
DejaVuSans-30_00000181078573574186182820000001138011467323782077_	figures/combined-sparsity-plots.svg	/^							C-709,321.1-702.8,324.4-694.6,324.4z"\/>$/;"	i
DejaVuSans-30_00000183932923519390085520000005235479399477239960_	figures/combined-sparsity-plots.svg	/^							C-645.4,321.1-639.1,324.4-631,324.4z"\/>$/;"	i
DejaVuSans-31_00000018218283320255539050000009718952252950567812_	figures/combined-sparsity-plots.svg	/^							l17.4,3.5h9.9v-64.6h16.1v-8.3h-42V-4493.3z"\/>$/;"	i
DejaVuSans-31_00000020382529495337232130000005302697125966456716_	figures/combined-sparsity-plots.svg	/^						l17.4,3.5h9.9v-64.6h16.1v-8.3h-42V2301.1z"\/>$/;"	i
DejaVuSans-31_00000027592553185297233670000013345868402014435739_	figures/combined-sparsity-plots.svg	/^							l17.4,3.5h9.9v-64.6h16.1v-8.3h-42V-4489.9z"\/>$/;"	i
DejaVuSans-31_00000047771885016384825510000003142051455705015450_	figures/combined-sparsity-plots.svg	/^							h9.9v-64.6h16.1v-8.3h-42V258.4z"\/>$/;"	i
DejaVuSans-31_00000068672091308357063340000017288544470722493320_	figures/combined-sparsity-plots.svg	/^							h9.9v-64.6h16.1v-8.3h-42V258.4z"\/>$/;"	i
DejaVuSans-31_00000074407414476304076570000013918588270420790709_	figures/combined-sparsity-plots.svg	/^							h9.9v-64.6h16.1v-8.3h-42V258.4z"\/>$/;"	i
DejaVuSans-31_00000091707629037581364110000000361287181611806384_	figures/combined-sparsity-plots.svg	/^						l17.4,3.5h9.9v-64.6h16.1v-8.3h-42V2301.1z"\/>$/;"	i
DejaVuSans-31_00000099651071325849880620000009099840671276134059_	figures/combined-sparsity-plots.svg	/^						l17.4,3.5h9.9v-64.6h16.1v-8.3h-42V2301.1z"\/>$/;"	i
DejaVuSans-31_00000109709426733532242300000005501907580141960871_	figures/combined-sparsity-plots.svg	/^							h9.9v-64.6h16.1v-8.3h-42V258.4z"\/>$/;"	i
DejaVuSans-31_00000119825462073358631640000007655537143743015306_	figures/combined-sparsity-plots.svg	/^							h9.9v-64.6h16.1v-8.3h-42V258.4z"\/>$/;"	i
DejaVuSans-31_00000121986717684649326720000014976156559449513091_	figures/combined-sparsity-plots.svg	/^							l17.4,3.5h9.9v-64.6h16.1v-8.3h-42V-4493.3z"\/>$/;"	i
DejaVuSans-31_00000129907022450403065430000008436949722138026144_	figures/combined-sparsity-plots.svg	/^							h9.9v-64.6h16.1v-8.3h-42V258.4z"\/>$/;"	i
DejaVuSans-31_00000131346888674424497440000015446466227898563219_	figures/combined-sparsity-plots.svg	/^							h9.9v-64.6h16.1v-8.3h-42V258.4z"\/>$/;"	i
DejaVuSans-31_00000134228817449210125750000005040129129381022345_	figures/combined-sparsity-plots.svg	/^						l17.4,3.5h9.9v-64.6h16.1v-8.3h-42V2301.1z"\/>$/;"	i
DejaVuSans-31_00000137823461874164291920000015518573840709432980_	figures/combined-sparsity-plots.svg	/^						l17.4,3.5h9.9v-64.6h16.1v-8.3h-42V324.5z"\/>$/;"	i
DejaVuSans-31_00000160163308442471720820000006493370044173847740_	figures/combined-sparsity-plots.svg	/^							l17.4,3.5h9.9v-64.6h16.1v-8.3h-42V-4493.3z"\/>$/;"	i
DejaVuSans-31_00000162342677554347698030000000398149961603990419_	figures/combined-sparsity-plots.svg	/^							l17.4,3.5h9.9v-64.6h16.1v-8.3h-42V-4493.3z"\/>$/;"	i
DejaVuSans-31_00000163756118730809960770000013202583952944799632_	figures/combined-sparsity-plots.svg	/^							h9.9v-64.6h16.1v-8.3h-42V258.4z"\/>$/;"	i
DejaVuSans-31_00000168814043367402134470000004523058362002749592_	figures/combined-sparsity-plots.svg	/^							h9.9v-64.6h16.1v-8.3h-42V258.4z"\/>$/;"	i
DejaVuSans-31_00000174583176109002569210000009473623169953113535_	figures/combined-sparsity-plots.svg	/^							h9.9v-64.6h16.1v-8.3h-42V348.4z"\/>$/;"	i
DejaVuSans-31_00000180357842419838361100000007078918664946096568_	figures/combined-sparsity-plots.svg	/^							h9.9v-64.6h16.1v-8.3h-42V258.4z"\/>$/;"	i
DejaVuSans-32_00000021810621619247320530000014765722345560048539_	figures/combined-sparsity-plots.svg	/^						c-0.8-0.9-3.4-3.7-7.8-8.2C-660,338.9-666.2,332.6-674.1,324.5z"\/>$/;"	i
DejaVuSans-32_00000024693523853653453560000018018763872395571337_	figures/combined-sparsity-plots.svg	/^							c-0.8-0.9-3.4-3.7-7.8-8.2C-700.5-4475.4-706.7-4481.8-714.6-4489.9z"\/>$/;"	i
DejaVuSans-32_00000056405245612592316530000011319361297115175573_	figures/combined-sparsity-plots.svg	/^							c-0.8-0.9-3.4-3.7-7.8-8.2C-693.1,272.8-699.2,266.5-707.2,258.4z"\/>$/;"	i
DejaVuSans-32_00000063631827081292065190000005908732869365528239_	figures/combined-sparsity-plots.svg	/^							c-0.8-0.9-3.4-3.7-7.8-8.2C-600.2-4478.9-606.4-4485.2-614.3-4493.3z"\/>$/;"	i
DejaVuSans-32_00000088825191520434309760000017823029453398612365_	figures/combined-sparsity-plots.svg	/^							c-0.8-0.9-3.4-3.7-7.8-8.2C-605.1-4475.4-611.3-4481.8-619.2-4489.9z"\/>$/;"	i
DejaVuSans-32_00000093141779390458242420000003183308670023172741_	figures/combined-sparsity-plots.svg	/^							c-0.8-0.9-3.4-3.7-7.8-8.2C-632-4478.9-638.2-4485.2-646.1-4493.3z"\/>$/;"	i
DejaVuSans-32_00000094586413220886362880000016238707711212340138_	figures/combined-sparsity-plots.svg	/^							c-0.8-0.9-3.4-3.7-7.8-8.2C-597.7,372.8-603.8,366.5-611.8,358.4z"\/>$/;"	i
DejaVuSans-32_00000102543667091513030250000003472025509589253533_	figures/combined-sparsity-plots.svg	/^							c-0.8-0.9-3.4-3.7-7.8-8.2C-597.7,362.8-603.8,356.5-611.8,348.4z"\/>$/;"	i
DejaVuSans-32_00000115512672742482984550000006745583511801867659_	figures/combined-sparsity-plots.svg	/^							c-0.8-0.9-3.4-3.7-7.8-8.2C-693.1,362.8-699.2,356.5-707.2,348.4z"\/>$/;"	i
DejaVuSans-32_00000132766194396532599500000006762502700682397083_	figures/combined-sparsity-plots.svg	/^						c-0.8-0.9-3.4-3.7-7.8-8.2C-628.2,2315.5-634.3,2309.2-642.3,2301.1z"\/>$/;"	i
DejaVuSans-32_00000132782276212627052410000013008628218770101151_	figures/combined-sparsity-plots.svg	/^							c-0.8-0.9-3.4-3.7-7.8-8.2C-695.6-4478.9-701.8-4485.2-709.7-4493.3z"\/>$/;"	i
DejaVuSans-32_00000139287570622375154870000006589353007577110186_	figures/combined-sparsity-plots.svg	/^							c-0.8-0.9-3.4-3.7-7.8-8.2C-629.5,272.8-635.6,266.5-643.6,258.4z"\/>$/;"	i
DejaVuSans-32_00000142867913662667213440000001437026186043282855_	figures/combined-sparsity-plots.svg	/^							c-0.8-0.9-3.4-3.7-7.8-8.2C-629.5,272.8-635.6,266.5-643.6,258.4z"\/>$/;"	i
DejaVuSans-32_00000165235711736150148270000018431739966805949056_	figures/combined-sparsity-plots.svg	/^							c-0.8-0.9-3.4-3.7-7.8-8.2C-693.1,272.8-699.2,266.5-707.2,258.4z"\/>$/;"	i
DejaVuSans-32_00000166657824489555542490000018298753742372082104_	figures/combined-sparsity-plots.svg	/^						c-0.8-0.9-3.4-3.7-7.8-8.2C-691.8,2315.5-697.9,2309.2-705.9,2301.1z"\/>$/;"	i
DejaVuSans-33	figures/combined-sparsity-plots.svg	/^							S-689-4457.8-693.3-4458.8z"\/>$/;"	i
DejaVuSans-33_00000051371811686950027810000006864642866578937253_	figures/combined-sparsity-plots.svg	/^						c7.5,0,13.4-1.7,17.8-5.1c4.4-3.4,6.5-8,6.5-13.8c0-4-1.2-7.5-3.5-10.2S-648.5,356.6-652.7,35/;"	i
DejaVuSans-33_00000156560132486900903680000016500073631717952912_	figures/combined-sparsity-plots.svg	/^							c4.4-3.4,6.5-8,6.5-13.8c0-4-1.2-7.5-3.5-10.2S-681.5,380.5-685.8,379.5z"\/>$/;"	i
DejaVuSans-34_00000019669455955418661250000017256416545217388462_	figures/combined-sparsity-plots.svg	/^							 M-603.2-4425.2h12.4v-47.5h10.4v-8.2h-10.4v-17.2h-9.8v17.2h-32.9v9.5L-603.2-4425.2z"\/>$/;"	i
DejaVuSans-34_00000067925876492080628510000016480307908463256999_	figures/combined-sparsity-plots.svg	/^							 M-595.8,413h12.4v-47.5h10.4v-8.2h-10.4v-17.2h-9.8v17.2h-32.9v9.5L-595.8,413z"\/>$/;"	i
DejaVuSans-34_00000093885955143799942800000006486917450747031937_	figures/combined-sparsity-plots.svg	/^							 M-691.2,413h12.4v-47.5h10.4v-8.2h-10.4v-17.2h-9.8v17.2h-32.9v9.5L-691.2,413z"\/>$/;"	i
DejaVuSans-34_00000095319658090913029180000016978673772049494717_	figures/combined-sparsity-plots.svg	/^							 M-698.6-4425.2h12.4v-47.5h10.4v-8.2h-10.4v-17.2h-9.8v17.2h-32.9v9.5L-698.6-4425.2z"\/>$/;"	i
DejaVuSans-34_00000099629737810956846340000010572344426381259919_	figures/combined-sparsity-plots.svg	/^							 M-598.3-4428.7h12.4v-47.5h10.4v-8.2h-10.4v-17.2h-9.8v17.2h-32.9v9.5L-598.3-4428.7z"\/>$/;"	i
DejaVuSans-34_00000125581301968594655260000017420003338783472783_	figures/combined-sparsity-plots.svg	/^						 M-658.1,389.1h12.4v-47.5h10.4v-8.2h-10.4v-17.2h-9.8v17.2h-32.9v9.5L-658.1,389.1z"\/>$/;"	i
DejaVuSans-34_00000134941745493278088930000012531927968710390704_	figures/combined-sparsity-plots.svg	/^							 M-595.8,423h12.4v-47.5h10.4v-8.2h-10.4v-17.2h-9.8v17.2h-32.9v9.5L-595.8,423z"\/>$/;"	i
DejaVuSans-35_00000008118368543674201540000013907922664150206099_	figures/combined-sparsity-plots.svg	/^							c-2.6,0-5.3-0.3-7.9-0.9c-2.6-0.6-5.3-1.5-8-2.7V413H-715.6z"\/>$/;"	i
DejaVuSans-35_00000011747268279728947370000006653662874250853290_	figures/combined-sparsity-plots.svg	/^						c-2.6-0.6-5.3-1.5-8-2.7v36.7H-587z"\/>$/;"	i
DejaVuSans-35_00000012464148371433114660000016763194794683794582_	figures/combined-sparsity-plots.svg	/^						c-2.6-0.6-5.3-1.5-8-2.7v36.7H-714.3z"\/>$/;"	i
DejaVuSans-35_00000016070588370875067650000008993449657908527237_	figures/combined-sparsity-plots.svg	/^							c-2.6,0-5.3-0.3-7.9-0.9c-2.6-0.6-5.3-1.5-8-2.7V323H-652z"\/>$/;"	i
DejaVuSans-35_00000022550848845160232860000001878536275473577393_	figures/combined-sparsity-plots.svg	/^						c-2.6-0.6-5.3-1.5-8-2.7v36.7H-682.5z"\/>$/;"	i
DejaVuSans-35_00000023249686561915673720000004812796055155677101_	figures/combined-sparsity-plots.svg	/^						c-2.6-0.6-5.3-1.5-8-2.7v36.7H-587z"\/>$/;"	i
DejaVuSans-35_00000034786665350858791920000017890400823312540583_	figures/combined-sparsity-plots.svg	/^						c-2.6-0.6-5.3-1.5-8-2.7v36.7H-650.7z"\/>$/;"	i
DejaVuSans-35_00000038402707921700232000000017859976686466479030_	figures/combined-sparsity-plots.svg	/^							c-2.6,0-5.3-0.3-7.9-0.9c-2.6-0.6-5.3-1.5-8-2.7V323H-652z"\/>$/;"	i
DejaVuSans-35_00000044888726000207339250000015970367224136464268_	figures/combined-sparsity-plots.svg	/^						c-2.6-0.6-5.3-1.5-8-2.7v36.7H-650.7z"\/>$/;"	i
DejaVuSans-35_00000047050482456399878610000006258791071035101613_	figures/combined-sparsity-plots.svg	/^							c-2.6,0-5.3-0.3-7.9-0.9c-2.6-0.6-5.3-1.5-8-2.7V323H-588.3z"\/>$/;"	i
DejaVuSans-35_00000050621972416904425280000014963396537093353603_	figures/combined-sparsity-plots.svg	/^							c-2.6,0-5.3-0.3-7.9-0.9c-2.6-0.6-5.3-1.5-8-2.7V323H-588.3z"\/>$/;"	i
DejaVuSans-35_00000051369383475329974300000006549556642788256147_	figures/combined-sparsity-plots.svg	/^							c-2.6,0-5.3-0.3-7.9-0.9c-2.6-0.6-5.3-1.5-8-2.7V323H-620.2z"\/>$/;"	i
DejaVuSans-35_00000053529569438784784270000012098519444111103411_	figures/combined-sparsity-plots.svg	/^							c-2.6,0-5.3-0.3-7.9-0.9c-2.6-0.6-5.3-1.5-8-2.7V323H-652z"\/>$/;"	i
DejaVuSans-35_00000056422765999647751380000017608535517558011021_	figures/combined-sparsity-plots.svg	/^							c-2.6,0-5.3-0.3-7.9-0.9c-2.6-0.6-5.3-1.5-8-2.7v36.7H-590.9z"\/>$/;"	i
DejaVuSans-35_00000060011883861267187090000016159006799350848397_	figures/combined-sparsity-plots.svg	/^							c-2.6,0-5.3-0.3-7.9-0.9c-2.6-0.6-5.3-1.5-8-2.7v36.7H-654.5z"\/>$/;"	i
DejaVuSans-35_00000067932908629602969310000008975364225297077653_	figures/combined-sparsity-plots.svg	/^							c-2.6,0-5.3-0.3-7.9-0.9c-2.6-0.6-5.3-1.5-8-2.7V323H-715.6z"\/>$/;"	i
DejaVuSans-35_00000075126133686214869400000003322574711089456257_	figures/combined-sparsity-plots.svg	/^							c-2.6,0-5.3-0.3-7.9-0.9c-2.6-0.6-5.3-1.5-8-2.7V323H-588.3z"\/>$/;"	i
DejaVuSans-35_00000077307334033984245820000008514393293091730854_	figures/combined-sparsity-plots.svg	/^							c-2.6,0-5.3-0.3-7.9-0.9c-2.6-0.6-5.3-1.5-8-2.7v36.7H-723z"\/>$/;"	i
DejaVuSans-35_00000080893835850598628190000013043175876812704150_	figures/combined-sparsity-plots.svg	/^							c-2.6,0-5.3-0.3-7.9-0.9c-2.6-0.6-5.3-1.5-8-2.7V323H-652z"\/>$/;"	i
DejaVuSans-35_00000092441126674255937360000006265123742167549364_	figures/combined-sparsity-plots.svg	/^							c-2.6,0-5.3-0.3-7.9-0.9c-2.6-0.6-5.3-1.5-8-2.7v36.7H-590.9z"\/>$/;"	i
DejaVuSans-35_00000111903706077285169710000005938842713151808657_	figures/combined-sparsity-plots.svg	/^							c-2.6,0-5.3-0.3-7.9-0.9c-2.6-0.6-5.3-1.5-8-2.7V323H-652z"\/>$/;"	i
DejaVuSans-35_00000115516479312868344800000009199414853144704669_	figures/combined-sparsity-plots.svg	/^							c-2.6,0-5.3-0.3-7.9-0.9c-2.6-0.6-5.3-1.5-8-2.7v36.7H-654.5z"\/>$/;"	i
DejaVuSans-35_00000116952045962691702980000017613507264207426233_	figures/combined-sparsity-plots.svg	/^							c-2.6,0-5.3-0.3-7.9-0.9c-2.6-0.6-5.3-1.5-8-2.7v36.7H-654.5z"\/>$/;"	i
DejaVuSans-35_00000144331146897057797380000004041875239063278270_	figures/combined-sparsity-plots.svg	/^						c-2.6-0.6-5.3-1.5-8-2.7v36.7H-650.7z"\/>$/;"	i
DejaVuSans-35_00000157990854727525805870000007678839019175711628_	figures/combined-sparsity-plots.svg	/^							c-2.6,0-5.3-0.3-7.9-0.9c-2.6-0.6-5.3-1.5-8-2.7v36.7H-718.1z"\/>$/;"	i
DejaVuSans-35_00000163766751523001188620000007125993962829701300_	figures/combined-sparsity-plots.svg	/^							c-2.6,0-5.3-0.3-7.9-0.9c-2.6-0.6-5.3-1.5-8-2.7V323H-588.3z"\/>$/;"	i
DejaVuSans-35_00000164503400834444423830000006466052095174422149_	figures/combined-sparsity-plots.svg	/^							c-2.6,0-5.3-0.3-7.9-0.9c-2.6-0.6-5.3-1.5-8-2.7V323H-715.6z"\/>$/;"	i
DejaVuSans-35_00000173122525215133979480000003325437221922651069_	figures/combined-sparsity-plots.svg	/^							c-2.6,0-5.3-0.3-7.9-0.9c-2.6-0.6-5.3-1.5-8-2.7V323H-652z"\/>$/;"	i
DejaVuSans-35_00000178201228991721968960000014905153865867661700_	figures/combined-sparsity-plots.svg	/^							c-2.6,0-5.3-0.3-7.9-0.9c-2.6-0.6-5.3-1.5-8-2.7V323H-620.2z"\/>$/;"	i
DejaVuSans-36_00000005947216752411923880000001086426224510945203_	figures/combined-sparsity-plots.svg	/^							c0,11.5,2.7,20.7,8.2,27.6s12.8,10.3,22,10.3c2.5,0,5-0.2,7.5-0.7C-583.7,413.1-581.1,412.4-/;"	i
DejaVuSans-36_00000011006320015942810940000008720082211144444039_	figures/combined-sparsity-plots.svg	/^							c0,11.5,2.7,20.7,8.2,27.6s12.8,10.3,22,10.3c2.5,0,5-0.2,7.5-0.7S-581.1,322.4-578.4,321.4z/;"	i
DejaVuSans-36_00000011713168779888074650000015619278907570570145_	figures/combined-sparsity-plots.svg	/^							c0,11.5,2.7,20.7,8.2,27.6s12.8,10.3,22,10.3c2.5,0,5-0.2,7.5-0.7S-676.5,412.4-673.8,411.4z/;"	i
DejaVuSans-36_00000036212062543715627170000004265696423748291488_	figures/combined-sparsity-plots.svg	/^							c0,11.5,2.7,20.7,8.2,27.6s12.8,10.3,22,10.3c2.5,0,5-0.2,7.5-0.7S-581.1,322.4-578.4,321.4z/;"	i
DejaVuSans-36_00000043420916412796338210000009572951814399223195_	figures/combined-sparsity-plots.svg	/^							c0,11.5,2.7,20.7,8.2,27.6s12.8,10.3,22,10.3c2.5,0,5-0.2,7.5-0.7S-588.6-4425.9-585.8-4426./;"	i
DejaVuSans-36_00000131348457804515078370000017639743400843813270_	figures/combined-sparsity-plots.svg	/^						c0,11.5,2.7,20.7,8.2,27.6s12.8,10.3,22,10.3c2.5,0,5-0.2,7.5-0.7C-646.1,389.2-643.5,388.5-6/;"	i
DejaVuSans-36_00000136386450044838266490000016119500790741124532_	figures/combined-sparsity-plots.svg	/^							c0,11.5,2.7,20.7,8.2,27.6s12.8,10.3,22,10.3c2.5,0,5-0.2,7.5-0.7C-583.7,423.1-581.1,422.4-/;"	i
DejaVuSans-36_00000152241977186214530320000012406149233645409685_	figures/combined-sparsity-plots.svg	/^							C-586.3-4428.6-583.7-4429.3-580.9-4430.3z"\/>$/;"	i
DejaVuSans-36_00000152970380763738288710000017639881812835711897_	figures/combined-sparsity-plots.svg	/^							c0,11.5,2.7,20.7,8.2,27.6s12.8,10.3,22,10.3c2.5,0,5-0.2,7.5-0.7S-684-4425.9-681.2-4426.9z/;"	i
DejaVuSans-37_00000005233916078304826470000010935275377396701329_	figures/combined-sparsity-plots.svg	/^						l24.9,64.6h-35C-653.2,2357.4-653.2,2365.7-653.2,2365.7z"\/>$/;"	i
DejaVuSans-37_00000013887028468248552900000004675277089915382192_	figures/combined-sparsity-plots.svg	/^							l24.9,64.6h-35C-622.8,314.7-622.8,323-622.8,323z"\/>$/;"	i
DejaVuSans-37_00000064317940925216473720000015795051264548804510_	figures/combined-sparsity-plots.svg	/^							l24.9,64.6h-35V-4428.7z"\/>$/;"	i
DejaVuSans-37_00000083782579147233738940000010269803391431081618_	figures/combined-sparsity-plots.svg	/^							l24.9,64.6h-35C-720.7-4437-720.7-4428.7-720.7-4428.7z"\/>$/;"	i
DejaVuSans-37_00000098186046007251217240000005980215431823917970_	figures/combined-sparsity-plots.svg	/^							l24.9,64.6h-35C-718.2,314.7-718.2,323-718.2,323z"\/>$/;"	i
DejaVuSans-37_00000130632577400285759920000000772670832653042059_	figures/combined-sparsity-plots.svg	/^							l24.9,64.6h-35C-654.5,314.7-654.5,323-654.5,323z"\/>$/;"	i
DejaVuSans-37_00000130641833619487322380000014113759436267211685_	figures/combined-sparsity-plots.svg	/^						l24.9,64.6h-35V389.1z"\/>$/;"	i
DejaVuSans-37_00000142151573171406777250000004685067269287909539_	figures/combined-sparsity-plots.svg	/^						l24.9,64.6h-35C-716.9,2357.4-716.9,2365.7-716.9,2365.7z"\/>$/;"	i
DejaVuSans-37_00000145750053405787425190000004405231333614476988_	figures/combined-sparsity-plots.svg	/^							l24.9,64.6h-35C-622.8,314.7-622.8,323-622.8,323z"\/>$/;"	i
DejaVuSans-37_00000152961216771672232250000008265703360759850118_	figures/combined-sparsity-plots.svg	/^							l24.9,64.6h-35C-718.2,314.7-718.2,323-718.2,323z"\/>$/;"	i
DejaVuSans-37_00000178188594659056096010000011459662915251781519_	figures/combined-sparsity-plots.svg	/^							l24.9,64.6h-35C-654.5,314.7-654.5,323-654.5,323z"\/>$/;"	i
DejaVuSans-38_00000044141076458275346430000002772508328070575536_	figures/combined-sparsity-plots.svg	/^						c-2.4,2.1-5.7,3.2-9.9,3.2c-4.3,0-7.6-1.1-9.9-3.2C-673.8,377.3-675,374.4-675,370.6z"\/>$/;"	i
DejaVuSans-38_00000124145071182309644020000000424311744059340197_	figures/combined-sparsity-plots.svg	/^							c-2.4,2.1-5.7,3.2-9.9,3.2c-4.3,0-7.6-1.1-9.9-3.2C-611.5,311.3-612.6,308.3-612.6,304.5z"\//;"	i
DejaVuSans-38_00000176746058408764358230000012333067157242434746_	figures/combined-sparsity-plots.svg	/^							c-2.4,2.1-5.7,3.2-9.9,3.2c-4.3,0-7.6-1.1-9.9-3.2C-611.5,311.3-612.6,308.3-612.6,304.5z"\//;"	i
DejaVuSans-39_00000086661176191799151060000015804224281083981441_	figures/combined-sparsity-plots.svg	/^							c-2.6-3-3.9-7.2-3.9-12.4c0-5.3,1.3-9.4,3.9-12.5C-608.3,284.1-604.8,282.6-600.4,282.6z"\/>$/;"	i
DejaVuSans-39_00000111886028244447090950000007496930105993710508_	figures/combined-sparsity-plots.svg	/^						s-3.9-7.2-3.9-12.4c0-5.3,1.3-9.4,3.9-12.5C-670.6,350.1-667.1,348.6-662.7,348.6z"\/>$/;"	i
DejaVuSans-39_00000150084862920850444740000009676169584462610098_	figures/combined-sparsity-plots.svg	/^							c-2.6-3-3.9-7.2-3.9-12.4c0-5.3,1.3-9.4,3.9-12.5C-608.3,284.1-604.8,282.6-600.4,282.6z"\/>$/;"	i
DejaVuSans-61_00000003088098218455022670000008910649034093817771_	figures/combined-sparsity-plots.svg	/^						C-223.1,361.9-221.2,355.7-221.2,347.4z"\/>$/;"	i
DejaVuSans-61_00000005245697966058948990000015272317863068991365_	figures/combined-sparsity-plots.svg	/^						C-286.8,361.9-284.8,355.7-284.8,347.4z"\/>$/;"	i
DejaVuSans-61_00000007398745779953039660000017774702840810752447_	figures/combined-sparsity-plots.svg	/^						C82.9,361.9,84.9,355.7,84.9,347.4z"\/>$/;"	i
DejaVuSans-61_00000019644335602443282650000014330476669073784493_	figures/combined-sparsity-plots.svg	/^						"\/>$/;"	i
DejaVuSans-61_00000027581269217486608370000010006441697446388357_	figures/combined-sparsity-plots.svg	/^						C82.9,361.9,84.9,355.7,84.9,347.4z"\/>$/;"	i
DejaVuSans-61_00000029756137557133960850000016731789863062026919_	figures/combined-sparsity-plots.svg	/^						C1264.5,772.1,1266.4,765.9,1266.4,757.6z"\/>$/;"	i
DejaVuSans-61_00000034081617620539037060000018076553697082511273_	figures/combined-sparsity-plots.svg	/^						C-325.5,361.9-323.6,355.7-323.6,347.4z"\/>$/;"	i
DejaVuSans-61_00000034768058515794006470000008202648497057171842_	figures/combined-sparsity-plots.svg	/^						C-223.1,361.9-221.2,355.7-221.2,347.4z"\/>$/;"	i
DejaVuSans-61_00000043417579826375087380000007472414269613692851_	figures/combined-sparsity-plots.svg	/^						C82.9,361.9,84.9,355.7,84.9,347.4z"\/>$/;"	i
DejaVuSans-61_00000050650909443947314980000003576303340708072362_	figures/combined-sparsity-plots.svg	/^						c3.3,1.3,6.5,2.2,9.6,2.8c3.1,0.6,6.1,1,9,1c7.9,0,13.8-2.1,17.7-6.2C82.9,361.9,84.9,355.7,8/;"	i
DejaVuSans-61_00000053536660391011753470000011017599325847457153_	figures/combined-sparsity-plots.svg	/^						C-506.5,295.9-504.5,289.7-504.5,281.3z"\/>$/;"	i
DejaVuSans-61_00000057830913082622476230000005815480681914965638_	figures/combined-sparsity-plots.svg	/^						C-223.1,361.9-221.2,355.7-221.2,347.4z"\/>$/;"	i
DejaVuSans-61_00000064347242675638335430000008471070350895331229_	figures/combined-sparsity-plots.svg	/^						C-325.5,361.9-323.6,355.7-323.6,347.4z"\/>$/;"	i
DejaVuSans-61_00000077301648691714752250000009485516658175916701_	figures/combined-sparsity-plots.svg	/^						c3.3,1.3,6.5,2.2,9.6,2.8c3.1,0.6,6.1,1,9,1c7.9,0,13.8-2.1,17.7-6.2C-325.5,361.9-323.6,355./;"	i
DejaVuSans-61_00000078013155419774626280000004774462426506249149_	figures/combined-sparsity-plots.svg	/^						C-223.1,361.9-221.2,355.7-221.2,347.4z"\/>$/;"	i
DejaVuSans-61_00000088830821749822110310000004950331184356921260_	figures/combined-sparsity-plots.svg	/^						"\/>$/;"	i
DejaVuSans-61_00000095336757836002026140000005547933000482806960_	figures/combined-sparsity-plots.svg	/^						C1244.1,772.1,1246.1,765.9,1246.1,757.6z"\/>$/;"	i
DejaVuSans-61_00000101799622126062470780000004940497867584374707_	figures/combined-sparsity-plots.svg	/^						C-325.5,361.9-323.6,355.7-323.6,347.4z"\/>$/;"	i
DejaVuSans-61_00000103944757660393304440000003774189810847647410_	figures/combined-sparsity-plots.svg	/^						C-509-4455.8-507.1-4462-507.1-4470.4z"\/>$/;"	i
DejaVuSans-61_00000103972476906650908220000017343063227963225008_	figures/combined-sparsity-plots.svg	/^						c3.3,1.3,6.5,2.2,9.6,2.8c3.1,0.6,6.1,1,9,1c7.9,0,13.8-2.1,17.7-6.2C82.9,361.9,84.9,355.7,8/;"	i
DejaVuSans-61_00000104705458285844225290000006045483218919708589_	figures/combined-sparsity-plots.svg	/^						"\/>$/;"	i
DejaVuSans-61_00000106123091249634631620000009925410721925386921_	figures/combined-sparsity-plots.svg	/^						c3.3,1.3,6.5,2.2,9.6,2.8c3.1,0.6,6.1,1,9,1c7.9,0,13.8-2.1,17.7-6.2C82.9,361.9,84.9,355.7,8/;"	i
DejaVuSans-61_00000106133355655728473210000014655536361694713236_	figures/combined-sparsity-plots.svg	/^						C430.5,385.9,432.4,379.7,432.4,371.3z"\/>$/;"	i
DejaVuSans-61_00000107552941993080436190000004614100548531939518_	figures/combined-sparsity-plots.svg	/^						c3.3,1.3,6.5,2.2,9.6,2.8c3.1,0.6,6.1,1,9,1c7.9,0,13.8-2.1,17.7-6.2C-325.5,361.9-323.6,355./;"	i
DejaVuSans-61_00000109721698104531609170000011846543194557130167_	figures/combined-sparsity-plots.svg	/^						C82.9,361.9,84.9,355.7,84.9,347.4z"\/>$/;"	i
DejaVuSans-61_00000110457883971526473090000007000253481407145116_	figures/combined-sparsity-plots.svg	/^						C-506.5,295.9-504.5,289.7-504.5,281.3z"\/>$/;"	i
DejaVuSans-61_00000121963726269508695870000002057721377862206088_	figures/combined-sparsity-plots.svg	/^						C82.9,361.9,84.9,355.7,84.9,347.4z"\/>$/;"	i
DejaVuSans-61_00000125597589920679196340000004875925943266026641_	figures/combined-sparsity-plots.svg	/^						C82.9,361.9,84.9,355.7,84.9,347.4z"\/>$/;"	i
DejaVuSans-61_00000127728696156856267070000018431991905705401991_	figures/combined-sparsity-plots.svg	/^						C-223.1,361.9-221.2,355.7-221.2,347.4z"\/>$/;"	i
DejaVuSans-61_00000133500980740670378920000007926148694027442053_	figures/combined-sparsity-plots.svg	/^						C-389.2,361.9-387.2,355.7-387.2,347.4z"\/>$/;"	i
DejaVuSans-61_00000135662238430320849050000016760133616858862526_	figures/combined-sparsity-plots.svg	/^						C1692.2,772.1,1694.2,765.9,1694.2,757.6z"\/>$/;"	i
DejaVuSans-61_00000140724068409323905450000003311984379303172001_	figures/combined-sparsity-plots.svg	/^						v8.3c3.3,1.3,6.5,2.2,9.6,2.8c3.1,0.6,6.1,1,9,1c7.9,0,13.8-2.1,17.7-6.2C19.3,361.9,21.2,355/;"	i
DejaVuSans-61_00000145749591736430589650000009544588374307587252_	figures/combined-sparsity-plots.svg	/^						c3.3,1.3,6.5,2.2,9.6,2.8c3.1,0.6,6.1,1,9,1c7.9,0,13.8-2.1,17.7-6.2C423-4452.4,425-4458.6,4/;"	i
DejaVuSans-61_00000149366431323579443820000002251964331773899944_	figures/combined-sparsity-plots.svg	/^						C-223.1,361.9-221.2,355.7-221.2,347.4z"\/>$/;"	i
DejaVuSans-61_00000152230682351673482030000012561513865097715608_	figures/combined-sparsity-plots.svg	/^						C-223.1,361.9-221.2,355.7-221.2,347.4z"\/>$/;"	i
DejaVuSans-61_00000157277929325721098880000007621852458816824511_	figures/combined-sparsity-plots.svg	/^					C-505.2,2338.6-503.2,2332.4-503.2,2324z"\/>$/;"	i
DejaVuSans-61_00000158722964420037708670000006193033170946130312_	figures/combined-sparsity-plots.svg	/^						C-223.1,361.9-221.2,355.7-221.2,347.4z"\/>$/;"	i
DejaVuSans-61_00000161623285949154907340000005504443011310664088_	figures/combined-sparsity-plots.svg	/^						C-325.5,361.9-323.6,355.7-323.6,347.4z"\/>$/;"	i
DejaVuSans-61_00000165954118508661677680000003485482802332946876_	figures/combined-sparsity-plots.svg	/^						C-325.5,361.9-323.6,355.7-323.6,347.4z"\/>$/;"	i
DejaVuSans-61_00000166654765712488392580000015072212008869741234_	figures/combined-sparsity-plots.svg	/^						C-223.1,361.9-221.2,355.7-221.2,347.4z"\/>$/;"	i
DejaVuSans-61_00000173875492065788443920000004237402246450418610_	figures/combined-sparsity-plots.svg	/^						C-325.5,361.9-323.6,355.7-323.6,347.4z"\/>$/;"	i
DejaVuSans-61_00000174575849516897680350000003436502946699295367_	figures/combined-sparsity-plots.svg	/^						c3.3,1.3,6.5,2.2,9.6,2.8c3.1,0.6,6.1,1,9,1c7.9,0,13.8-2.1,17.7-6.2C-325.5,361.9-323.6,355./;"	i
DejaVuSans-61_00000175284328411305157050000000993801770405210558_	figures/combined-sparsity-plots.svg	/^						C-210.6-4452.4-208.7-4458.6-208.7-4466.9z"\/>$/;"	i
DejaVuSans-61_00000178885467541141788250000014001742342058911620_	figures/combined-sparsity-plots.svg	/^						C-203.2,385.9-201.2,379.7-201.2,371.3z"\/>$/;"	i
DejaVuSans-63	figures/combined-sparsity-plots.svg	/^						c4.9,5.1,11.6,7.7,20.2,7.7c2.8,0,5.5-0.3,8.1-0.9C-690.1-4443.6-687.5-4444.4-685.1-4445.6z"/;"	i
DejaVuSans-63_00000021840405307615247630000004052895575486629761_	figures/combined-sparsity-plots.svg	/^						C-682.6,394.7-680.1,393.9-677.6,392.7z"\/>$/;"	i
DejaVuSans-63_00000039128967022680778700000018422745001940794803_	figures/combined-sparsity-plots.svg	/^						c0,8.9,2.4,15.9,7.3,21s11.6,7.7,20.2,7.7c2.8,0,5.5-0.3,8.1-0.9C1298.9,780.9,1301.5,780.1,1/;"	i
DejaVuSans-63_00000111885669033053894650000013611857286315156920_	figures/combined-sparsity-plots.svg	/^						c0,8.9,2.4,15.9,7.3,21s11.6,7.7,20.2,7.7c2.8,0,5.5-0.3,8.1-0.9C1747,780.9,1749.6,780.1,175/;"	i
DejaVuSans-63_00000119840593978600375410000003324657475145245348_	figures/combined-sparsity-plots.svg	/^						"\/>$/;"	i
DejaVuSans-63_00000131330499636012805560000011279128883434561720_	figures/combined-sparsity-plots.svg	/^						c0,8.9,2.4,15.9,7.3,21s11.6,7.7,20.2,7.7c2.8,0,5.5-0.3,8.1-0.9C355.2,780.9,357.7,780.1,360/;"	i
DejaVuSans-64	figures/combined-sparsity-plots.svg	/^						c2.7,3.8,4.1,8.9,4.1,15.5s-1.4,11.8-4.1,15.5c-2.7,3.8-6.5,5.6-11.2,5.6s-8.5-1.9-11.2-5.6S-/;"	i
DejaVuSans-64_00000070111146531870538970000001223939831803681431_	figures/combined-sparsity-plots.svg	/^						s-8.5-1.9-11.2-5.6C131.5,379.2,130.1,374,130.1,367.4z"\/>$/;"	i
DejaVuSans-64_00000111871033305681206900000005121151834899241397_	figures/combined-sparsity-plots.svg	/^						s-8.5-1.9-11.2-5.6C-176,379.2-177.3,374-177.3,367.4z"\/>$/;"	i
DejaVuSans-64_00000152946954947012686480000002825273800874319771_	figures/combined-sparsity-plots.svg	/^						C124.1-4459.1,122.7-4464.3,122.7-4470.9z"\/>$/;"	i
DejaVuSans-65_00000002364342036286581810000003755892601116726678_	figures/combined-sparsity-plots.svg	/^						c-0.1,4.9-1.4,8.8-4.1,11.8c-2.7,2.9-6.2,4.4-10.7,4.4c-5,0-9-1.4-12-4.2s-4.7-6.8-5.2-12H514/;"	i
DejaVuSans-65_00000002376552440720060880000003530861241206960777_	figures/combined-sparsity-plots.svg	/^						c-2.7,2.9-6.2,4.4-10.7,4.4c-5,0-9-1.4-12-4.2c-3-2.8-4.7-6.8-5.2-12L-612.2,282.4z"\/>$/;"	i
DejaVuSans-65_00000019660224490483824540000008521336139364850587_	figures/combined-sparsity-plots.svg	/^						c-0.1,4.9-1.4,8.8-4.1,11.8c-2.7,2.9-6.2,4.4-10.7,4.4c-5,0-9-1.4-12-4.2s-4.7-6.8-5.2-12H694/;"	i
DejaVuSans-65_00000023278286718682776670000013408818994322659227_	figures/combined-sparsity-plots.svg	/^						c-2.7,2.9-6.2,4.4-10.7,4.4c-5,0-9-1.4-12-4.2c-3-2.8-4.7-6.8-5.2-12L-612.2,282.4z"\/>$/;"	i
DejaVuSans-65_00000035513824341204672670000009990070859570955931_	figures/combined-sparsity-plots.svg	/^						c-2.7,2.9-6.2,4.4-10.7,4.4c-5,0-9-1.4-12-4.2c-3-2.8-4.7-6.8-5.2-12L93.6-4465.9z"\/>$/;"	i
DejaVuSans-65_00000036244276636410962150000005739876414969376400_	figures/combined-sparsity-plots.svg	/^						c-2.7,2.9-6.2,4.4-10.7,4.4c-5,0-9-1.4-12-4.2c-3-2.8-4.7-6.8-5.2-12L-614.7-4469.3z"\/>$/;"	i
DejaVuSans-65_00000044175721880002566410000002573843905378954417_	figures/combined-sparsity-plots.svg	/^						c-0.1,4.9-1.4,8.8-4.1,11.8c-2.7,2.9-6.2,4.4-10.7,4.4c-5,0-9-1.4-12-4.2c-3-2.8-4.7-6.8-5.2-/;"	i
DejaVuSans-65_00000052097126113535231460000013798717652823967675_	figures/combined-sparsity-plots.svg	/^						c-2.7,2.9-6.2,4.4-10.7,4.4c-5,0-9-1.4-12-4.2c-3-2.8-4.7-6.8-5.2-12L101,372.4z"\/>$/;"	i
DejaVuSans-65_00000129891722561064296150000012526022033735401623_	figures/combined-sparsity-plots.svg	/^						c-0.1,4.9-1.4,8.8-4.1,11.8c-2.7,2.9-6.2,4.4-10.7,4.4c-5,0-9-1.4-12-4.2c-3-2.8-4.7-6.8-5.2-/;"	i
DejaVuSans-65_00000130629865924359300940000012059258571959807144_	figures/combined-sparsity-plots.svg	/^						c-0.1,4.9-1.4,8.8-4.1,11.8c-2.7,2.9-6.2,4.4-10.7,4.4c-5,0-9-1.4-12-4.2c-3-2.8-4.7-6.8-5.2-/;"	i
DejaVuSans-65_00000152978407523456328720000011235711007672245404_	figures/combined-sparsity-plots.svg	/^					c-0.1,4.9-1.4,8.8-4.1,11.8c-2.7,2.9-6.2,4.4-10.7,4.4c-5,0-9-1.4-12-4.2c-3-2.8-4.7-6.8-5.2-1/;"	i
DejaVuSans-65_00000177461347844922341830000000537029944333542817_	figures/combined-sparsity-plots.svg	/^						c-0.1,4.9-1.4,8.8-4.1,11.8c-2.7,2.9-6.2,4.4-10.7,4.4c-5,0-9-1.4-12-4.2c-3-2.8-4.7-6.8-5.2-/;"	i
DejaVuSans-66_00000067205748937063601490000014525321109900286358_	figures/combined-sparsity-plots.svg	/^						c2.8,2.8,7.3,4.2,13.5,4.2H1154.7z"\/>$/;"	i
DejaVuSans-66_00000140722866940747810960000018376630254508589731_	figures/combined-sparsity-plots.svg	/^						c2.8,2.8,7.3,4.2,13.5,4.2H1602.8z"\/>$/;"	i
DejaVuSans-66_00000182501598948549042420000017287076624998579646_	figures/combined-sparsity-plots.svg	/^						s-1.9-3.6-1.9-7v-4.8H376v-7h-14.8v-47.7h-9v47.7h-8.6v7h8.6v3.8c0,6.1,1.4,10.5,4.2,13.3c2.8/;"	i
DejaVuSans-69_00000000212292077404136740000003296623501693662603_	figures/combined-sparsity-plots.svg	/^						h9v-11.4h-9V392.2z"\/>$/;"	i
DejaVuSans-69_00000011007785449827693560000008728908868147565184_	figures/combined-sparsity-plots.svg	/^						 M212.5-4422.2h9v-11.4h-9V-4422.2z"\/>$/;"	i
DejaVuSans-69_00000011012422754658627960000009482086715915780226_	figures/combined-sparsity-plots.svg	/^					 M-715.6,2368.8h9v-11.4h-9V2368.8z"\/>$/;"	i
DejaVuSans-69_00000017475593068853651640000004271035711565063830_	figures/combined-sparsity-plots.svg	/^						 M1378.1,802.4h9V791h-9V802.4z"\/>$/;"	i
DejaVuSans-69_00000035489139319314070870000002613664939327930003_	figures/combined-sparsity-plots.svg	/^						h9V791h-9V802.4z"\/>$/;"	i
DejaVuSans-69_00000039110790074834992520000007637058010375692443_	figures/combined-sparsity-plots.svg	/^						h9v-11.4h-9V392.2z"\/>$/;"	i
DejaVuSans-69_00000054266372354518777230000001502402119470128801_	figures/combined-sparsity-plots.svg	/^						h9v-11.4h-9V392.2z"\/>$/;"	i
DejaVuSans-69_00000058570003811540608160000003523150927352467362_	figures/combined-sparsity-plots.svg	/^						h9v-11.4h-9V392.2z"\/>$/;"	i
DejaVuSans-69_00000077300852593293972850000017618619539767942281_	figures/combined-sparsity-plots.svg	/^						V791h-9V802.4z"\/>$/;"	i
DejaVuSans-69_00000082369625631037273250000003768672064156350608_	figures/combined-sparsity-plots.svg	/^						 M1806.9,802.4h9V791h-9V802.4z"\/>$/;"	i
DejaVuSans-69_00000085246304805571728370000013189823152355460999_	figures/combined-sparsity-plots.svg	/^						 M-449.4-4425.6h9v-11.4h-9V-4425.6z"\/>$/;"	i
DejaVuSans-69_00000085969454303515389990000010033151607514032800_	figures/combined-sparsity-plots.svg	/^						v-11.4h-9V392.2z"\/>$/;"	i
DejaVuSans-69_00000088851677267015374980000003805280754308672694_	figures/combined-sparsity-plots.svg	/^						h9v-11.4h-9V392.2z"\/>$/;"	i
DejaVuSans-69_00000092450895270812228230000008112514836703311028_	figures/combined-sparsity-plots.svg	/^						v-11.4h-9V416.1z"\/>$/;"	i
DejaVuSans-69_00000100360291796619707520000015751012599607329696_	figures/combined-sparsity-plots.svg	/^						 M-446.8,326.1h9v-11.4h-9V326.1z"\/>$/;"	i
DejaVuSans-69_00000106840929572395628100000015240727358461796004_	figures/combined-sparsity-plots.svg	/^						 M-716.9,326.1h9v-11.4h-9V326.1z"\/>$/;"	i
DejaVuSans-69_00000107570780199477079730000007198942274308881561_	figures/combined-sparsity-plots.svg	/^						h9v-11.4h-9V416.1z"\/>$/;"	i
DejaVuSans-69_00000112622305636048990100000006945655808266445455_	figures/combined-sparsity-plots.svg	/^						 M-716.9,326.1h9v-11.4h-9V326.1z"\/>$/;"	i
DejaVuSans-69_00000123433947746333501500000009290301403874219652_	figures/combined-sparsity-plots.svg	/^						 M-719.5-4425.6h9v-11.4h-9V-4425.6z"\/>$/;"	i
DejaVuSans-69_00000126314262102673530780000015056746408572612517_	figures/combined-sparsity-plots.svg	/^						h9v-11.4h-9V392.2z"\/>$/;"	i
DejaVuSans-69_00000132787116427420657090000009752410067266584235_	figures/combined-sparsity-plots.svg	/^					 M-445.5,2368.8h9v-11.4h-9V2368.8z"\/>$/;"	i
DejaVuSans-69_00000136398192463510692880000009866485580967978930_	figures/combined-sparsity-plots.svg	/^						 M482.7-4422.2h9v-11.4h-9V-4422.2z"\/>$/;"	i
DejaVuSans-69_00000137132052091835585320000012782015439341018517_	figures/combined-sparsity-plots.svg	/^						h9v-11.4h-9V392.2z"\/>$/;"	i
DejaVuSans-69_00000139973237614925476650000017198311290435068588_	figures/combined-sparsity-plots.svg	/^						 M-446.8,326.1h9v-11.4h-9V326.1z"\/>$/;"	i
DejaVuSans-69_00000146500751508014178990000005582178652686644353_	figures/combined-sparsity-plots.svg	/^						V791h-9V802.4z"\/>$/;"	i
DejaVuSans-69_00000147930108589209496990000008422725271182705543_	figures/combined-sparsity-plots.svg	/^						 M1358.8,802.4h9V791h-9V802.4z"\/>$/;"	i
DejaVuSans-69_00000163789919597419546070000016590453526855154823_	figures/combined-sparsity-plots.svg	/^						h9v-11.4h-9V392.2z"\/>$/;"	i
DejaVuSans-69_00000167360583120298735380000014811095244138049680_	figures/combined-sparsity-plots.svg	/^						h9v-11.4h-9V392.2z"\/>$/;"	i
DejaVuSans-69_00000168089591551838442080000000568745099852610988_	figures/combined-sparsity-plots.svg	/^						V791h-9V802.4z"\/>$/;"	i
DejaVuSans-69_00000172402105773442588860000016634130081982793649_	figures/combined-sparsity-plots.svg	/^						h9V791h-9V802.4z"\/>$/;"	i
DejaVuSans-6a	figures/combined-sparsity-plots.svg	/^						c3.4,0,5.7,0.8,7,2.4c1.2,1.6,1.9,4.8,1.9,9.8L-126.7-4443.5L-126.7-4443.5z M-126.7-4422.2h9/;"	i
DejaVuSans-6a_00000021798597950040972420000008143159713133196721_	figures/combined-sparsity-plots.svg	/^						V416.1z"\/>$/;"	i
DejaVuSans-6c_00000083061741829091720590000002003721035842813861_	figures/combined-sparsity-plots.svg	/^					<path id="DejaVuSans-6c_00000083061741829091720590000002003721035842813861_" d="M349.6,802./;"	i
DejaVuSans-6c_00000088845877994391318870000010553798453971511433_	figures/combined-sparsity-plots.svg	/^					<path id="DejaVuSans-6c_00000088845877994391318870000010553798453971511433_" d="M-4488.7,80/;"	i
DejaVuSans-6c_00000096777702580003771080000009044701561531530684_	figures/combined-sparsity-plots.svg	/^					<path id="DejaVuSans-6c_00000096777702580003771080000009044701561531530684_" d="M385.9,802./;"	i
DejaVuSans-6c_00000097461343712641399290000004423277033857625475_	figures/combined-sparsity-plots.svg	/^					<path id="DejaVuSans-6c_00000097461343712641399290000004423277033857625475_" d="M359.6,802./;"	i
DejaVuSans-6c_00000106118477162987764280000011573405705311308971_	figures/combined-sparsity-plots.svg	/^					<path id="DejaVuSans-6c_00000106118477162987764280000011573405705311308971_" d="M-4492.1,80/;"	i
DejaVuSans-6d	figures/combined-sparsity-plots.svg	/^						c2.1,3.4,4.5,5.8,7.4,7.4s6.3,2.4,10.2,2.4c4,0,7.4-1,10.1-3C-569.1-4447.2-567-4450.1-565.7-/;"	i
DejaVuSans-6d_00000012449291823375728430000018392648328325476526_	figures/combined-sparsity-plots.svg	/^						C-163.5,367.2-161.4,364.2-160.1,360.4z"\/>$/;"	i
DejaVuSans-6d_00000027606817856563031760000007334743979136299184_	figures/combined-sparsity-plots.svg	/^						C-163.5,367.2-161.4,364.2-160.1,360.4z"\/>$/;"	i
DejaVuSans-6d_00000036215771755575107700000001203342479290377115_	figures/combined-sparsity-plots.svg	/^						C-163.5,367.2-161.4,364.2-160.1,360.4z"\/>$/;"	i
DejaVuSans-6d_00000038390507615791120050000012762888431628721324_	figures/combined-sparsity-plots.svg	/^						C-163.5,367.2-161.4,364.2-160.1,360.4z"\/>$/;"	i
DejaVuSans-6d_00000110458503471015737620000011798033582076853910_	figures/combined-sparsity-plots.svg	/^						C-163.5,367.2-161.4,364.2-160.1,360.4z"\/>$/;"	i
DejaVuSans-6d_00000111162375421228754730000005732519120434782876_	figures/combined-sparsity-plots.svg	/^						C-163.5,367.2-161.4,364.2-160.1,360.4z"\/>$/;"	i
DejaVuSans-6d_00000136406490189422214130000007755554261806445746_	figures/combined-sparsity-plots.svg	/^						C-227.1,367.2-225.1,364.2-223.7,360.4z"\/>$/;"	i
DejaVuSans-6d_00000137103426105635867580000001976662721412470192_	figures/combined-sparsity-plots.svg	/^						C-163.5,367.2-161.4,364.2-160.1,360.4z"\/>$/;"	i
DejaVuSans-6d_00000145031213520993920150000015834751618980488579_	figures/combined-sparsity-plots.svg	/^						s6.3,2.4,10.2,2.4c4,0,7.4-1,10.1-3C-561.6,391.1-559.5,388.2-558.2,384.3z"\/>$/;"	i
DejaVuSans-6d_00000145046310355782831900000007916288817048660129_	figures/combined-sparsity-plots.svg	/^						C-163.5,367.2-161.4,364.2-160.1,360.4z"\/>$/;"	i
DejaVuSans-6d_00000152266590478789689600000001155797964564012728_	figures/combined-sparsity-plots.svg	/^						C-163.5,367.2-161.4,364.2-160.1,360.4z"\/>$/;"	i
DejaVuSans-6d_00000178926323501941845540000001450761349809386392_	figures/combined-sparsity-plots.svg	/^						C789.5,777.3,791.5,774.4,792.9,770.6z"\/>$/;"	i
DejaVuSans-6e_00000012459299983987605790000017983975555657996687_	figures/combined-sparsity-plots.svg	/^						c2.9,1.6,6.3,2.4,10.1,2.4c6.3,0,11-1.9,14.2-5.8C615.5-4451.9,617.1-4457.6,617.1-4465.1z"\//;"	i
DejaVuSans-6e_00000016761974483029888830000016597333763489758909_	figures/combined-sparsity-plots.svg	/^					c2.9,1.6,6.3,2.4,10.1,2.4c6.3,0,11-1.9,14.2-5.8C-312.7,2339.1-311.1,2333.4-311.1,2325.9z"\//;"	i
DejaVuSans-6e_00000024705027071027393540000013331911476540146365_	figures/combined-sparsity-plots.svg	/^						c6.3,0,11-1.9,14.2-5.8C-316.6-4455.3-315-4461-315-4468.5z"\/>$/;"	i
DejaVuSans-6e_00000034779483616403140780000011740085586572582811_	figures/combined-sparsity-plots.svg	/^						c6.3,0,11-1.9,14.2-5.8C-314,296.4-312.4,290.7-312.4,283.2z"\/>$/;"	i
DejaVuSans-6e_00000098935571438709697010000006945856211538347403_	figures/combined-sparsity-plots.svg	/^						c2.9,1.6,6.3,2.4,10.1,2.4c6.3,0,11-1.9,14.2-5.8C1491.6,772.7,1493.2,766.9,1493.2,759.4z"\//;"	i
DejaVuSans-6e_00000137824280914140315630000011082709589617295513_	figures/combined-sparsity-plots.svg	/^						c2.9,1.6,6.3,2.4,10.1,2.4c6.3,0,11-1.9,14.2-5.8C582.5,772.7,584.1,766.9,584.1,759.4z"\/>$/;"	i
DejaVuSans-6e_00000141420002334978859560000004362018948376893375_	figures/combined-sparsity-plots.svg	/^						c2.9,1.6,6.3,2.4,10.1,2.4c6.3,0,11-1.9,14.2-5.8C623,386.4,624.6,380.7,624.6,373.2z"\/>$/;"	i
DejaVuSans-6e_00000165192411187435325880000009929295147327919279_	figures/combined-sparsity-plots.svg	/^						c2.9,1.6,6.3,2.4,10.1,2.4c6.3,0,11-1.9,14.2-5.8C331.2,772.7,332.8,766.9,332.8,759.4z"\/>$/;"	i
DejaVuSans-6e_00000168090771574405674560000003826428024163869061_	figures/combined-sparsity-plots.svg	/^						c2.9,1.6,6.3,2.4,10.1,2.4c6.3,0,11-1.9,14.2-5.8C1939.7,772.7,1941.3,766.9,1941.3,759.4z"\//;"	i
DejaVuSans-6e_00000181076130002068837060000015685083976327698585_	figures/combined-sparsity-plots.svg	/^						c6.3,0,11-1.9,14.2-5.8C-314,296.4-312.4,290.7-312.4,283.2z"\/>$/;"	i
DejaVuSans-6f_00000005258165862241688460000017709323571918432673_	figures/combined-sparsity-plots.svg	/^						C517.6-4444.7,523.8-4442.2,531.6-4442.2z"\/>$/;"	i
DejaVuSans-6f_00000023248356880207236400000007309232850522226860_	figures/combined-sparsity-plots.svg	/^						s-10.6-7.6-18.4-7.6s-14,2.5-18.4,7.6s-6.7,12.1-6.7,21.1s2.2,16,6.7,21.1C1841.9,779.8,1848,/;"	i
DejaVuSans-6f_00000027571299429567707220000009804017021928718769_	figures/combined-sparsity-plots.svg	/^						s-10.6-7.6-18.4-7.6s-14,2.5-18.4,7.6s-6.7,12.1-6.7,21.1s2.2,16,6.7,21.1C-4453.7,787.3-4447/;"	i
DejaVuSans-6f_00000030464589919675071000000011549988097008972177_	figures/combined-sparsity-plots.svg	/^						C394.5,779.8,400.7,782.4,408.5,782.4z"\/>$/;"	i
DejaVuSans-6f_00000048484425668361394820000013352434262404999082_	figures/combined-sparsity-plots.svg	/^						C-4457.2,782.4-4451,784.9-4443.2,784.9z"\/>$/;"	i
DejaVuSans-6f_00000062154202069492279300000017724992655008087741_	figures/combined-sparsity-plots.svg	/^						s-10.6-7.6-18.4-7.6c-7.8,0-14,2.5-18.4,7.6s-6.7,12.1-6.7,21.1s2.2,16,6.7,21.1C-662.2-4444./;"	i
DejaVuSans-6f_00000066474615774648977820000016890718775354620552_	figures/combined-sparsity-plots.svg	/^						C384.5,779.8,390.7,782.4,398.5,782.4z"\/>$/;"	i
DejaVuSans-6f_00000123435574096369265950000006832664022515147675_	figures/combined-sparsity-plots.svg	/^						C-411.9,303.6-405.7,306.1-397.9,306.1z"\/>$/;"	i
DejaVuSans-6f_00000128458317469581510690000010497890337043296388_	figures/combined-sparsity-plots.svg	/^						C-654.8,393.6-648.6,396.1-640.8,396.1z"\/>$/;"	i
DejaVuSans-6f_00000143601023804039611970000005357794626673553055_	figures/combined-sparsity-plots.svg	/^						s-10.6-7.6-18.4-7.6s-14,2.5-18.4,7.6s-6.7,12.1-6.7,21.1s2.2,16,6.7,21.1C1393.8,779.8,1399./;"	i
DejaVuSans-6f_00000150812234536557962860000016145169605907266432_	figures/combined-sparsity-plots.svg	/^						C-411.9,303.6-405.7,306.1-397.9,306.1z"\/>$/;"	i
DejaVuSans-6f_00000160184650537292426740000010373396115351553686_	figures/combined-sparsity-plots.svg	/^						C525.1,393.6,531.3,396.1,539.1,396.1z"\/>$/;"	i
DejaVuSans-6f_00000165928370828200316350000007665183680038666418_	figures/combined-sparsity-plots.svg	/^						s2.2,16,6.7,21.1C-414.4-4448.1-408.3-4445.6-400.4-4445.6z"\/>$/;"	i
DejaVuSans-6f_00000173123514796083717810000003732238629711985300_	figures/combined-sparsity-plots.svg	/^					C-410.6,2346.3-404.4,2348.8-396.6,2348.8z"\/>$/;"	i
DejaVuSans-70	figures/combined-sparsity-plots.svg	/^						s-4.1-8.9-4.1-15.5s1.4-11.8,4.1-15.5s6.5-5.6,11.2-5.6c4.8,0,8.5,1.9,11.2,5.6S-471.6-4477.5/;"	i
DejaVuSans-70_00000001651147620835435910000008624499507436512153_	figures/combined-sparsity-plots.svg	/^						S1199.4,747.1,1199.4,753.7z"\/>$/;"	i
DejaVuSans-70_00000008834526929764092430000012002590878450861744_	figures/combined-sparsity-plots.svg	/^						S17.9,336.9,17.9,343.5z"\/>$/;"	i
DejaVuSans-70_00000018215495147448805310000003183981447916408704_	figures/combined-sparsity-plots.svg	/^						S-390.6,336.9-390.6,343.5z"\/>$/;"	i
DejaVuSans-70_00000018953724405842745010000010415501370041894331_	figures/combined-sparsity-plots.svg	/^						c4.8,0,8.5,1.9,11.2,5.6S17.9,336.9,17.9,343.5z"\/>$/;"	i
DejaVuSans-70_00000022561009881269241980000008020930156836818069_	figures/combined-sparsity-plots.svg	/^						c4.8,0,8.5,1.9,11.2,5.6S17.9,336.9,17.9,343.5z"\/>$/;"	i
DejaVuSans-70_00000036218710044153237820000001663774782189208734_	figures/combined-sparsity-plots.svg	/^						c4.8,0,8.5,1.9,11.2,5.6S17.9,336.9,17.9,343.5z"\/>$/;"	i
DejaVuSans-70_00000047746231751364622430000011668685641116273836_	figures/combined-sparsity-plots.svg	/^						S-390.6,336.9-390.6,343.5z"\/>$/;"	i
DejaVuSans-70_00000059269056078531633010000007162647206510078338_	figures/combined-sparsity-plots.svg	/^						c4.8,0,8.5,1.9,11.2,5.6S-390.6,336.9-390.6,343.5z"\/>$/;"	i
DejaVuSans-70_00000065037416616584257960000016598266372129225631_	figures/combined-sparsity-plots.svg	/^						S-390.6,336.9-390.6,343.5z"\/>$/;"	i
DejaVuSans-70_00000067956295333441821320000014247289327311967622_	figures/combined-sparsity-plots.svg	/^						c4.8,0,8.5,1.9,11.2,5.6S-454.2,336.9-454.2,343.5z"\/>$/;"	i
DejaVuSans-70_00000088816298904582807780000014595488193423121589_	figures/combined-sparsity-plots.svg	/^						S17.9,336.9,17.9,343.5z"\/>$/;"	i
DejaVuSans-70_00000089552454984559137170000002905121383133801101_	figures/combined-sparsity-plots.svg	/^						c4.8,0,8.5,1.9,11.2,5.6C-465.5,355.7-464.1,360.8-464.1,367.4z"\/>$/;"	i
DejaVuSans-70_00000089562585549875080260000000975955189263921320_	figures/combined-sparsity-plots.svg	/^						S17.9,336.9,17.9,343.5z"\/>$/;"	i
DejaVuSans-70_00000090259658480759034030000003498071056817813133_	figures/combined-sparsity-plots.svg	/^						S751.3,747.1,751.3,753.7z"\/>$/;"	i
DejaVuSans-70_00000102513964120815839220000013811755727826669207_	figures/combined-sparsity-plots.svg	/^						c4.8,0,8.5,1.9,11.2,5.6C-391.9,331.7-390.6,336.9-390.6,343.5z"\/>$/;"	i
DejaVuSans-70_00000102537576337413426810000010134904663372578981_	figures/combined-sparsity-plots.svg	/^						c4.8,0,8.5,1.9,11.2,5.6C-391.9,331.7-390.6,336.9-390.6,343.5z"\/>$/;"	i
DejaVuSans-70_00000111905732244390618580000016384813225098157714_	figures/combined-sparsity-plots.svg	/^						c4.8,0,8.5,1.9,11.2,5.6C-47.1,331.7-45.7,336.9-45.7,343.5z"\/>$/;"	i
DejaVuSans-70_00000127729987903304287360000014583841766681785501_	figures/combined-sparsity-plots.svg	/^						c4.8,0,8.5,1.9,11.2,5.6C-391.9,331.7-390.6,336.9-390.6,343.5z"\/>$/;"	i
DejaVuSans-70_00000140715629700653350370000012947502246961584310_	figures/combined-sparsity-plots.svg	/^						c4.8,0,8.5,1.9,11.2,5.6S17.9,336.9,17.9,343.5z"\/>$/;"	i
DejaVuSans-70_00000142890815397927334720000000096489437703284609_	figures/combined-sparsity-plots.svg	/^						c4.8,0,8.5,1.9,11.2,5.6S17.9,336.9,17.9,343.5z"\/>$/;"	i
DejaVuSans-70_00000151504991625723964540000007947420428560938923_	figures/combined-sparsity-plots.svg	/^						c4.8,0,8.5,1.9,11.2,5.6S-390.6,336.9-390.6,343.5z"\/>$/;"	i
DejaVuSans-70_00000160875023155443237610000002269674391604161963_	figures/combined-sparsity-plots.svg	/^						c4.8,0,8.5,1.9,11.2,5.6S17.9,336.9,17.9,343.5z"\/>$/;"	i
DejaVuSans-70_00000163771813912239684070000017389703414818779804_	figures/combined-sparsity-plots.svg	/^						c4.8,0,8.5,1.9,11.2,5.6C-391.9,331.7-390.6,336.9-390.6,343.5z"\/>$/;"	i
DejaVuSans-72_00000003788028163734500770000007081409972955919492_	figures/combined-sparsity-plots.svg	/^						c0.6,0,1.3,0,2-0.1c0.8-0.1,1.6-0.2,2.5-0.4L-273.4,362.5z"\/>$/;"	i
DejaVuSans-72_00000008116431949631970010000003866229257176616894_	figures/combined-sparsity-plots.svg	/^						c0.6,0,1.3,0,2-0.1c0.8-0.1,1.6-0.2,2.5-0.4L-273.4,362.5z"\/>$/;"	i
DejaVuSans-72_00000013904241335015651850000012654151457739225530_	figures/combined-sparsity-plots.svg	/^						c0.6,0,1.3,0,2-0.1c0.8-0.1,1.6-0.2,2.5-0.4L135.1,362.5z"\/>$/;"	i
DejaVuSans-72_00000018220483621281011890000009843214359925071263_	figures/combined-sparsity-plots.svg	/^					c3,1.6,6.7,2.4,11,2.4c0.6,0,1.3,0,2-0.1c0.8-0.1,1.6-0.2,2.5-0.4L-555.4,2339.1z"\/>$/;"	i
DejaVuSans-72_00000020360700904362569970000015481430402560154017_	figures/combined-sparsity-plots.svg	/^						c0.6,0,1.3,0,2-0.1c0.8-0.1,1.6-0.2,2.5-0.4L-273.4,362.5z"\/>$/;"	i
DejaVuSans-72_00000021804588742511142000000009543159030746562454_	figures/combined-sparsity-plots.svg	/^						c0.6,0,1.3,0,2-0.1c0.8-0.1,1.6-0.2,2.5-0.4L868.5,772.7z"\/>$/;"	i
DejaVuSans-72_00000026874170401068485760000017022964108902529442_	figures/combined-sparsity-plots.svg	/^						c3,1.6,6.7,2.4,11,2.4c0.6,0,1.3,0,2-0.1c0.8-0.1,1.6-0.2,2.5-0.4L1316.6,772.7z"\/>$/;"	i
DejaVuSans-72_00000027577108030864573240000010234399229174796421_	figures/combined-sparsity-plots.svg	/^						c0.6,0,1.3,0,2-0.1c0.8-0.1,1.6-0.2,2.5-0.4L-273.4,362.5z"\/>$/;"	i
DejaVuSans-72_00000031181411631626258430000007667787363181346962_	figures/combined-sparsity-plots.svg	/^						c0.6,0,1.3,0,2-0.1c0.8-0.1,1.6-0.2,2.5-0.4L-556.7,296.4z"\/>$/;"	i
DejaVuSans-72_00000034768141510517673980000014674469012624407194_	figures/combined-sparsity-plots.svg	/^						c0.6,0,1.3,0,2-0.1c0.8-0.1,1.6-0.2,2.5-0.4L-273.4,362.5z"\/>$/;"	i
DejaVuSans-72_00000063602030451075210380000016750433985044947112_	figures/combined-sparsity-plots.svg	/^						c0.6,0,1.3,0,2-0.1c0.8-0.1,1.6-0.2,2.5-0.4L380.2,386.4z"\/>$/;"	i
DejaVuSans-72_00000068677919546692065180000010522839987529358728_	figures/combined-sparsity-plots.svg	/^						c0.6,0,1.3,0,2-0.1c0.8-0.1,1.6-0.2,2.5-0.4L135.1,362.5z"\/>$/;"	i
DejaVuSans-72_00000070839349455691210870000004173705399224163507_	figures/combined-sparsity-plots.svg	/^						c0.6,0,1.3,0,2-0.1c0.8-0.1,1.6-0.2,2.5-0.4L135.1,362.5z"\/>$/;"	i
DejaVuSans-72_00000072261176204470486310000011989981683382932885_	figures/combined-sparsity-plots.svg	/^						c0.6,0,1.3,0,2-0.1c0.8-0.1,1.6-0.2,2.5-0.4L-273.4,362.5z"\/>$/;"	i
DejaVuSans-72_00000078750624729257213550000002699597066312268938_	figures/combined-sparsity-plots.svg	/^						c0.6,0,1.3,0,2-0.1c0.8-0.1,1.6-0.2,2.5-0.4L-556.7,296.4z"\/>$/;"	i
DejaVuSans-72_00000082356138151053509100000002716810940090096260_	figures/combined-sparsity-plots.svg	/^						c0.6,0,1.3,0,2-0.1c0.8-0.1,1.6-0.2,2.5-0.4L135.1,362.5z"\/>$/;"	i
DejaVuSans-72_00000083080387941825957130000014077304453764464542_	figures/combined-sparsity-plots.svg	/^						c0.6,0,1.3,0,2-0.1c0.8-0.1,1.6-0.2,2.5-0.4L372.8-4451.9z"\/>$/;"	i
DejaVuSans-72_00000088836431125165000530000007179729537807754913_	figures/combined-sparsity-plots.svg	/^						c0.6,0,1.3,0,2-0.1c0.8-0.1,1.6-0.2,2.5-0.4L135.1,362.5z"\/>$/;"	i
DejaVuSans-72_00000095318597246216164790000017521118946077123236_	figures/combined-sparsity-plots.svg	/^						c0.6,0,1.3,0,2-0.1c0.8-0.1,1.6-0.2,2.5-0.4L-559.3-4455.3z"\/>$/;"	i
DejaVuSans-72_00000101081941023333968670000001118094349846679182_	figures/combined-sparsity-plots.svg	/^						c0.6,0,1.3,0,2-0.1c0.8-0.1,1.6-0.2,2.5-0.4L135.1,362.5z"\/>$/;"	i
DejaVuSans-72_00000113330786563309666840000001995257594958331282_	figures/combined-sparsity-plots.svg	/^						c0.6,0,1.3,0,2-0.1c0.8-0.1,1.6-0.2,2.5-0.4L71.4,362.5z"\/>$/;"	i
DejaVuSans-72_00000121970093520670384240000009962956245454672827_	figures/combined-sparsity-plots.svg	/^						c0.6,0,1.3,0,2-0.1c0.8-0.1,1.6-0.2,2.5-0.4L979.9,772.7z"\/>$/;"	i
DejaVuSans-72_00000132794590296616470230000011971860901207505556_	figures/combined-sparsity-plots.svg	/^						c0.6,0,1.3,0,2-0.1c0.8-0.1,1.6-0.2,2.5-0.4L-273.4,362.5z"\/>$/;"	i
DejaVuSans-72_00000156552506356148742980000016542544701056782209_	figures/combined-sparsity-plots.svg	/^						c3,1.6,6.7,2.4,11,2.4c0.6,0,1.3,0,2-0.1c0.8-0.1,1.6-0.2,2.5-0.4L1642,772.7z"\/>$/;"	i
DejaVuSans-72_00000161622657767540834170000012193393808431736204_	figures/combined-sparsity-plots.svg	/^						c0.6,0,1.3,0,2-0.1c0.8-0.1,1.6-0.2,2.5-0.4L135.1,362.5z"\/>$/;"	i
DejaVuSans-72_00000165920377801949100570000002583859885900944542_	figures/combined-sparsity-plots.svg	/^						c0.6,0,1.3,0,2-0.1c0.8-0.1,1.6-0.2,2.5-0.4L-337,362.5z"\/>$/;"	i
DejaVuSans-72_00000171690224269782885700000016518965717008465297_	figures/combined-sparsity-plots.svg	/^						c0.6,0,1.3,0,2-0.1c0.8-0.1,1.6-0.2,2.5-0.4L-273.4,362.5z"\/>$/;"	i
DejaVuSans-72_00000175280199361517835280000004792799359533370016_	figures/combined-sparsity-plots.svg	/^						c0.6,0,1.3,0,2-0.1c0.8-0.1,1.6-0.2,2.5-0.4L-273.4,362.5z"\/>$/;"	i
DejaVuSans-72_00000178894381081741326660000018069004896555184771_	figures/combined-sparsity-plots.svg	/^						c0.6,0,1.3,0,2-0.1c0.8-0.1,1.6-0.2,2.5-0.4L135.1,362.5z"\/>$/;"	i
DejaVuSans-72_00000178910902288826609830000013880636530109285511_	figures/combined-sparsity-plots.svg	/^						c0.6,0,1.3,0,2-0.1c0.8-0.1,1.6-0.2,2.5-0.4L135.1,362.5z"\/>$/;"	i
DejaVuSans-72_00000181077581951516407770000006142752639459149210_	figures/combined-sparsity-plots.svg	/^						c3,1.6,6.7,2.4,11,2.4c0.6,0,1.3,0,2-0.1c0.8-0.1,1.6-0.2,2.5-0.4L1193.9,772.7z"\/>$/;"	i
DejaVuSans-73_00000009575743936459654880000006708639450990710437_	figures/combined-sparsity-plots.svg	/^						c3.6,2.8,8.8,4.2,15.5,4.2c3.3,0,6.4-0.2,9.4-0.7C-5.9-4443.4-3.2-4444.1-0.7-4445.1z"\/>$/;"	i
DejaVuSans-73_00000019671172893138951170000017844232957189380481_	figures/combined-sparsity-plots.svg	/^						c3.6,2.8,8.8,4.2,15.5,4.2c3.3,0,6.4-0.2,9.4-0.7C-43.8,371-41.1,370.3-38.6,369.3z"\/>$/;"	i
DejaVuSans-73_00000024001838953802793760000005695081947790847122_	figures/combined-sparsity-plots.svg	/^						c3.6,2.8,8.8,4.2,15.5,4.2c3.3,0,6.4-0.2,9.4-0.7C174.2,371,176.9,370.3,179.3,369.3z"\/>$/;"	i
DejaVuSans-73_00000025422903494423948330000017627245088699712904_	figures/combined-sparsity-plots.svg	/^						c3.6,2.8,8.8,4.2,15.5,4.2c3.3,0,6.4-0.2,9.4-0.7C664.7-4443.4,667.4-4444.1,669.9-4445.1z"\//;"	i
DejaVuSans-73_00000026847314949005944160000013524263098787828866_	figures/combined-sparsity-plots.svg	/^						c3.6,2.8,8.8,4.2,15.5,4.2c3.3,0,6.4-0.2,9.4-0.7C-107.4,371-104.7,370.3-102.3,369.3z"\/>$/;"	i
DejaVuSans-73_00000034781289939733981660000008460142680751303040_	figures/combined-sparsity-plots.svg	/^						c3.6,2.8,8.8,4.2,15.5,4.2c3.3,0,6.4-0.2,9.4-0.7C-43.8,371-41.1,370.3-38.6,369.3z"\/>$/;"	i
DejaVuSans-73_00000040565685950029245200000005990999428920698556_	figures/combined-sparsity-plots.svg	/^						c3.6,2.8,8.8,4.2,15.5,4.2c3.3,0,6.4-0.2,9.4-0.7C2084.3,781.2,2087,780.4,2089.5,779.4z"\/>$/;"	i
DejaVuSans-73_00000041285326702255001390000000657730911878775977_	figures/combined-sparsity-plots.svg	/^						c3.6,2.8,8.8,4.2,15.5,4.2c3.3,0,6.4-0.2,9.4-0.7C1636.2,781.2,1638.9,780.4,1641.4,779.4z"\//;"	i
DejaVuSans-73_00000044871047319454827580000000024009378077297554_	figures/combined-sparsity-plots.svg	/^						c3.6,2.8,8.8,4.2,15.5,4.2c3.3,0,6.4-0.2,9.4-0.7C174.2,371,176.9,370.3,179.3,369.3z"\/>$/;"	i
DejaVuSans-73_00000048496689709808262730000002849330281182816950_	figures/combined-sparsity-plots.svg	/^						c3.6,2.8,8.8,4.2,15.5,4.2c3.3,0,6.4-0.2,9.4-0.7C174.2,371,176.9,370.3,179.3,369.3z"\/>$/;"	i
DejaVuSans-73_00000052824070883035000820000006338226810551934900_	figures/combined-sparsity-plots.svg	/^					c3.3,0,6.4-0.2,9.4-0.7C-263.5,2347.6-260.8,2346.9-258.3,2345.9z"\/>$/;"	i
DejaVuSans-73_00000057839104191095999200000010730477027283797639_	figures/combined-sparsity-plots.svg	/^						c3.6,2.8,8.8,4.2,15.5,4.2c3.3,0,6.4-0.2,9.4-0.7C-4373.5,783.7-4370.8,783-4368.3,782z"\/>$/;"	i
DejaVuSans-73_00000059274561950612515940000005552828928819215775_	figures/combined-sparsity-plots.svg	/^						c3.6,2.8,8.8,4.2,15.5,4.2c3.3,0,6.4-0.2,9.4-0.7C530.3,781.2,533,780.4,535.5,779.4z"\/>$/;"	i
DejaVuSans-73_00000067194867467711630240000008011680386443035041_	figures/combined-sparsity-plots.svg	/^						c3.6,2.8,8.8,4.2,15.5,4.2c3.3,0,6.4-0.2,9.4-0.7C174.2,371,176.9,370.3,179.3,369.3z"\/>$/;"	i
DejaVuSans-73_00000067938232694549604900000002979523777718530976_	figures/combined-sparsity-plots.svg	/^						c3.6,2.8,8.8,4.2,15.5,4.2c3.3,0,6.4-0.2,9.4-0.7C-4321.4,783.7-4318.7,783-4316.2,782z"\/>$/;"	i
DejaVuSans-73_00000069358905722816794470000015773259984017707704_	figures/combined-sparsity-plots.svg	/^						c3.6,2.8,8.8,4.2,15.5,4.2c3.3,0,6.4-0.2,9.4-0.7C-43.8,371-41.1,370.3-38.6,369.3z"\/>$/;"	i
DejaVuSans-73_00000072971917375273792870000005246833788781067175_	figures/combined-sparsity-plots.svg	/^						c3.6,2.8,8.8,4.2,15.5,4.2c3.3,0,6.4-0.2,9.4-0.7C1.6,394.9,4.3,394.2,6.8,393.2z"\/>$/;"	i
DejaVuSans-73_00000074438491212517391690000001659063279245726610_	figures/combined-sparsity-plots.svg	/^						c3.6,2.8,8.8,4.2,15.5,4.2c3.3,0,6.4-0.2,9.4-0.7C468.2,781.2,470.9,780.4,473.4,779.4z"\/>$/;"	i
DejaVuSans-73_00000080887066044300287180000000681295932323472265_	figures/combined-sparsity-plots.svg	/^						c3.6,2.8,8.8,4.2,15.5,4.2c3.3,0,6.4-0.2,9.4-0.7C-267.4-4446.8-264.6-4447.5-262.2-4448.5z"\//;"	i
DejaVuSans-73_00000083084941671066424220000016170248624059972765_	figures/combined-sparsity-plots.svg	/^						c3.6,2.8,8.8,4.2,15.5,4.2c3.3,0,6.4-0.2,9.4-0.7C-43.8,371-41.1,370.3-38.6,369.3z"\/>$/;"	i
DejaVuSans-73_00000087397928539405828970000008322515383081817503_	figures/combined-sparsity-plots.svg	/^						c3.6,2.8,8.8,4.2,15.5,4.2c3.3,0,6.4-0.2,9.4-0.7C-43.8,371-41.1,370.3-38.6,369.3z"\/>$/;"	i
DejaVuSans-73_00000093855568438530762800000006968318521851607687_	figures/combined-sparsity-plots.svg	/^						c3.6,2.8,8.8,4.2,15.5,4.2c3.3,0,6.4-0.2,9.4-0.7C-264.8,304.9-262.1,304.2-259.6,303.2z"\/>$/;"	i
DejaVuSans-73_00000098204852541650607450000011834122319777120664_	figures/combined-sparsity-plots.svg	/^						c3.6,2.8,8.8,4.2,15.5,4.2c3.3,0,6.4-0.2,9.4-0.7C174.2,371,176.9,370.3,179.3,369.3z"\/>$/;"	i
DejaVuSans-73_00000101061013011415276750000010598057710540843159_	figures/combined-sparsity-plots.svg	/^						c3.6,2.8,8.8,4.2,15.5,4.2c3.3,0,6.4-0.2,9.4-0.7C1355.7,781.2,1358.4,780.4,1360.9,779.4z"\//;"	i
DejaVuSans-73_00000101783047360742609970000007106745093011648178_	figures/combined-sparsity-plots.svg	/^						c3.6,2.8,8.8,4.2,15.5,4.2c3.3,0,6.4-0.2,9.4-0.7C110.5,371,113.2,370.3,115.7,369.3z"\/>$/;"	i
DejaVuSans-73_00000114765144656124981440000004532964635966673845_	figures/combined-sparsity-plots.svg	/^						c3.6,2.8,8.8,4.2,15.5,4.2c3.3,0,6.4-0.2,9.4-0.7C174.2,371,176.9,370.3,179.3,369.3z"\/>$/;"	i
DejaVuSans-73_00000134936660538497732800000018310037622389483907_	figures/combined-sparsity-plots.svg	/^						c3.6,2.8,8.8,4.2,15.5,4.2c3.3,0,6.4-0.2,9.4-0.7C174.2,371,176.9,370.3,179.3,369.3z"\/>$/;"	i
DejaVuSans-73_00000138552055223404149960000014668183052652917888_	figures/combined-sparsity-plots.svg	/^						c3.6,2.8,8.8,4.2,15.5,4.2c3.3,0,6.4-0.2,9.4-0.7C672.2,394.9,674.9,394.2,677.3,393.2z"\/>$/;"	i
DejaVuSans-73_00000139258979890116620350000016474697859036449927_	figures/combined-sparsity-plots.svg	/^						c3.6,2.8,8.8,4.2,15.5,4.2c3.3,0,6.4-0.2,9.4-0.7C520.3,781.2,523,780.4,525.5,779.4z"\/>$/;"	i
DejaVuSans-73_00000141439894029301783160000014337594027294982543_	figures/combined-sparsity-plots.svg	/^						c3.6,2.8,8.8,4.2,15.5,4.2c3.3,0,6.4-0.2,9.4-0.7C478.2,781.2,480.9,780.4,483.4,779.4z"\/>$/;"	i
DejaVuSans-73_00000143609495783294763260000014866377134377628554_	figures/combined-sparsity-plots.svg	/^						c3.6,2.8,8.8,4.2,15.5,4.2c3.3,0,6.4-0.2,9.4-0.7C-4318,788.6-4315.3,787.9-4312.8,786.9z"\/>$/;"	i
DejaVuSans-73_00000146496612742875577240000007804482261095475628_	figures/combined-sparsity-plots.svg	/^						c3.6,2.8,8.8,4.2,15.5,4.2c3.3,0,6.4-0.2,9.4-0.7C689.6,781.2,692.3,780.4,694.8,779.4z"\/>$/;"	i
DejaVuSans-73_00000154422877302581955220000016470901789415421080_	figures/combined-sparsity-plots.svg	/^						c3.6,2.8,8.8,4.2,15.5,4.2c3.3,0,6.4-0.2,9.4-0.7C-264.8,304.9-262.1,304.2-259.6,303.2z"\/>$/;"	i
DejaVuSans-73_00000157995978204416678460000011679605939266976644_	figures/combined-sparsity-plots.svg	/^						c3.6,2.8,8.8,4.2,15.5,4.2c3.3,0,6.4-0.2,9.4-0.7C-43.8,371-41.1,370.3-38.6,369.3z"\/>$/;"	i
DejaVuSans-73_00000158015122024829318260000018130716500904576685_	figures/combined-sparsity-plots.svg	/^						c3.6,2.8,8.8,4.2,15.5,4.2c3.3,0,6.4-0.2,9.4-0.7C-4370.1,788.6-4367.4,787.9-4364.9,786.9z"\//;"	i
DejaVuSans-73_00000158721975742386125670000004277013434166528162_	figures/combined-sparsity-plots.svg	/^						c3.6,2.8,8.8,4.2,15.5,4.2c3.3,0,6.4-0.2,9.4-0.7C-43.8,371-41.1,370.3-38.6,369.3z"\/>$/;"	i
DejaVuSans-73_00000161615550653310574030000017941293663957803154_	figures/combined-sparsity-plots.svg	/^						c3.6,2.8,8.8,4.2,15.5,4.2c3.3,0,6.4-0.2,9.4-0.7C1137.7,781.2,1140.4,780.4,1142.9,779.4z"\//;"	i
DejaVuSans-73_00000167374563570585576830000013263908017738498435_	figures/combined-sparsity-plots.svg	/^						c3.6,2.8,8.8,4.2,15.5,4.2c3.3,0,6.4-0.2,9.4-0.7C174.2,371,176.9,370.3,179.3,369.3z"\/>$/;"	i
DejaVuSans-73_00000173877086203276254360000002527062027071177892_	figures/combined-sparsity-plots.svg	/^						c3.6,2.8,8.8,4.2,15.5,4.2c3.3,0,6.4-0.2,9.4-0.7C174.2,371,176.9,370.3,179.3,369.3z"\/>$/;"	i
DejaVuSans-73_00000175299053236271109680000014022700282597176734_	figures/combined-sparsity-plots.svg	/^						c3.6,2.8,8.8,4.2,15.5,4.2c3.3,0,6.4-0.2,9.4-0.7C907.6,781.2,910.3,780.4,912.8,779.4z"\/>$/;"	i
DejaVuSans-73_00000180369081731217864150000010875358762845114287_	figures/combined-sparsity-plots.svg	/^						c3.6,2.8,8.8,4.2,15.5,4.2c3.3,0,6.4-0.2,9.4-0.7C-43.8,371-41.1,370.3-38.6,369.3z"\/>$/;"	i
DejaVuSans-73_00000181052302003324391200000011808730321518039168_	figures/combined-sparsity-plots.svg	/^						c3.6,2.8,8.8,4.2,15.5,4.2c3.3,0,6.4-0.2,9.4-0.7C-43.8,371-41.1,370.3-38.6,369.3z"\/>$/;"	i
DejaVuSans-74_00000001631887977574564410000009234494528187531185_	figures/combined-sparsity-plots.svg	/^						H25.4z"\/>$/;"	i
DejaVuSans-74_00000010297487865706150950000014054051517822805400_	figures/combined-sparsity-plots.svg	/^						h6.6v15.5H-367.6z"\/>$/;"	i
DejaVuSans-74_00000011749474435161566920000005480911282714382498_	figures/combined-sparsity-plots.svg	/^						h6.6v15.5H233.3z"\/>$/;"	i
DejaVuSans-74_00000020359809679541941730000013161406618855790244_	figures/combined-sparsity-plots.svg	/^						h6.6v15.5H233.3z"\/>$/;"	i
DejaVuSans-74_00000032607810446603737940000009243724053877694622_	figures/combined-sparsity-plots.svg	/^						H452.3z"\/>$/;"	i
DejaVuSans-74_00000034792000029377102310000001433122367549005956_	figures/combined-sparsity-plots.svg	/^						h6.6v15.5H-682.8z"\/>$/;"	i
DejaVuSans-74_00000038390503999067250320000002688993234439155599_	figures/combined-sparsity-plots.svg	/^					H-679z"\/>$/;"	i
DejaVuSans-74_00000046329261138332058900000016263943233771940484_	figures/combined-sparsity-plots.svg	/^						H917.9z"\/>$/;"	i
DejaVuSans-74_00000069376397739445003170000005882189536184244889_	figures/combined-sparsity-plots.svg	/^						H966.7z"\/>$/;"	i
DejaVuSans-74_00000071558489713161187620000010168225341555645100_	figures/combined-sparsity-plots.svg	/^						h6.6v15.5H233.3z"\/>$/;"	i
DejaVuSans-74_00000078723437661258538310000013105834222495820458_	figures/combined-sparsity-plots.svg	/^						H1328.5z"\/>$/;"	i
DejaVuSans-74_00000091702960336715802000000006788707502803312537_	figures/combined-sparsity-plots.svg	/^						H-375.1z"\/>$/;"	i
DejaVuSans-74_00000095305217506482774740000007381340177854659247_	figures/combined-sparsity-plots.svg	/^						H249.2z"\/>$/;"	i
DejaVuSans-74_00000096053487637326583590000016282852791069625013_	figures/combined-sparsity-plots.svg	/^						h6.6v15.5H233.3z"\/>$/;"	i
DejaVuSans-74_00000096762876463616679310000006921388420845556117_	figures/combined-sparsity-plots.svg	/^						h6.6v15.5H-477.1z"\/>$/;"	i
DejaVuSans-74_00000096765112602269827110000009212079295695684009_	figures/combined-sparsity-plots.svg	/^						h6.6v15.5H-479.7z"\/>$/;"	i
DejaVuSans-74_00000113327961102783851830000016811036100232567978_	figures/combined-sparsity-plots.svg	/^						H1414.8z"\/>$/;"	i
DejaVuSans-74_00000116925340184177584620000006640830638202517417_	figures/combined-sparsity-plots.svg	/^						H384.7z"\/>$/;"	i
DejaVuSans-74_00000120532580833313816490000007785528234027201446_	figures/combined-sparsity-plots.svg	/^						v15.5H256.7z"\/>$/;"	i
DejaVuSans-74_00000131365248216060604540000006599649005985867922_	figures/combined-sparsity-plots.svg	/^						h6.6v15.5H233.3z"\/>$/;"	i
DejaVuSans-74_00000132084334153144935440000015749808537610222765_	figures/combined-sparsity-plots.svg	/^						h6.6v15.5H-680.3z"\/>$/;"	i
DejaVuSans-74_00000134240461441233900840000001238667921849740680_	figures/combined-sparsity-plots.svg	/^						h6.6v15.5H233.3z"\/>$/;"	i
DejaVuSans-74_00000136390591071681907360000013497070333204351155_	figures/combined-sparsity-plots.svg	/^						h6.6v15.5H233.3z"\/>$/;"	i
DejaVuSans-74_00000139255621957740892160000010930137381020006542_	figures/combined-sparsity-plots.svg	/^						h6.6v15.5H-477.1z"\/>$/;"	i
DejaVuSans-74_00000144336663469219552410000013542486550684146308_	figures/combined-sparsity-plots.svg	/^						h6.6v15.5H32.9z"\/>$/;"	i
DejaVuSans-74_00000147901479168044596700000000970393117258227587_	figures/combined-sparsity-plots.svg	/^						H538.7z"\/>$/;"	i
DejaVuSans-74_00000147917177766925164940000013472749870404372132_	figures/combined-sparsity-plots.svg	/^					v15.5H-475.8z"\/>$/;"	i
DejaVuSans-74_00000168116495219518133750000008728489824110862226_	figures/combined-sparsity-plots.svg	/^						h6.6v15.5H233.3z"\/>$/;"	i
DejaVuSans-74_00000173126709717606987370000002231527389281016970_	figures/combined-sparsity-plots.svg	/^						h6.6v15.5H-680.3z"\/>$/;"	i
DejaVuSans-74_00000174591398844982584170000013859421332217307285_	figures/combined-sparsity-plots.svg	/^						H1776.6z"\/>$/;"	i
DejaVuSans-74_00000180339521284161422130000012008098079075272122_	figures/combined-sparsity-plots.svg	/^						h6.6v15.5H459.8z"\/>$/;"	i
DejaVuSans-74_00000181059158887438240860000001370951486230754949_	figures/combined-sparsity-plots.svg	/^						v15.5H169.6z"\/>$/;"	i
DejaVuSans-74_00000181079472845101158800000007216323535821936025_	figures/combined-sparsity-plots.svg	/^						h6.6v15.5H233.3z"\/>$/;"	i
DejaVuSans-75	figures/combined-sparsity-plots.svg	/^						C-446.7-4489.8-448.3-4484.1-448.3-4476.6z M-425.7-4442.2L-425.7-4442.2z"\/>$/;"	i
DejaVuSans-75_00000011017213758940876360000015989964855586408349_	figures/combined-sparsity-plots.svg	/^						c-2.9-1.6-6.2-2.4-10-2.4c-6.3,0-11.1,2-14.3,5.9C414.4,734.7,412.8,740.4,412.8,747.9z M435./;"	i
DejaVuSans-75_00000052822269081384563470000010806465154583031693_	figures/combined-sparsity-plots.svg	/^						c-6.3,0-11.1,2-14.3,5.9C-90.8,348.5-92.4,354.2-92.4,361.7z M-69.8,396.1L-69.8,396.1z"\/>$/;"	i
DejaVuSans-75_00000116953709196686210180000007395117991854880936_	figures/combined-sparsity-plots.svg	/^						c-6.3,0-11.1,2-14.3,5.9C-439.2,348.5-440.8,354.2-440.8,361.7z M-418.2,396.1L-418.2,396.1z"/;"	i
DejaVuSans-75_00000173856038333904470870000012858193262628475273_	figures/combined-sparsity-plots.svg	/^						s-6.2-2.4-10-2.4c-6.3,0-11.1,2-14.3,5.9C-98.2-4489.8-99.8-4484.1-99.8-4476.6z M-77.2-4442./;"	i
DejaVuSans-76_00000079484140213394075970000004947069348583171508_	figures/combined-sparsity-plots.svg	/^						l-20.5-54.7h-12.2L436.4,781.1z"\/>$/;"	i
DejaVuSans-78_00000163753020319229989230000003205477889147459223_	figures/combined-sparsity-plots.svg	/^						l-15.9,21.5l-15.9-21.5h-10.6l21.2,28.6l-19.4,26.1h10.6l14.5-19.5l14.5,19.5H1062.6z"\/>$/;"	i
DejaVuSans-79_00000003102003971491814280000001066376010219411611_	figures/combined-sparsity-plots.svg	/^						h9.5L1019.8,721.3z"\/>$/;"	i
DejaVuSans-79_00000021825542404251065550000015031670314368505233_	figures/combined-sparsity-plots.svg	/^						h9.5L286.3,311.1z"\/>$/;"	i
DejaVuSans-79_00000092435997682243937550000000877011628052784798_	figures/combined-sparsity-plots.svg	/^						h9.5L286.3,311.1z"\/>$/;"	i
DejaVuSans-79_00000110436749300350367980000005871089247880499591_	figures/combined-sparsity-plots.svg	/^						h9.5L286.3,311.1z"\/>$/;"	i
DejaVuSans-79_00000135676975762987781120000017459101221484566937_	figures/combined-sparsity-plots.svg	/^						h9.5L591.7,721.3z"\/>$/;"	i
DejaVuSans-79_00000140737389194441120830000002371574239472911247_	figures/combined-sparsity-plots.svg	/^						h9.5L222.7,311.1z"\/>$/;"	i
DejaVuSans-79_00000151530652732163328030000018251885057041631110_	figures/combined-sparsity-plots.svg	/^						h9.5L286.3,311.1z"\/>$/;"	i
DejaVuSans-79_00000154408343683337729660000014860879845122854279_	figures/combined-sparsity-plots.svg	/^						h9.5L286.3,311.1z"\/>$/;"	i
DejaVuSans-79_00000154427290199195789410000006749170356212689054_	figures/combined-sparsity-plots.svg	/^						h9.5L286.3,311.1z"\/>$/;"	i
DejaVuSans-79_00000166644136060244237720000013153064936196487866_	figures/combined-sparsity-plots.svg	/^						h9.5L286.3,311.1z"\/>$/;"	i
DejaVuSans-79_00000169543869061668253140000012222963591167929759_	figures/combined-sparsity-plots.svg	/^						h9.5L286.3,311.1z"\/>$/;"	i
DejaVuSans-79_00000178199542529532957060000016171159718505938342_	figures/combined-sparsity-plots.svg	/^						h9.5L286.3,311.1z"\/>$/;"	i
DejaVuSans-79_00000181809079146027402900000016751780238097206174_	figures/combined-sparsity-plots.svg	/^						L1467.9,721.3z"\/>$/;"	i
Discussion	main.tex	/^\\section{Discussion}\\label{sec:discussion}$/;"	s
DropConnect	references.bib	/^@InProceedings{DropConnect,$/;"	j
DynamicEvaluation	references.bib	/^@InProceedings{DynamicEvaluation,$/;"	j
Efficient RTRL with activity AND parameter sparsity	main.tex	/^\\section{Efficient RTRL with activity AND parameter sparsity}$/;"	s
Efficient RTRL with activity sparsity	main.tex	/^\\section{Efficient RTRL with activity sparsity}$/;"	s
Gewaltig2007NEST	references.bib	/^@article{Gewaltig2007NEST,$/;"	a
Introduction	main.tex	/^\\section{Introduction}$/;"	s
LMZaremba	references.bib	/^@misc{LMZaremba,$/;"	n
Layer_1	figures/combined-sparsity-plots.svg	/^	 viewBox="0 0 928 657" style="enable-background:new 0 0 928 657;" xml:space="preserve">$/;"	i
Melis2018	references.bib	/^@inproceedings{Melis2018,$/;"	j
NeuralCache	references.bib	/^@inproceedings{NeuralCache,$/;"	j
PennTreebank	references.bib	/^@article{PennTreebank,$/;"	a
PolyCollection_10_00000060735618176643067240000012493213719306289087_	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_10_00000060735618176643067240000012493213719306289087_">$/;"	i
PolyCollection_10_00000116933582099618035480000009133485343621842572_	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_10_00000116933582099618035480000009133485343621842572_">$/;"	i
PolyCollection_11	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_11">$/;"	i
PolyCollection_11_00000069365210121898797670000011539364323312400028_	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_11_00000069365210121898797670000011539364323312400028_">$/;"	i
PolyCollection_12	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_12">$/;"	i
PolyCollection_12_00000028305248537295650140000012756715301909973148_	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_12_00000028305248537295650140000012756715301909973148_">$/;"	i
PolyCollection_13	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_13">$/;"	i
PolyCollection_13_00000092425445056490091330000013255465857992659872_	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_13_00000092425445056490091330000013255465857992659872_">$/;"	i
PolyCollection_14	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_14">$/;"	i
PolyCollection_14_00000001628193252111969080000008904187218233110944_	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_14_00000001628193252111969080000008904187218233110944_">$/;"	i
PolyCollection_15	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_15">$/;"	i
PolyCollection_15_00000092452452279075028930000000725615493829215650_	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_15_00000092452452279075028930000000725615493829215650_">$/;"	i
PolyCollection_16	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_16">$/;"	i
PolyCollection_16_00000160178664671203602850000003890458905132751277_	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_16_00000160178664671203602850000003890458905132751277_">$/;"	i
PolyCollection_17	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_17">$/;"	i
PolyCollection_17_00000008842239296126696810000014191217386944968347_	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_17_00000008842239296126696810000014191217386944968347_">$/;"	i
PolyCollection_18	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_18">$/;"	i
PolyCollection_18_00000078025779591470710030000004786935618722475650_	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_18_00000078025779591470710030000004786935618722475650_">$/;"	i
PolyCollection_19	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_19">$/;"	i
PolyCollection_19_00000117671617066792930440000011359649918968640151_	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_19_00000117671617066792930440000011359649918968640151_">$/;"	i
PolyCollection_1_00000131364506359579476230000005409750591226576277_	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_1_00000131364506359579476230000005409750591226576277_">$/;"	i
PolyCollection_1_00000167396180975778983290000010451736528175694757_	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_1_00000167396180975778983290000010451736528175694757_">$/;"	i
PolyCollection_20	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_20">$/;"	i
PolyCollection_20_00000036937138145744432460000013790488776361569215_	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_20_00000036937138145744432460000013790488776361569215_">$/;"	i
PolyCollection_21_00000072281674673875581840000006799080311868024741_	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_21_00000072281674673875581840000006799080311868024741_">$/;"	i
PolyCollection_22_00000029750435382610868430000003381934016233164681_	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_22_00000029750435382610868430000003381934016233164681_">$/;"	i
PolyCollection_23_00000018946500677383475640000013456004049684041878_	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_23_00000018946500677383475640000013456004049684041878_">$/;"	i
PolyCollection_24_00000101781855275739290820000010985760042334326688_	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_24_00000101781855275739290820000010985760042334326688_">$/;"	i
PolyCollection_25_00000010299623978147081700000015406253034106371256_	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_25_00000010299623978147081700000015406253034106371256_">$/;"	i
PolyCollection_26_00000168837701269515314870000017752059546519163808_	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_26_00000168837701269515314870000017752059546519163808_">$/;"	i
PolyCollection_27_00000119079106909489922510000000701366012200114056_	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_27_00000119079106909489922510000000701366012200114056_">$/;"	i
PolyCollection_28_00000149364516823511178440000013873135761767217830_	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_28_00000149364516823511178440000013873135761767217830_">$/;"	i
PolyCollection_29_00000062905038278633005540000014089262132102068151_	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_29_00000062905038278633005540000014089262132102068151_">$/;"	i
PolyCollection_2_00000083794628800591037600000012430630887713653169_	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_2_00000083794628800591037600000012430630887713653169_">$/;"	i
PolyCollection_2_00000139261798688278066110000007346242754042578595_	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_2_00000139261798688278066110000007346242754042578595_">$/;"	i
PolyCollection_30_00000126295828540848146970000018199790740381595793_	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_30_00000126295828540848146970000018199790740381595793_">$/;"	i
PolyCollection_31_00000103241708628885275120000005343792890025930383_	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_31_00000103241708628885275120000005343792890025930383_">$/;"	i
PolyCollection_32_00000023991858715014615910000018436129810465355196_	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_32_00000023991858715014615910000018436129810465355196_">$/;"	i
PolyCollection_33_00000153678490580531254430000009081153555984523143_	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_33_00000153678490580531254430000009081153555984523143_">$/;"	i
PolyCollection_34_00000135685620991160586240000002954203904844928923_	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_34_00000135685620991160586240000002954203904844928923_">$/;"	i
PolyCollection_35_00000111893185422652096770000017156570099116787124_	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_35_00000111893185422652096770000017156570099116787124_">$/;"	i
PolyCollection_36_00000012450630180519839730000000167984333747862446_	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_36_00000012450630180519839730000000167984333747862446_">$/;"	i
PolyCollection_37_00000098196304870760504940000001088788206921165737_	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_37_00000098196304870760504940000001088788206921165737_">$/;"	i
PolyCollection_38_00000038387745913239360140000001318968374404258951_	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_38_00000038387745913239360140000001318968374404258951_">$/;"	i
PolyCollection_39_00000098941308919646765340000004829692479949422007_	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_39_00000098941308919646765340000004829692479949422007_">$/;"	i
PolyCollection_3_00000105399663971036139580000018190188528546427548_	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_3_00000105399663971036139580000018190188528546427548_">$/;"	i
PolyCollection_3_00000122679185321291017670000014537116523917158017_	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_3_00000122679185321291017670000014537116523917158017_">$/;"	i
PolyCollection_40_00000112608613894075815090000000679029627362013627_	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_40_00000112608613894075815090000000679029627362013627_">$/;"	i
PolyCollection_4_00000150814623089147559050000014751742038281599366_	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_4_00000150814623089147559050000014751742038281599366_">$/;"	i
PolyCollection_4_00000158009389379620948670000004499067236054373815_	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_4_00000158009389379620948670000004499067236054373815_">$/;"	i
PolyCollection_5_00000055685848108692162270000007303018277474779530_	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_5_00000055685848108692162270000007303018277474779530_">$/;"	i
PolyCollection_5_00000170242620188641189390000004060183992267869597_	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_5_00000170242620188641189390000004060183992267869597_">$/;"	i
PolyCollection_6_00000044885974303119086000000010849253301248996534_	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_6_00000044885974303119086000000010849253301248996534_">$/;"	i
PolyCollection_6_00000106130572101198322170000013330549078835829175_	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_6_00000106130572101198322170000013330549078835829175_">$/;"	i
PolyCollection_7_00000031889245908098526230000017880183033101443766_	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_7_00000031889245908098526230000017880183033101443766_">$/;"	i
PolyCollection_7_00000071542621001098237040000017301068024303005859_	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_7_00000071542621001098237040000017301068024303005859_">$/;"	i
PolyCollection_8_00000052795286530027426940000015416225559574634401_	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_8_00000052795286530027426940000015416225559574634401_">$/;"	i
PolyCollection_8_00000116932464913493731370000012867081797150312602_	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_8_00000116932464913493731370000012867081797150312602_">$/;"	i
PolyCollection_9_00000035518975326875082420000014543479534513566358_	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_9_00000035518975326875082420000014543479534513566358_">$/;"	i
PolyCollection_9_00000039118916124557349340000001243504086768070532_	figures/combined-sparsity-plots.svg	/^	<g id="PolyCollection_9_00000039118916124557349340000001243504086768070532_">$/;"	i
Real Time Recurrent Learning	main.tex	/^\\section{Real Time Recurrent Learning}$/;"	s
Related work	main.tex	/^\\section{Related work}$/;"	s
Results	main.tex	/^\\section{Results}$/;"	s
SVGID_00000000223328424809645530000000444089946208402110_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000000223328424809645530000000444089946208402110_">$/;"	i
SVGID_00000000911457068503216580000000806340862833587095_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000000911457068503216580000000806340862833587095_" x="518.2" y="493" widt/;"	d
SVGID_00000000911457068503216580000000806340862833587095_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000000911457068503216580000000806340862833587095_" x="518.2" y="493" widt/;"	i
SVGID_00000000940519219827916080000000965633771449961138_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000000940519219827916080000000965633771449961138_">$/;"	i
SVGID_00000001650598774438930130000005216267860333486249_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000001650598774438930130000005216267860333486249_">$/;"	i
SVGID_00000001653133892919124550000000112336479616280221_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000001653133892919124550000000112336479616280221_">$/;"	i
SVGID_00000002343008978857398680000015976043458020037792_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000002343008978857398680000015976043458020037792_" x="518.9" y="257.1" wi/;"	d
SVGID_00000002343008978857398680000015976043458020037792_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000002343008978857398680000015976043458020037792_" x="518.9" y="257.1" wi/;"	i
SVGID_00000002361182376672300840000000961304923794982556_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000002361182376672300840000000961304923794982556_" x="62.4" y="51.4" widt/;"	d
SVGID_00000002361182376672300840000000961304923794982556_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000002361182376672300840000000961304923794982556_" x="62.4" y="51.4" widt/;"	i
SVGID_00000003094146568885214540000006751435924399656326_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000003094146568885214540000006751435924399656326_">$/;"	i
SVGID_00000005956505624137992610000010127064399245825716_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000005956505624137992610000010127064399245825716_" x="62.4" y="51.4" widt/;"	d
SVGID_00000005956505624137992610000010127064399245825716_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000005956505624137992610000010127064399245825716_" x="62.4" y="51.4" widt/;"	i
SVGID_00000006686401193090897620000015462588117321799566_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000006686401193090897620000015462588117321799566_" x="518.9" y="52.4" wid/;"	d
SVGID_00000006686401193090897620000015462588117321799566_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000006686401193090897620000015462588117321799566_" x="518.9" y="52.4" wid/;"	i
SVGID_00000006687552801527891270000008838809867450419593_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000006687552801527891270000008838809867450419593_">$/;"	i
SVGID_00000007388179263750596820000010755696509028603787_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000007388179263750596820000010755696509028603787_" x="62.1" y="493.4" wid/;"	d
SVGID_00000007388179263750596820000010755696509028603787_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000007388179263750596820000010755696509028603787_" x="62.1" y="493.4" wid/;"	i
SVGID_00000007420129605571602010000004864812905763396238_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000007420129605571602010000004864812905763396238_">$/;"	i
SVGID_00000008848413721638836320000015049464514660617392_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000008848413721638836320000015049464514660617392_" x="62.4" y="51.4" widt/;"	d
SVGID_00000008848413721638836320000015049464514660617392_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000008848413721638836320000015049464514660617392_" x="62.4" y="51.4" widt/;"	i
SVGID_00000009571520401750645600000003752798624073174454_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000009571520401750645600000003752798624073174454_" x="518.2" y="493" widt/;"	d
SVGID_00000009571520401750645600000003752798624073174454_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000009571520401750645600000003752798624073174454_" x="518.2" y="493" widt/;"	i
SVGID_00000009582970449613699350000007923318576237386920_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000009582970449613699350000007923318576237386920_" x="518.9" y="257.1" wi/;"	d
SVGID_00000009582970449613699350000007923318576237386920_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000009582970449613699350000007923318576237386920_" x="518.9" y="257.1" wi/;"	i
SVGID_00000011731491804933093240000015920864892210338455_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000011731491804933093240000015920864892210338455_">$/;"	i
SVGID_00000012441239450255490170000001426990443448978075_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000012441239450255490170000001426990443448978075_">$/;"	i
SVGID_00000012458039864533832200000017342480360640672139_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000012458039864533832200000017342480360640672139_" x="62.1" y="493.4" wid/;"	d
SVGID_00000012458039864533832200000017342480360640672139_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000012458039864533832200000017342480360640672139_" x="62.1" y="493.4" wid/;"	i
SVGID_00000013192423918773773400000014735117618091122049_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000013192423918773773400000014735117618091122049_" x="518.9" y="52.4" wid/;"	d
SVGID_00000013192423918773773400000014735117618091122049_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000013192423918773773400000014735117618091122049_" x="518.9" y="52.4" wid/;"	i
SVGID_00000014613134530641137460000014272133482405362828_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000014613134530641137460000014272133482405362828_" x="518.9" y="257.1" wi/;"	d
SVGID_00000014613134530641137460000014272133482405362828_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000014613134530641137460000014272133482405362828_" x="518.9" y="257.1" wi/;"	i
SVGID_00000015325875818237736400000002306224065875446437_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000015325875818237736400000002306224065875446437_">$/;"	i
SVGID_00000015329129478999301860000013345444465265772691_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000015329129478999301860000013345444465265772691_">$/;"	i
SVGID_00000016072072629963643810000011370317388712336550_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000016072072629963643810000011370317388712336550_">$/;"	i
SVGID_00000018230288918150934790000002768637216831382152_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000018230288918150934790000002768637216831382152_" x="62.4" y="257.1" wid/;"	d
SVGID_00000018230288918150934790000002768637216831382152_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000018230288918150934790000002768637216831382152_" x="62.4" y="257.1" wid/;"	i
SVGID_00000018956267941595098320000009800759059601586851_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000018956267941595098320000009800759059601586851_">$/;"	i
SVGID_00000019670517107459898200000013129212208944561825_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000019670517107459898200000013129212208944561825_">$/;"	i
SVGID_00000020366024168239227140000001190962458886463654_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000020366024168239227140000001190962458886463654_" x="518.9" y="52.4" wid/;"	d
SVGID_00000020366024168239227140000001190962458886463654_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000020366024168239227140000001190962458886463654_" x="518.9" y="52.4" wid/;"	i
SVGID_00000021799446363863960580000002648153267114412461_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000021799446363863960580000002648153267114412461_" x="518.2" y="493" widt/;"	d
SVGID_00000021799446363863960580000002648153267114412461_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000021799446363863960580000002648153267114412461_" x="518.2" y="493" widt/;"	i
SVGID_00000022558619016338996610000014232092862130105737_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000022558619016338996610000014232092862130105737_">$/;"	i
SVGID_00000023249018180448339770000003930921894561446832_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000023249018180448339770000003930921894561446832_" x="518.2" y="493" widt/;"	d
SVGID_00000023249018180448339770000003930921894561446832_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000023249018180448339770000003930921894561446832_" x="518.2" y="493" widt/;"	i
SVGID_00000025406153955556018680000013955059386859013023_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000025406153955556018680000013955059386859013023_" x="518.9" y="52.4" wid/;"	d
SVGID_00000025406153955556018680000013955059386859013023_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000025406153955556018680000013955059386859013023_" x="518.9" y="52.4" wid/;"	i
SVGID_00000025409257226209571790000004220297230694940838_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000025409257226209571790000004220297230694940838_">$/;"	i
SVGID_00000026122987972215142590000007947422250482900620_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000026122987972215142590000007947422250482900620_">$/;"	i
SVGID_00000026863289351770131200000017014335542209655682_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000026863289351770131200000017014335542209655682_">$/;"	i
SVGID_00000027590069239273803020000009559425818301028765_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000027590069239273803020000009559425818301028765_">$/;"	i
SVGID_00000027595042576843832700000013776559850954927778_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000027595042576843832700000013776559850954927778_">$/;"	i
SVGID_00000028322381142252320840000002453676626420017550_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000028322381142252320840000002453676626420017550_">$/;"	i
SVGID_00000029004033559706232680000014467564047519786381_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000029004033559706232680000014467564047519786381_" x="62.1" y="493.4" wid/;"	d
SVGID_00000029004033559706232680000014467564047519786381_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000029004033559706232680000014467564047519786381_" x="62.1" y="493.4" wid/;"	i
SVGID_00000029010431564330226110000016928683183128611258_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000029010431564330226110000016928683183128611258_" x="518.9" y="52.4" wid/;"	d
SVGID_00000029010431564330226110000016928683183128611258_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000029010431564330226110000016928683183128611258_" x="518.9" y="52.4" wid/;"	i
SVGID_00000029029156442125040910000000875317355045485226_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000029029156442125040910000000875317355045485226_" x="518.9" y="257.1" wi/;"	d
SVGID_00000029029156442125040910000000875317355045485226_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000029029156442125040910000000875317355045485226_" x="518.9" y="257.1" wi/;"	i
SVGID_00000029737429452937414330000002076649619143601830_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000029737429452937414330000002076649619143601830_">$/;"	i
SVGID_00000029754613902643153650000005966933660853471129_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000029754613902643153650000005966933660853471129_">$/;"	i
SVGID_00000029758560266395173200000006884237633108416896_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000029758560266395173200000006884237633108416896_">$/;"	i
SVGID_00000030446071131310578610000006775448281766015150_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000030446071131310578610000006775448281766015150_" x="518.2" y="493" widt/;"	d
SVGID_00000030446071131310578610000006775448281766015150_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000030446071131310578610000006775448281766015150_" x="518.2" y="493" widt/;"	i
SVGID_00000030482307578111711990000002015932958505759422_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000030482307578111711990000002015932958505759422_">$/;"	i
SVGID_00000031209794053344138350000002020207625793685926_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000031209794053344138350000002020207625793685926_">$/;"	i
SVGID_00000031886342287604040350000002865146713643578018_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000031886342287604040350000002865146713643578018_" x="518.9" y="257.1" wi/;"	d
SVGID_00000031886342287604040350000002865146713643578018_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000031886342287604040350000002865146713643578018_" x="518.9" y="257.1" wi/;"	i
SVGID_00000031909177700253756590000002071129317614755001_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000031909177700253756590000002071129317614755001_" x="62.4" y="51.4" widt/;"	d
SVGID_00000031909177700253756590000002071129317614755001_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000031909177700253756590000002071129317614755001_" x="62.4" y="51.4" widt/;"	i
SVGID_00000031915499903332921950000012423737319708034206_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000031915499903332921950000012423737319708034206_" x="62.4" y="51.4" widt/;"	d
SVGID_00000031915499903332921950000012423737319708034206_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000031915499903332921950000012423737319708034206_" x="62.4" y="51.4" widt/;"	i
SVGID_00000032621950100377214160000014348090687249856385_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000032621950100377214160000014348090687249856385_" x="518.9" y="52.4" wid/;"	d
SVGID_00000032621950100377214160000014348090687249856385_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000032621950100377214160000014348090687249856385_" x="518.9" y="52.4" wid/;"	i
SVGID_00000032635612416860777010000012312376181463843494_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000032635612416860777010000012312376181463843494_">$/;"	i
SVGID_00000033367394737268997470000013851479229372776597_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000033367394737268997470000013851479229372776597_" x="518.9" y="257.1" wi/;"	d
SVGID_00000033367394737268997470000013851479229372776597_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000033367394737268997470000013851479229372776597_" x="518.9" y="257.1" wi/;"	i
SVGID_00000034775916705328280260000010025631816961490567_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000034775916705328280260000010025631816961490567_" x="62.1" y="493.4" wid/;"	d
SVGID_00000034775916705328280260000010025631816961490567_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000034775916705328280260000010025631816961490567_" x="62.1" y="493.4" wid/;"	i
SVGID_00000034797008402958681140000013883770311767648139_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000034797008402958681140000013883770311767648139_" x="62.1" y="493.4" wid/;"	d
SVGID_00000034797008402958681140000013883770311767648139_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000034797008402958681140000013883770311767648139_" x="62.1" y="493.4" wid/;"	i
SVGID_00000035514485474289200120000010171327465431029126_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000035514485474289200120000010171327465431029126_">$/;"	i
SVGID_00000036247092873976579320000017032174770108024453_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000036247092873976579320000017032174770108024453_">$/;"	i
SVGID_00000038392714553711721480000016821597016071621265_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000038392714553711721480000016821597016071621265_">$/;"	i
SVGID_00000038397041605504458130000007422171460219248063_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000038397041605504458130000007422171460219248063_" x="62.4" y="51.4" widt/;"	d
SVGID_00000038397041605504458130000007422171460219248063_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000038397041605504458130000007422171460219248063_" x="62.4" y="51.4" widt/;"	i
SVGID_00000039135675251853230930000011195168626807930545_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000039135675251853230930000011195168626807930545_">$/;"	i
SVGID_00000039840904486396737060000006633079094325817002_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000039840904486396737060000006633079094325817002_">$/;"	i
SVGID_00000039853104085318159380000016838995201029287580_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000039853104085318159380000016838995201029287580_">$/;"	i
SVGID_00000040539272115032682790000007967581420289223564_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000040539272115032682790000007967581420289223564_">$/;"	i
SVGID_00000041256540259209755300000002797201962061433994_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000041256540259209755300000002797201962061433994_" x="518.9" y="52.4" wid/;"	d
SVGID_00000041256540259209755300000002797201962061433994_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000041256540259209755300000002797201962061433994_" x="518.9" y="52.4" wid/;"	i
SVGID_00000041274529303194746070000014525795903669846423_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000041274529303194746070000014525795903669846423_" x="518.9" y="257.1" wi/;"	d
SVGID_00000041274529303194746070000014525795903669846423_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000041274529303194746070000014525795903669846423_" x="518.9" y="257.1" wi/;"	i
SVGID_00000041289295220639795930000014193164088617141911_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000041289295220639795930000014193164088617141911_">$/;"	i
SVGID_00000042696181878571151380000010590901671589970057_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000042696181878571151380000010590901671589970057_">$/;"	i
SVGID_00000042731776168878880880000012933177106469664136_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000042731776168878880880000012933177106469664136_" x="62.4" y="257.1" wid/;"	d
SVGID_00000042731776168878880880000012933177106469664136_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000042731776168878880880000012933177106469664136_" x="62.4" y="257.1" wid/;"	i
SVGID_00000044178978788579857620000009072259264494322318_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000044178978788579857620000009072259264494322318_">$/;"	i
SVGID_00000046307748240302838290000013992525440293411210_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000046307748240302838290000013992525440293411210_">$/;"	i
SVGID_00000047756690678077948900000004887991122846361534_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000047756690678077948900000004887991122846361534_">$/;"	i
SVGID_00000048469503859161993820000002722478436589636280_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000048469503859161993820000002722478436589636280_" x="62.4" y="257.1" wid/;"	d
SVGID_00000048469503859161993820000002722478436589636280_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000048469503859161993820000002722478436589636280_" x="62.4" y="257.1" wid/;"	i
SVGID_00000048484885061789498260000008569226749072227721_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000048484885061789498260000008569226749072227721_">$/;"	i
SVGID_00000049937861384507189130000002076013526895059878_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000049937861384507189130000002076013526895059878_">$/;"	i
SVGID_00000050642792070896778090000009624196685654669246_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000050642792070896778090000009624196685654669246_">$/;"	i
SVGID_00000050644940142332307680000002176907977547205527_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000050644940142332307680000002176907977547205527_">$/;"	i
SVGID_00000050646662689429511360000016960143706660175286_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000050646662689429511360000016960143706660175286_">$/;"	i
SVGID_00000050654760574633121410000003696107655515932606_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000050654760574633121410000003696107655515932606_">$/;"	i
SVGID_00000052065295784515778840000016052983535016214684_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000052065295784515778840000016052983535016214684_">$/;"	i
SVGID_00000052102719550622334960000018196234903834245507_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000052102719550622334960000018196234903834245507_" x="62.4" y="51.4" widt/;"	d
SVGID_00000052102719550622334960000018196234903834245507_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000052102719550622334960000018196234903834245507_" x="62.4" y="51.4" widt/;"	i
SVGID_00000052790341484210342390000006149485985518630299_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000052790341484210342390000006149485985518630299_" x="62.4" y="51.4" widt/;"	d
SVGID_00000052790341484210342390000006149485985518630299_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000052790341484210342390000006149485985518630299_" x="62.4" y="51.4" widt/;"	i
SVGID_00000052804075892968792210000006065035944572581820_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000052804075892968792210000006065035944572581820_" x="62.4" y="257.1" wid/;"	d
SVGID_00000052804075892968792210000006065035944572581820_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000052804075892968792210000006065035944572581820_" x="62.4" y="257.1" wid/;"	i
SVGID_00000053539727951076990730000006160195282588193952_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000053539727951076990730000006160195282588193952_">$/;"	i
SVGID_00000053540000524746393030000009381772575223768750_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000053540000524746393030000009381772575223768750_">$/;"	i
SVGID_00000053541612615457537170000009705209988365433782_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000053541612615457537170000009705209988365433782_">$/;"	i
SVGID_00000054236320117991524180000000727713967104683925_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000054236320117991524180000000727713967104683925_">$/;"	i
SVGID_00000054237549933704207630000002196172257279379643_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000054237549933704207630000002196172257279379643_">$/;"	i
SVGID_00000054241947843305373620000017359221428141349292_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000054241947843305373620000017359221428141349292_" x="62.4" y="51.4" widt/;"	d
SVGID_00000054241947843305373620000017359221428141349292_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000054241947843305373620000017359221428141349292_" x="62.4" y="51.4" widt/;"	i
SVGID_00000054983119321710574000000001186409446777922486_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000054983119321710574000000001186409446777922486_" x="518.2" y="493" widt/;"	d
SVGID_00000054983119321710574000000001186409446777922486_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000054983119321710574000000001186409446777922486_" x="518.2" y="493" widt/;"	i
SVGID_00000057122040716662282820000004882187360591867803_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000057122040716662282820000004882187360591867803_" x="518.2" y="493" widt/;"	d
SVGID_00000057122040716662282820000004882187360591867803_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000057122040716662282820000004882187360591867803_" x="518.2" y="493" widt/;"	i
SVGID_00000057141520434405635620000015312127604356843947_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000057141520434405635620000015312127604356843947_" x="518.9" y="257.1" wi/;"	d
SVGID_00000057141520434405635620000015312127604356843947_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000057141520434405635620000015312127604356843947_" x="518.9" y="257.1" wi/;"	i
SVGID_00000057145166601901628810000010424241125950858896_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000057145166601901628810000010424241125950858896_">$/;"	i
SVGID_00000057827825117575700630000007886388688362138542_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000057827825117575700630000007886388688362138542_" x="62.4" y="51.4" widt/;"	d
SVGID_00000057827825117575700630000007886388688362138542_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000057827825117575700630000007886388688362138542_" x="62.4" y="51.4" widt/;"	i
SVGID_00000057853272517858717040000010443461099091698577_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000057853272517858717040000010443461099091698577_">$/;"	i
SVGID_00000060015953991236912230000006016046639238901428_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000060015953991236912230000006016046639238901428_" x="518.9" y="52.4" wid/;"	d
SVGID_00000060015953991236912230000006016046639238901428_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000060015953991236912230000006016046639238901428_" x="518.9" y="52.4" wid/;"	i
SVGID_00000060027278497638102450000010709768004959525540_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000060027278497638102450000010709768004959525540_">$/;"	i
SVGID_00000060708816353654902670000008163140542919357102_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000060708816353654902670000008163140542919357102_">$/;"	i
SVGID_00000060750058479217716360000001312173477399617940_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000060750058479217716360000001312173477399617940_">$/;"	i
SVGID_00000061449207166971145030000014275357539787309732_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000061449207166971145030000014275357539787309732_" x="518.9" y="257.1" wi/;"	d
SVGID_00000061449207166971145030000014275357539787309732_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000061449207166971145030000014275357539787309732_" x="518.9" y="257.1" wi/;"	i
SVGID_00000063619815244122606700000006130969371606442644_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000063619815244122606700000006130969371606442644_" x="62.1" y="493.4" wid/;"	d
SVGID_00000063619815244122606700000006130969371606442644_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000063619815244122606700000006130969371606442644_" x="62.1" y="493.4" wid/;"	i
SVGID_00000065044846692365479160000017890609946601836434_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000065044846692365479160000017890609946601836434_" x="518.9" y="52.4" wid/;"	d
SVGID_00000065044846692365479160000017890609946601836434_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000065044846692365479160000017890609946601836434_" x="518.9" y="52.4" wid/;"	i
SVGID_00000067234831833496640980000008476344382705028996_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000067234831833496640980000008476344382705028996_">$/;"	i
SVGID_00000067947873181987977190000016841132816507595185_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000067947873181987977190000016841132816507595185_">$/;"	i
SVGID_00000068673846260506023460000006551360980010951856_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000068673846260506023460000006551360980010951856_" x="518.9" y="52.4" wid/;"	d
SVGID_00000068673846260506023460000006551360980010951856_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000068673846260506023460000006551360980010951856_" x="518.9" y="52.4" wid/;"	i
SVGID_00000068674893341147839210000018281483382997822897_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000068674893341147839210000018281483382997822897_" x="62.4" y="51.4" widt/;"	d
SVGID_00000068674893341147839210000018281483382997822897_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000068674893341147839210000018281483382997822897_" x="62.4" y="51.4" widt/;"	i
SVGID_00000069386430022253303380000014502980693445414054_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000069386430022253303380000014502980693445414054_">$/;"	i
SVGID_00000069397872715864894810000009843864366818712738_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000069397872715864894810000009843864366818712738_" x="62.4" y="51.4" widt/;"	d
SVGID_00000069397872715864894810000009843864366818712738_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000069397872715864894810000009843864366818712738_" x="62.4" y="51.4" widt/;"	i
SVGID_00000070816889165657918060000004637795590813732771_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000070816889165657918060000004637795590813732771_" x="522.2" y="446.1" wi/;"	d
SVGID_00000070816889165657918060000004637795590813732771_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000070816889165657918060000004637795590813732771_" x="522.2" y="446.1" wi/;"	i
SVGID_00000070839741462874578230000006277870396752783256_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000070839741462874578230000006277870396752783256_" x="518.2" y="493" widt/;"	d
SVGID_00000070839741462874578230000006277870396752783256_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000070839741462874578230000006277870396752783256_" x="518.2" y="493" widt/;"	i
SVGID_00000070840475676944271280000005573062118323243925_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000070840475676944271280000005573062118323243925_">$/;"	i
SVGID_00000071517470304293448840000002704407558823240881_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000071517470304293448840000002704407558823240881_" x="518.9" y="257.1" wi/;"	d
SVGID_00000071517470304293448840000002704407558823240881_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000071517470304293448840000002704407558823240881_" x="518.9" y="257.1" wi/;"	i
SVGID_00000071546749717535050270000017258336239459058048_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000071546749717535050270000017258336239459058048_" x="518.9" y="257.1" wi/;"	d
SVGID_00000071546749717535050270000017258336239459058048_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000071546749717535050270000017258336239459058048_" x="518.9" y="257.1" wi/;"	i
SVGID_00000073696817167784026490000017867253013931704449_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000073696817167784026490000017867253013931704449_">$/;"	i
SVGID_00000073700410695294383360000003591400264687850924_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000073700410695294383360000003591400264687850924_">$/;"	i
SVGID_00000073721405706032831740000010610840541962391698_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000073721405706032831740000010610840541962391698_" x="62.1" y="493.4" wid/;"	d
SVGID_00000073721405706032831740000010610840541962391698_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000073721405706032831740000010610840541962391698_" x="62.1" y="493.4" wid/;"	i
SVGID_00000075126445619205289630000000844966432716723072_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000075126445619205289630000000844966432716723072_" x="62.4" y="257.1" wid/;"	d
SVGID_00000075126445619205289630000000844966432716723072_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000075126445619205289630000000844966432716723072_" x="62.4" y="257.1" wid/;"	i
SVGID_00000075137493729715026660000004200777858021912242_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000075137493729715026660000004200777858021912242_">$/;"	i
SVGID_00000077286580201766794910000007156856626970333878_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000077286580201766794910000007156856626970333878_">$/;"	i
SVGID_00000078004805635637107520000003473447843170887048_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000078004805635637107520000003473447843170887048_">$/;"	i
SVGID_00000079460534386428201820000006360838433639041442_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000079460534386428201820000006360838433639041442_" x="518.9" y="52.4" wid/;"	d
SVGID_00000079460534386428201820000006360838433639041442_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000079460534386428201820000006360838433639041442_" x="518.9" y="52.4" wid/;"	i
SVGID_00000080886729446832905280000013075230983408558508_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000080886729446832905280000013075230983408558508_" x="62.4" y="257.1" wid/;"	d
SVGID_00000080886729446832905280000013075230983408558508_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000080886729446832905280000013075230983408558508_" x="62.4" y="257.1" wid/;"	i
SVGID_00000080890932939331951820000004955766037990749072_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000080890932939331951820000004955766037990749072_" x="518.2" y="493" widt/;"	d
SVGID_00000080890932939331951820000004955766037990749072_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000080890932939331951820000004955766037990749072_" x="518.2" y="493" widt/;"	i
SVGID_00000080898214430183166600000012679202586299311772_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000080898214430183166600000012679202586299311772_">$/;"	i
SVGID_00000080915161492052818090000001464101742701617064_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000080915161492052818090000001464101742701617064_" x="518.9" y="52.4" wid/;"	d
SVGID_00000080915161492052818090000001464101742701617064_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000080915161492052818090000001464101742701617064_" x="518.9" y="52.4" wid/;"	i
SVGID_00000081615731846670846720000002598025231220288185_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000081615731846670846720000002598025231220288185_">$/;"	i
SVGID_00000081627235572079281450000013762279434456424344_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000081627235572079281450000013762279434456424344_" x="518.9" y="52.4" wid/;"	d
SVGID_00000081627235572079281450000013762279434456424344_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000081627235572079281450000013762279434456424344_" x="518.9" y="52.4" wid/;"	i
SVGID_00000081649682775292393710000017187405065058336170_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000081649682775292393710000017187405065058336170_">$/;"	i
SVGID_00000083046972440966411370000011740130287929459352_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000083046972440966411370000011740130287929459352_" x="518.2" y="493" widt/;"	d
SVGID_00000083046972440966411370000011740130287929459352_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000083046972440966411370000011740130287929459352_" x="518.2" y="493" widt/;"	i
SVGID_00000083795918035859638970000005951152818991530917_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000083795918035859638970000005951152818991530917_" x="518.9" y="257.1" wi/;"	d
SVGID_00000083795918035859638970000005951152818991530917_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000083795918035859638970000005951152818991530917_" x="518.9" y="257.1" wi/;"	i
SVGID_00000084494906429034316860000010555516676115722938_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000084494906429034316860000010555516676115722938_">$/;"	i
SVGID_00000086656510920743487460000014380013931080627376_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000086656510920743487460000014380013931080627376_" x="62.4" y="257.1" wid/;"	d
SVGID_00000086656510920743487460000014380013931080627376_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000086656510920743487460000014380013931080627376_" x="62.4" y="257.1" wid/;"	i
SVGID_00000086659529586615223840000001096171815689174438_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000086659529586615223840000001096171815689174438_" x="62.4" y="257.1" wid/;"	d
SVGID_00000086659529586615223840000001096171815689174438_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000086659529586615223840000001096171815689174438_" x="62.4" y="257.1" wid/;"	i
SVGID_00000086663580441253275650000003051001442294579631_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000086663580441253275650000003051001442294579631_" x="62.4" y="257.1" wid/;"	d
SVGID_00000086663580441253275650000003051001442294579631_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000086663580441253275650000003051001442294579631_" x="62.4" y="257.1" wid/;"	i
SVGID_00000086689413198506228420000001072277910557616260_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000086689413198506228420000001072277910557616260_">$/;"	i
SVGID_00000087384564297013253590000018422822758310512563_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000087384564297013253590000018422822758310512563_">$/;"	i
SVGID_00000087385122243603814880000010724394403219991718_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000087385122243603814880000010724394403219991718_">$/;"	i
SVGID_00000087393662235936905860000002070477915684303769_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000087393662235936905860000002070477915684303769_">$/;"	i
SVGID_00000088114057994070835930000000934184857105511829_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000088114057994070835930000000934184857105511829_" x="518.9" y="257.1" wi/;"	d
SVGID_00000088114057994070835930000000934184857105511829_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000088114057994070835930000000934184857105511829_" x="518.9" y="257.1" wi/;"	i
SVGID_00000090988536419419039450000005710549119370370487_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000090988536419419039450000005710549119370370487_">$/;"	i
SVGID_00000091006435822590514140000010290999656939124103_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000091006435822590514140000010290999656939124103_" x="62.4" y="257.1" wid/;"	d
SVGID_00000091006435822590514140000010290999656939124103_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000091006435822590514140000010290999656939124103_" x="62.4" y="257.1" wid/;"	i
SVGID_00000091734877654441927810000004896794007924952735_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000091734877654441927810000004896794007924952735_">$/;"	i
SVGID_00000092428928142810046750000012191397861223705523_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000092428928142810046750000012191397861223705523_" x="522.2" y="446.1" wi/;"	d
SVGID_00000092428928142810046750000012191397861223705523_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000092428928142810046750000012191397861223705523_" x="522.2" y="446.1" wi/;"	i
SVGID_00000093151651131053245630000006555229434223496862_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000093151651131053245630000006555229434223496862_">$/;"	i
SVGID_00000093168939675750065960000012426566289132365961_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000093168939675750065960000012426566289132365961_" x="62.1" y="493.4" wid/;"	d
SVGID_00000093168939675750065960000012426566289132365961_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000093168939675750065960000012426566289132365961_" x="62.1" y="493.4" wid/;"	i
SVGID_00000093871654253318951000000004328918295119064454_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000093871654253318951000000004328918295119064454_">$/;"	i
SVGID_00000094596923266001150830000011207480430933302192_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000094596923266001150830000011207480430933302192_" x="518.9" y="52.4" wid/;"	d
SVGID_00000094596923266001150830000011207480430933302192_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000094596923266001150830000011207480430933302192_" x="518.9" y="52.4" wid/;"	i
SVGID_00000096764303591451694880000011169946816339784326_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000096764303591451694880000011169946816339784326_" x="518.9" y="52.4" wid/;"	d
SVGID_00000096764303591451694880000011169946816339784326_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000096764303591451694880000011169946816339784326_" x="518.9" y="52.4" wid/;"	i
SVGID_00000098902829507873966740000017652703409283181246_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000098902829507873966740000017652703409283181246_" x="62.1" y="493.4" wid/;"	d
SVGID_00000098902829507873966740000017652703409283181246_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000098902829507873966740000017652703409283181246_" x="62.1" y="493.4" wid/;"	i
SVGID_00000098903731636651917410000005585708155479466628_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000098903731636651917410000005585708155479466628_" x="518.9" y="52.4" wid/;"	d
SVGID_00000098903731636651917410000005585708155479466628_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000098903731636651917410000005585708155479466628_" x="518.9" y="52.4" wid/;"	i
SVGID_00000099634805363155443380000007565810252499652256_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000099634805363155443380000007565810252499652256_">$/;"	i
SVGID_00000099655085577151702080000011704302365633382275_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000099655085577151702080000011704302365633382275_" x="62.4" y="257.1" wid/;"	d
SVGID_00000099655085577151702080000011704302365633382275_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000099655085577151702080000011704302365633382275_" x="62.4" y="257.1" wid/;"	i
SVGID_00000100342819446092373910000004730980741151493310_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000100342819446092373910000004730980741151493310_">$/;"	i
SVGID_00000101084752533161235080000014374377528759247244_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000101084752533161235080000014374377528759247244_">$/;"	i
SVGID_00000101087818292300198000000009514728755290371216_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000101087818292300198000000009514728755290371216_" x="62.4" y="257.1" wid/;"	d
SVGID_00000101087818292300198000000009514728755290371216_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000101087818292300198000000009514728755290371216_" x="62.4" y="257.1" wid/;"	i
SVGID_00000101092859517635110140000000352372182101361593_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000101092859517635110140000000352372182101361593_">$/;"	i
SVGID_00000103243896393753129090000012174130195615436185_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000103243896393753129090000012174130195615436185_">$/;"	i
SVGID_00000104698785662254544400000004111871117065202354_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000104698785662254544400000004111871117065202354_">$/;"	i
SVGID_00000105391080664004596980000009717580251810554282_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000105391080664004596980000009717580251810554282_" x="62.4" y="257.1" wid/;"	d
SVGID_00000105391080664004596980000009717580251810554282_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000105391080664004596980000009717580251810554282_" x="62.4" y="257.1" wid/;"	i
SVGID_00000106122457475747482720000018008974168489252240_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000106122457475747482720000018008974168489252240_">$/;"	i
SVGID_00000106856388081190993400000004811746071988928913_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000106856388081190993400000004811746071988928913_">$/;"	i
SVGID_00000109030285824928534020000009852662850602874496_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000109030285824928534020000009852662850602874496_">$/;"	i
SVGID_00000111166570444521478790000007894061743637013413_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000111166570444521478790000007894061743637013413_" x="518.2" y="493" widt/;"	d
SVGID_00000111166570444521478790000007894061743637013413_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000111166570444521478790000007894061743637013413_" x="518.2" y="493" widt/;"	i
SVGID_00000112618511551420158410000006467962690093268104_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000112618511551420158410000006467962690093268104_" x="518.2" y="493" widt/;"	d
SVGID_00000112618511551420158410000006467962690093268104_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000112618511551420158410000006467962690093268104_" x="518.2" y="493" widt/;"	i
SVGID_00000114037210324814389480000007941749095363218587_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000114037210324814389480000007941749095363218587_" x="518.9" y="52.4" wid/;"	d
SVGID_00000114037210324814389480000007941749095363218587_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000114037210324814389480000007941749095363218587_" x="518.9" y="52.4" wid/;"	i
SVGID_00000114072918673026555510000016111316623333900689_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000114072918673026555510000016111316623333900689_">$/;"	i
SVGID_00000114758793451911256190000017163200193116200875_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000114758793451911256190000017163200193116200875_" x="62.4" y="51.4" widt/;"	d
SVGID_00000114758793451911256190000017163200193116200875_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000114758793451911256190000017163200193116200875_" x="62.4" y="51.4" widt/;"	i
SVGID_00000114782277392111916920000008095249763532997023_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000114782277392111916920000008095249763532997023_">$/;"	i
SVGID_00000115497919965859708430000005086620069298652800_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000115497919965859708430000005086620069298652800_">$/;"	i
SVGID_00000116955431306409296580000002467081015158050432_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000116955431306409296580000002467081015158050432_" x="518.2" y="493" widt/;"	d
SVGID_00000116955431306409296580000002467081015158050432_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000116955431306409296580000002467081015158050432_" x="518.2" y="493" widt/;"	i
SVGID_00000122711995888386590870000011283995862277928607_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000122711995888386590870000011283995862277928607_">$/;"	i
SVGID_00000123414776343525443310000009457246115990876565_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000123414776343525443310000009457246115990876565_">$/;"	i
SVGID_00000123433503841107169930000013306089293144108222_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000123433503841107169930000013306089293144108222_" x="518.9" y="257.1" wi/;"	d
SVGID_00000123433503841107169930000013306089293144108222_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000123433503841107169930000013306089293144108222_" x="518.9" y="257.1" wi/;"	i
SVGID_00000125586938658290945110000016393455337647009430_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000125586938658290945110000016393455337647009430_">$/;"	i
SVGID_00000126305942959185254960000002042081895005127614_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000126305942959185254960000002042081895005127614_" x="522.2" y="446.1" wi/;"	d
SVGID_00000126305942959185254960000002042081895005127614_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000126305942959185254960000002042081895005127614_" x="522.2" y="446.1" wi/;"	i
SVGID_00000129909873285364430180000013538356140005750944_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000129909873285364430180000013538356140005750944_" x="62.1" y="493.4" wid/;"	d
SVGID_00000129909873285364430180000013538356140005750944_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000129909873285364430180000013538356140005750944_" x="62.1" y="493.4" wid/;"	i
SVGID_00000129916039770227943520000007099006823084956567_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000129916039770227943520000007099006823084956567_">$/;"	i
SVGID_00000130618020947747880340000016142955599757828023_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000130618020947747880340000016142955599757828023_" x="62.4" y="257.1" wid/;"	d
SVGID_00000130618020947747880340000016142955599757828023_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000130618020947747880340000016142955599757828023_" x="62.4" y="257.1" wid/;"	i
SVGID_00000131329148749913972300000017055217003075129743_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000131329148749913972300000017055217003075129743_">$/;"	i
SVGID_00000132088175946793857670000005302175634685524892_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000132088175946793857670000005302175634685524892_" x="522.2" y="446.1" wi/;"	d
SVGID_00000132088175946793857670000005302175634685524892_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000132088175946793857670000005302175634685524892_" x="522.2" y="446.1" wi/;"	i
SVGID_00000132784284869007904100000012662136788845394069_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000132784284869007904100000012662136788845394069_" x="62.4" y="257.1" wid/;"	d
SVGID_00000132784284869007904100000012662136788845394069_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000132784284869007904100000012662136788845394069_" x="62.4" y="257.1" wid/;"	i
SVGID_00000133503127921723751380000010799617372920376735_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000133503127921723751380000010799617372920376735_" x="62.1" y="493.4" wid/;"	d
SVGID_00000133503127921723751380000010799617372920376735_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000133503127921723751380000010799617372920376735_" x="62.1" y="493.4" wid/;"	i
SVGID_00000133511093886426784180000006144821694577495480_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000133511093886426784180000006144821694577495480_">$/;"	i
SVGID_00000134960799800778975390000016886352082611991429_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000134960799800778975390000016886352082611991429_" x="518.2" y="493" widt/;"	d
SVGID_00000134960799800778975390000016886352082611991429_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000134960799800778975390000016886352082611991429_" x="518.2" y="493" widt/;"	i
SVGID_00000135653007709115924060000006668060846381662628_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000135653007709115924060000006668060846381662628_" x="62.1" y="493.4" wid/;"	d
SVGID_00000135653007709115924060000006668060846381662628_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000135653007709115924060000006668060846381662628_" x="62.1" y="493.4" wid/;"	i
SVGID_00000135687839860289246310000009465024950333685646_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000135687839860289246310000009465024950333685646_">$/;"	i
SVGID_00000136381502193294109250000001448087217408861827_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000136381502193294109250000001448087217408861827_">$/;"	i
SVGID_00000136396311993549388360000001124227475262044054_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000136396311993549388360000001124227475262044054_" x="62.4" y="257.1" wid/;"	d
SVGID_00000136396311993549388360000001124227475262044054_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000136396311993549388360000001124227475262044054_" x="62.4" y="257.1" wid/;"	i
SVGID_00000137129759188563244470000014098421984483242155_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000137129759188563244470000014098421984483242155_" x="62.4" y="51.4" widt/;"	d
SVGID_00000137129759188563244470000014098421984483242155_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000137129759188563244470000014098421984483242155_" x="62.4" y="51.4" widt/;"	i
SVGID_00000138538739470269519190000008612017215200327305_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000138538739470269519190000008612017215200327305_">$/;"	i
SVGID_00000138552142634443450090000012453546088451541403_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000138552142634443450090000012453546088451541403_" x="518.2" y="493" widt/;"	d
SVGID_00000138552142634443450090000012453546088451541403_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000138552142634443450090000012453546088451541403_" x="518.2" y="493" widt/;"	i
SVGID_00000140000684321229582360000008034951756628254856_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000140000684321229582360000008034951756628254856_">$/;"	i
SVGID_00000140698190662278380000000011344913997245640073_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000140698190662278380000000011344913997245640073_">$/;"	i
SVGID_00000140718625456317189550000010374422196947058876_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000140718625456317189550000010374422196947058876_" x="522.2" y="446.1" wi/;"	d
SVGID_00000140718625456317189550000010374422196947058876_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000140718625456317189550000010374422196947058876_" x="522.2" y="446.1" wi/;"	i
SVGID_00000140725040879718645760000007625666813827103934_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000140725040879718645760000007625666813827103934_" x="522.2" y="446.1" wi/;"	d
SVGID_00000140725040879718645760000007625666813827103934_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000140725040879718645760000007625666813827103934_" x="522.2" y="446.1" wi/;"	i
SVGID_00000142162477803911097850000008248515882113598903_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000142162477803911097850000008248515882113598903_">$/;"	i
SVGID_00000143590596850377348920000011380354039080571522_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000143590596850377348920000011380354039080571522_" x="62.4" y="51.4" widt/;"	d
SVGID_00000143590596850377348920000011380354039080571522_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000143590596850377348920000011380354039080571522_" x="62.4" y="51.4" widt/;"	i
SVGID_00000144303788410411558650000007895786757390886566_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000144303788410411558650000007895786757390886566_">$/;"	i
SVGID_00000145765929425866127300000000124297669311126159_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000145765929425866127300000000124297669311126159_">$/;"	i
SVGID_00000146493205004141360970000008824025253132962726_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000146493205004141360970000008824025253132962726_" x="518.9" y="52.4" wid/;"	d
SVGID_00000146493205004141360970000008824025253132962726_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000146493205004141360970000008824025253132962726_" x="518.9" y="52.4" wid/;"	i
SVGID_00000146499940594546000930000014205193774671458986_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000146499940594546000930000014205193774671458986_" x="518.9" y="52.4" wid/;"	d
SVGID_00000146499940594546000930000014205193774671458986_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000146499940594546000930000014205193774671458986_" x="518.9" y="52.4" wid/;"	i
SVGID_00000147206824710151206680000015508203279650094723_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000147206824710151206680000015508203279650094723_" x="522.2" y="446.1" wi/;"	d
SVGID_00000147206824710151206680000015508203279650094723_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000147206824710151206680000015508203279650094723_" x="522.2" y="446.1" wi/;"	i
SVGID_00000148657594842620063840000002303898214992786348_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000148657594842620063840000002303898214992786348_" x="62.1" y="493.4" wid/;"	d
SVGID_00000148657594842620063840000002303898214992786348_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000148657594842620063840000002303898214992786348_" x="62.1" y="493.4" wid/;"	i
SVGID_00000150789276323894406250000015546971250011987345_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000150789276323894406250000015546971250011987345_" x="62.1" y="493.4" wid/;"	d
SVGID_00000150789276323894406250000015546971250011987345_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000150789276323894406250000015546971250011987345_" x="62.1" y="493.4" wid/;"	i
SVGID_00000150802076654782140820000010303687186294497675_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000150802076654782140820000010303687186294497675_">$/;"	i
SVGID_00000151523771188303232710000017175401597829634693_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000151523771188303232710000017175401597829634693_">$/;"	i
SVGID_00000151542784491752250310000004750917121981646996_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000151542784491752250310000004750917121981646996_">$/;"	i
SVGID_00000152221820857865502880000011034105152858595757_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000152221820857865502880000011034105152858595757_">$/;"	i
SVGID_00000152239984874194368140000001299422974532127639_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000152239984874194368140000001299422974532127639_">$/;"	i
SVGID_00000152981692412391762160000015454470341501276320_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000152981692412391762160000015454470341501276320_">$/;"	i
SVGID_00000155828919843606950570000015969110452672513671_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000155828919843606950570000015969110452672513671_" x="518.9" y="257.1" wi/;"	d
SVGID_00000155828919843606950570000015969110452672513671_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000155828919843606950570000015969110452672513671_" x="518.9" y="257.1" wi/;"	i
SVGID_00000157302962731587975030000000358811706345985674_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000157302962731587975030000000358811706345985674_" x="62.4" y="51.4" widt/;"	d
SVGID_00000157302962731587975030000000358811706345985674_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000157302962731587975030000000358811706345985674_" x="62.4" y="51.4" widt/;"	i
SVGID_00000158023662163790439310000008282534772020272534_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000158023662163790439310000008282534772020272534_">$/;"	i
SVGID_00000158027923218653781590000015528189041273312896_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000158027923218653781590000015528189041273312896_">$/;"	i
SVGID_00000158719590360807481550000012140678827991217570_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000158719590360807481550000012140678827991217570_">$/;"	i
SVGID_00000158739335860590570820000009672263336232263554_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000158739335860590570820000009672263336232263554_">$/;"	i
SVGID_00000158748284081864722930000014464011618130033576_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000158748284081864722930000014464011618130033576_" x="62.1" y="493.4" wid/;"	d
SVGID_00000158748284081864722930000014464011618130033576_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000158748284081864722930000014464011618130033576_" x="62.1" y="493.4" wid/;"	i
SVGID_00000159451159607342841190000010643370508511930285_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000159451159607342841190000010643370508511930285_" x="62.1" y="493.4" wid/;"	d
SVGID_00000159451159607342841190000010643370508511930285_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000159451159607342841190000010643370508511930285_" x="62.1" y="493.4" wid/;"	i
SVGID_00000159465151633005412810000013209302716460413607_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000159465151633005412810000013209302716460413607_" x="518.9" y="257.1" wi/;"	d
SVGID_00000159465151633005412810000013209302716460413607_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000159465151633005412810000013209302716460413607_" x="518.9" y="257.1" wi/;"	i
SVGID_00000160161077671868400540000014971992794150045320_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000160161077671868400540000014971992794150045320_" x="518.9" y="257.1" wi/;"	d
SVGID_00000160161077671868400540000014971992794150045320_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000160161077671868400540000014971992794150045320_" x="518.9" y="257.1" wi/;"	i
SVGID_00000160164737793917518460000005076276915339774367_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000160164737793917518460000005076276915339774367_" x="518.2" y="493" widt/;"	d
SVGID_00000160164737793917518460000005076276915339774367_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000160164737793917518460000005076276915339774367_" x="518.2" y="493" widt/;"	i
SVGID_00000160173443867986926710000003745679552785285547_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000160173443867986926710000003745679552785285547_" x="518.2" y="493" widt/;"	d
SVGID_00000160173443867986926710000003745679552785285547_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000160173443867986926710000003745679552785285547_" x="518.2" y="493" widt/;"	i
SVGID_00000160869373294125422000000013194918097369352079_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000160869373294125422000000013194918097369352079_">$/;"	i
SVGID_00000162314872462842226820000005169559670752060589_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000162314872462842226820000005169559670752060589_" x="62.4" y="51.4" widt/;"	d
SVGID_00000162314872462842226820000005169559670752060589_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000162314872462842226820000005169559670752060589_" x="62.4" y="51.4" widt/;"	i
SVGID_00000162334930557948963460000011989030596088240531_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000162334930557948963460000011989030596088240531_" x="62.4" y="257.1" wid/;"	d
SVGID_00000162334930557948963460000011989030596088240531_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000162334930557948963460000011989030596088240531_" x="62.4" y="257.1" wid/;"	i
SVGID_00000163755139582992580470000006459539471379508364_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000163755139582992580470000006459539471379508364_" x="522.2" y="446.1" wi/;"	d
SVGID_00000163755139582992580470000006459539471379508364_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000163755139582992580470000006459539471379508364_" x="522.2" y="446.1" wi/;"	i
SVGID_00000163758059236605777410000017745499082213160623_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000163758059236605777410000017745499082213160623_" x="62.1" y="493.4" wid/;"	d
SVGID_00000163758059236605777410000017745499082213160623_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000163758059236605777410000017745499082213160623_" x="62.1" y="493.4" wid/;"	i
SVGID_00000163759372401468264160000006849697745824756654_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000163759372401468264160000006849697745824756654_" x="522.2" y="446.1" wi/;"	d
SVGID_00000163759372401468264160000006849697745824756654_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000163759372401468264160000006849697745824756654_" x="522.2" y="446.1" wi/;"	i
SVGID_00000163760020706885293370000009242466389293546664_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000163760020706885293370000009242466389293546664_">$/;"	i
SVGID_00000163780010097582948640000004571470443130096054_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000163780010097582948640000004571470443130096054_">$/;"	i
SVGID_00000163787915655414772450000018136717695189814187_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000163787915655414772450000018136717695189814187_" x="518.2" y="493" widt/;"	d
SVGID_00000163787915655414772450000018136717695189814187_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000163787915655414772450000018136717695189814187_" x="518.2" y="493" widt/;"	i
SVGID_00000165193669735338066770000015158863273929569715_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000165193669735338066770000015158863273929569715_" x="518.9" y="257.1" wi/;"	d
SVGID_00000165193669735338066770000015158863273929569715_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000165193669735338066770000015158863273929569715_" x="518.9" y="257.1" wi/;"	i
SVGID_00000165231713648174790450000014120050104577765785_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000165231713648174790450000014120050104577765785_">$/;"	i
SVGID_00000165917231316615544050000014800326615014911650_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000165917231316615544050000014800326615014911650_">$/;"	i
SVGID_00000166636157735529659920000005221233433834227846_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000166636157735529659920000005221233433834227846_" x="522.2" y="446.1" wi/;"	d
SVGID_00000166636157735529659920000005221233433834227846_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000166636157735529659920000005221233433834227846_" x="522.2" y="446.1" wi/;"	i
SVGID_00000167370704161276984810000014225452568330393494_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000167370704161276984810000014225452568330393494_">$/;"	i
SVGID_00000167388326292776131990000001689729312886565820_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000167388326292776131990000001689729312886565820_" x="62.1" y="493.4" wid/;"	d
SVGID_00000167388326292776131990000001689729312886565820_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000167388326292776131990000001689729312886565820_" x="62.1" y="493.4" wid/;"	i
SVGID_00000169530796856144343770000015167719619770549649_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000169530796856144343770000015167719619770549649_">$/;"	i
SVGID_00000169543869227391598750000017090113086764087696_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000169543869227391598750000017090113086764087696_" x="62.1" y="493.4" wid/;"	d
SVGID_00000169543869227391598750000017090113086764087696_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000169543869227391598750000017090113086764087696_" x="62.1" y="493.4" wid/;"	i
SVGID_00000170240776232879088420000000620068104962057364_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000170240776232879088420000000620068104962057364_" x="518.9" y="257.1" wi/;"	d
SVGID_00000170240776232879088420000000620068104962057364_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000170240776232879088420000000620068104962057364_" x="518.9" y="257.1" wi/;"	i
SVGID_00000170259449094773110220000016759249032490895745_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000170259449094773110220000016759249032490895745_" x="62.4" y="257.1" wid/;"	d
SVGID_00000170259449094773110220000016759249032490895745_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000170259449094773110220000016759249032490895745_" x="62.4" y="257.1" wid/;"	i
SVGID_00000170961257040683269020000003729561116279337352_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000170961257040683269020000003729561116279337352_" x="518.2" y="493" widt/;"	d
SVGID_00000170961257040683269020000003729561116279337352_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000170961257040683269020000003729561116279337352_" x="518.2" y="493" widt/;"	i
SVGID_00000172421946126992368820000014911327770157861040_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000172421946126992368820000014911327770157861040_">$/;"	i
SVGID_00000172431387196345489380000013424842921895512461_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000172431387196345489380000013424842921895512461_" x="62.4" y="51.4" widt/;"	d
SVGID_00000172431387196345489380000013424842921895512461_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000172431387196345489380000013424842921895512461_" x="62.4" y="51.4" widt/;"	i
SVGID_00000172435982769747129010000005112477516215756218_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000172435982769747129010000005112477516215756218_">$/;"	i
SVGID_00000173864776440148329380000018121860786442391431_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000173864776440148329380000018121860786442391431_" x="518.9" y="52.4" wid/;"	d
SVGID_00000173864776440148329380000018121860786442391431_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000173864776440148329380000018121860786442391431_" x="518.9" y="52.4" wid/;"	i
SVGID_00000176043041637035782540000007209291143453783433_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000176043041637035782540000007209291143453783433_">$/;"	i
SVGID_00000176726290945420400460000017892882036648998278_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000176726290945420400460000017892882036648998278_">$/;"	i
SVGID_00000176732933468599979800000010149218962007490744_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000176732933468599979800000010149218962007490744_">$/;"	i
SVGID_00000176740595437360469700000012098777397605814966_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000176740595437360469700000012098777397605814966_" x="62.4" y="257.1" wid/;"	d
SVGID_00000176740595437360469700000012098777397605814966_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000176740595437360469700000012098777397605814966_" x="62.4" y="257.1" wid/;"	i
SVGID_00000178168893601199409510000014851069164476710530_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000178168893601199409510000014851069164476710530_">$/;"	i
SVGID_00000178182859620291535270000018025789911502911645_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000178182859620291535270000018025789911502911645_">$/;"	i
SVGID_00000178197063738966448780000013205083071462854839_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000178197063738966448780000013205083071462854839_" x="62.4" y="51.4" widt/;"	d
SVGID_00000178197063738966448780000013205083071462854839_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000178197063738966448780000013205083071462854839_" x="62.4" y="51.4" widt/;"	i
SVGID_00000178206151219142874140000016521245507178700713_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000178206151219142874140000016521245507178700713_" x="62.4" y="51.4" widt/;"	d
SVGID_00000178206151219142874140000016521245507178700713_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000178206151219142874140000016521245507178700713_" x="62.4" y="51.4" widt/;"	i
SVGID_00000178924569187431824280000017555920404825714589_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000178924569187431824280000017555920404825714589_" x="62.4" y="257.1" wid/;"	d
SVGID_00000178924569187431824280000017555920404825714589_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000178924569187431824280000017555920404825714589_" x="62.4" y="257.1" wid/;"	i
SVGID_00000179638806551170565540000002717556461569668996_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000179638806551170565540000002717556461569668996_" x="518.9" y="257.1" wi/;"	d
SVGID_00000179638806551170565540000002717556461569668996_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000179638806551170565540000002717556461569668996_" x="518.9" y="257.1" wi/;"	i
SVGID_00000181062189848787164060000013539598462138583953_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000181062189848787164060000013539598462138583953_">$/;"	i
SVGID_00000183206571739401242990000000105454377430240393_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000183206571739401242990000000105454377430240393_" x="62.1" y="493.4" wid/;"	d
SVGID_00000183206571739401242990000000105454377430240393_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_00000183206571739401242990000000105454377430240393_" x="62.1" y="493.4" wid/;"	i
SVGID_00000183235442214089383580000006427968136308033466_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000183235442214089383580000006427968136308033466_">$/;"	i
SVGID_00000183961624220905880520000014301485943947703957_	figures/combined-sparsity-plots.svg	/^				<clipPath id="SVGID_00000183961624220905880520000014301485943947703957_">$/;"	i
SVGID_1_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_1_" x="518.2" y="493" width="380.5" height="126"\/>$/;"	d
SVGID_1_	figures/combined-sparsity-plots.svg	/^					<rect id="SVGID_1_" x="518.2" y="493" width="380.5" height="126"\/>$/;"	i
VariationalDropout	references.bib	/^@inproceedings{VariationalDropout,$/;"	j
WeightTyingInan	references.bib	/^@inproceedings{WeightTyingInan,$/;"	j
WeightTyingPress	references.bib	/^@inproceedings{WeightTyingPress,$/;"	j
WikiText	references.bib	/^@misc{WikiText,$/;"	n
\\bbR	math-symbols.tex	/^\\newcommand{\\bbR}{\\ensuremath{\\mathbb{R}}}$/;"	C
\\bfJ	math-symbols.tex	/^\\newcommand{\\bfJ}{\\ensuremath{\\mathbf{J}}}$/;"	C
\\bfJt	math-symbols.tex	/^\\newcommand{\\bfJt}{\\ensuremath{\\bfJ\\supt}}$/;"	C
\\bfM	math-symbols.tex	/^\\newcommand{\\bfM}{\\ensuremath{\\mathbf{M}}}$/;"	C
\\bfMt	math-symbols.tex	/^\\newcommand{\\bfMt}{\\ensuremath{\\bfM\\supt}}$/;"	C
\\bfMtm	math-symbols.tex	/^\\newcommand{\\bfMtm}{\\ensuremath{\\bfM\\suptm}}$/;"	C
\\bfU	math-symbols.tex	/^\\newcommand{\\bfU}{\\ensuremath{\\mathbf{U}}}$/;"	C
\\bfV	math-symbols.tex	/^\\newcommand{\\bfV}{\\ensuremath{\\mathbf{V}}}$/;"	C
\\bfW	math-symbols.tex	/^\\newcommand{\\bfW}{\\ensuremath{\\mathbf{W}}}$/;"	C
\\bfa	math-symbols.tex	/^\\newcommand{\\bfa}{\\mathbf{a}}$/;"	C
\\bfalpha	math-symbols.tex	/^\\newcommand{\\bfalpha}{\\boldsymbol{\\alpha}}$/;"	C
\\bfat	math-symbols.tex	/^\\newcommand{\\bfat}{\\ensuremath{\\bfa\\supt}}$/;"	C
\\bfatm	math-symbols.tex	/^\\newcommand{\\bfatm}{\\ensuremath{\\bfa\\suptm}}$/;"	C
\\bfb	math-symbols.tex	/^\\newcommand{\\bfb}{\\ensuremath{\\mathbf{b}}}$/;"	C
\\bfbM	math-symbols.tex	/^\\newcommand{\\bfbM}{\\ensuremath{\\bar{\\mathbf{M}}}}$/;"	C
\\bfbc	math-symbols.tex	/^\\newcommand{\\bfbc}{\\ensuremath{\\bar{\\mathbf{c}}}}$/;"	C
\\bfbct	math-symbols.tex	/^\\newcommand{\\bfbct}{\\ensuremath{\\bfbc\\supt}}$/;"	C
\\bfbeta	math-symbols.tex	/^\\newcommand{\\bfbeta}{\\boldsymbol{\\beta}}$/;"	C
\\bfc	math-symbols.tex	/^\\newcommand{\\bfc}{\\mathbf{c}}$/;"	C
\\bfe	math-symbols.tex	/^\\newcommand{\\bfe}{\\mathbf{e}}$/;"	C
\\bfgamma	math-symbols.tex	/^\\newcommand{\\bfgamma}{\\boldsymbol{\\gamma}}$/;"	C
\\bflambda	math-symbols.tex	/^\\newcommand{\\bflambda}{\\boldsymbol{\\lambda}}$/;"	C
\\bfmu	math-symbols.tex	/^\\newcommand{\\bfmu}{\\boldsymbol{\\mu}}$/;"	C
\\bfo	math-symbols.tex	/^\\newcommand{\\bfo}{\\mathbf{o}}$/;"	C
\\bfr	math-symbols.tex	/^\\newcommand{\\bfr}{\\mathbf{r}}$/;"	C
\\bfs	math-symbols.tex	/^\\newcommand{\\bfs}{\\mathbf{s}}$/;"	C
\\bfth	math-symbols.tex	/^\\newcommand{\\bfth}{\\boldsymbol{\\vartheta}}$/;"	C
\\bfu	math-symbols.tex	/^\\newcommand{\\bfu}{\\mathbf{u}}$/;"	C
\\bfv	math-symbols.tex	/^\\newcommand{\\bfv}{\\ensuremath{\\mathbf{v}}}$/;"	C
\\bfvth	math-symbols.tex	/^\\newcommand{\\bfvth}{\\ensuremath{\\mathbf{\\vartheta}}}$/;"	C
\\bfw	math-symbols.tex	/^\\newcommand{\\bfw}{\\ensuremath{\\mathbf{w}}}$/;"	C
\\bfx	math-symbols.tex	/^\\newcommand{\\bfx}{\\mathbf{x}}$/;"	C
\\bfxi	math-symbols.tex	/^\\newcommand{\\bfxi}{\\boldsymbol{\\xi}}$/;"	C
\\bfy	math-symbols.tex	/^\\newcommand{\\bfy}{\\mathbf{y}}$/;"	C
\\bfz	math-symbols.tex	/^\\newcommand{\\bfz}{\\mathbf{z}}$/;"	C
\\bwrap	math-symbols.tex	/^\\newcommand{\\bwrap}[1]{\\left( #1 \\right)}$/;"	C
\\cL	math-symbols.tex	/^\\newcommand{\\cL}{\\mathcal{L}}$/;"	C
\\cO	math-symbols.tex	/^\\newcommand{\\cO}{\\ensuremath{\\mathcal{O}}}$/;"	C
\\cfun	math-symbols.tex	/^\\newcommand{\\cfun}[3]{\\fun{#1}{ #2 \\,\\middle\\vert\\, #3 }}$/;"	C
\\concat	math-symbols.tex	/^\\newcommand{\\concat}[1]{\\left[ #1 \\right]}$/;"	C
\\dbyd	math-symbols.tex	/^\\newcommand{\\dbyd}[2]{\\frac{d #1}{d #2}}$/;"	C
\\dobydo	math-symbols.tex	/^\\newcommand{\\dobydo}[2]{\\frac{\\partial #1}{\\partial #2}}$/;"	C
\\dotcm	math-symbols.tex	/^\\newcommand{\\dotcm}{\\dot{c}_m}$/;"	C
\\dotcnk	math-symbols.tex	/^\\newcommand{\\dotcnk}{\\dot{c}_\\nk}$/;"	C
\\dti	math-symbols.tex	/^\\newcommand{\\dti}{^{\\langle t \\rangle}}$/;"	C
\\dtim	math-symbols.tex	/^\\newcommand{\\dtim}[1]{^{\\langle t-{#1} \\rangle}}$/;"	C
\\dtip	math-symbols.tex	/^\\newcommand{\\dtip}[1]{^{\\langle t+{#1} \\rangle}}$/;"	C
\\ek	math-symbols.tex	/^\\newcommand{\\ek}{\\ensuremath{{e_\\tinyk}}}$/;"	C
\\fix	main.tex	/^\\newcommand{\\fix}{\\marginpar{FIX}}$/;"	C
\\fun	math-symbols.tex	/^\\newcommand{\\fun}[2]{{#1}\\bwrap{#2}}$/;"	C
\\hp	math-symbols.tex	/^\\newcommand{\\hp}{{\\,\\mathrel{\\vcenter{\\hbox{\\tiny$\\odot$}}}\\,}}$/;"	C
\\ik	math-symbols.tex	/^\\newcommand{\\ik}{\\ensuremath{{i_\\tinyk}}}$/;"	C
\\narrowstyle	math-symbols.tex	/^\\newcommand\\narrowstyle{\\SetTracking{encoding=*}{-40}\\lsstyle}$/;"	C
\\new	main.tex	/^\\newcommand{\\new}{\\marginpar{NEW}}$/;"	C
\\nk	math-symbols.tex	/^\\newcommand{\\nk}{\\ensuremath{{n_\\tinyk}}}$/;"	C
\\nkm	math-symbols.tex	/^\\newcommand{\\nkm}{\\ensuremath{{n_\\tinykm}}}$/;"	C
\\nkp	math-symbols.tex	/^\\newcommand{\\nkp}{\\ensuremath{{n_\\tinykp}}}$/;"	C
\\ours	math-symbols.tex	/^\\newcommand{\\ours}{\\textbf{ours}}$/;"	C
\\red	main.tex	/^\\newcommand{\\red}[1]{\\textcolor{red}{#1}}$/;"	C
\\scx	math-symbols.tex	/^\\newcommand{\\scx}{\\textsc{x}}$/;"	C
\\sk	math-symbols.tex	/^\\newcommand{\\sk}{\\ensuremath{{s_\\tinyk}}}$/;"	C
\\skm	math-symbols.tex	/^\\newcommand{\\skm}{\\ensuremath{{s_\\tinykm}}}$/;"	C
\\skp	math-symbols.tex	/^\\newcommand{\\skp}{\\ensuremath{{s_\\tinykp}}}$/;"	C
\\sups	math-symbols.tex	/^\\newcommand{\\sups}{\\ensuremath{^{(s)}}}$/;"	C
\\supt	math-symbols.tex	/^\\newcommand{\\supt}{\\ensuremath{^{(t)}}}$/;"	C
\\suptm	math-symbols.tex	/^\\newcommand{\\suptm}{\\ensuremath{^{(t-1)}}}$/;"	C
\\tek	math-symbols.tex	/^\\newcommand{\\tek}{\\ensuremath{{\\tilde{e}_\\tinyk}}}$/;"	C
\\tia	math-symbols.tex	/^\\newcommand{\\tia}{\\ensuremath{\\tilde{\\alpha}}}$/;"	C
\\tib	math-symbols.tex	/^\\newcommand{\\tib}{\\ensuremath{\\tilde{\\beta}}}$/;"	C
\\tinyk	math-symbols.tex	/^\\newcommand{\\tinyk}{\\text{\\scalebox{0.75}{\\hspace{-0.5pt}$k$}}}$/;"	C
\\tinykm	math-symbols.tex	/^\\newcommand{\\tinykm}{\\text{\\scalebox{0.75}{\\hspace{-0.5pt}$k-1$}}}$/;"	C
\\tinykp	math-symbols.tex	/^\\newcommand{\\tinykp}{\\text{\\scalebox{0.75}{\\hspace{-0.5pt}$k+1$}}}$/;"	C
\\tio	math-symbols.tex	/^\\newcommand{\\tio}{\\ensuremath{\\tilde{\\omega}}}$/;"	C
\\updated	main.tex	/^\\newcommand{\\updated}[1]{\\textcolor{blue}{#1}}$/;"	C
\\vji	math-symbols.tex	/^\\newcommand{\\vji}{\\ensuremath{v_{ji}}}$/;"	C
_TuringNLG_2020	references.bib	/^@misc{_TuringNLG_2020,$/;"	n
amir2017low	references.bib	/^@inproceedings{amir2017low,$/;"	j
axes_1_00000023270426867544736580000017173583425015905456_	figures/combined-sparsity-plots.svg	/^<g id="axes_1_00000023270426867544736580000017173583425015905456_">$/;"	i
axes_1_00000106855205435804047330000018295762245467367814_	figures/combined-sparsity-plots.svg	/^<g id="axes_1_00000106855205435804047330000018295762245467367814_">$/;"	i
axes_2	figures/combined-sparsity-plots.svg	/^<g id="axes_2">$/;"	i
axes_2_00000062902309342542668400000010395500875705497023_	figures/combined-sparsity-plots.svg	/^<g id="axes_2_00000062902309342542668400000010395500875705497023_">$/;"	i
axes_3_00000103250286677678878030000004929683155943265189_	figures/combined-sparsity-plots.svg	/^<g id="axes_3_00000103250286677678878030000004929683155943265189_">$/;"	i
axes_4_00000039850927196085700150000008982226111754729893_	figures/combined-sparsity-plots.svg	/^<g id="axes_4_00000039850927196085700150000008982226111754729893_">$/;"	i
axes_6	figures/combined-sparsity-plots.svg	/^<g id="axes_6">$/;"	i
barton_modeling_2002	references.bib	/^@article{barton_modeling_2002,$/;"	a
base	figures/pseudo-derivative.svg	/^     inkscape:deskcolor="#d1d1d1">$/;"	i
beer_Dynamics_1995	references.bib	/^@article{beer_Dynamics_1995,$/;"	a
bellec2018deep	references.bib	/^@inproceedings{bellec2018deep,$/;"	j
bellec_Long_2018	references.bib	/^@inproceedings{bellec_Long_2018,$/;"	j
bellec_solution_2020	references.bib	/^@article{bellec_solution_2020,$/;"	a
bender2021dangers	references.bib	/^@inproceedings{bender2021dangers,$/;"	j
birhane2021values	references.bib	/^@article{birhane2021values,$/;"	a
bohning_Multinomial_1992	references.bib	/^@article{bohning_Multinomial_1992,$/;"	a
bommasani2021opportunities	references.bib	/^@article{bommasani2021opportunities,$/;"	a
bradbury_QuasiRecurrent_2016	references.bib	/^@article{bradbury_QuasiRecurrent_2016,$/;"	a
brown_Language_2020	references.bib	/^@article{brown_Language_2020,$/;"	a
bryson_applied_2018	references.bib	/^@book{bryson_applied_2018,$/;"	b
cc	figures/pseudo-derivative.svg	/^   xmlns:dc="http:\/\/purl.org\/dc\/elements\/1.1\/">$/;"	n	uri:http://creativecommons.org/ns#
cerebras	references.bib	/^@misc{cerebras,$/;"	n
chang_AntisymmetricRNN_2019	references.bib	/^@article{chang_AntisymmetricRNN_2019,$/;"	a
chavent_identification_1974	references.bib	/^@article{chavent_identification_1974,$/;"	a
chen2020learning	references.bib	/^@inproceedings{chen2020learning,$/;"	j
chen_Neural_2018	references.bib	/^@incollection{chen_Neural_2018,$/;"	I
cho2014learning	references.bib	/^@article{cho2014learning,$/;"	a
choi_Attention_2019	references.bib	/^@inproceedings{choi_Attention_2019,$/;"	j
christensen2022roadmap	references.bib	/^@article{christensen2022roadmap,$/;"	a
corbetta2002control	references.bib	/^@article{corbetta2002control,$/;"	a
corollary	main.tex	/^\\newtheorem{corollary}{Corollary}$/;"	t
danihelka2016associative	references.bib	/^@misc{danihelka2016associative,$/;"	n
davies2018loihi	references.bib	/^@article{davies2018loihi,$/;"	a
dc	figures/pseudo-derivative.svg	/^   xmlns:dc="http:\/\/purl.org\/dc\/elements\/1.1\/">$/;"	n	uri:http://purl.org/dc/elements/1.1/
debrouwer2019gruodebayesa	references.bib	/^@inproceedings{debrouwer2019gruodebayesa,$/;"	j
decandia2007dynamo	references.bib	/^@article{decandia2007dynamo,$/;"	a
defs143459	figures/pseudo-derivative.svg	/^     id="defs143459">$/;"	i
dehghani2018universal	references.bib	/^@inproceedings{dehghani2018universal,$/;"	j
desislavov2021compute	references.bib	/^@misc{desislavov2021compute,$/;"	n
eq:barM	main.tex	/^\\begin{equation}\\label{eq:barM}$/;"	l
eq:jacobian	main.tex	/^\\begin{align}\\label{eq:jacobian}$/;"	l
eq:main-recursive	main.tex	/^\\begin{equation}\\label{eq:main-recursive}$/;"	l
espeholt_IMPALA_2018	references.bib	/^@article{espeholt_IMPALA_2018,$/;"	a
esser_Convolutional_2016	references.bib	/^@article{esser_Convolutional_2016,$/;"	a
fedus_Switch_2021	references.bib	/^@article{fedus_Switch_2021,$/;"	a
feehery_Efficient_1997	references.bib	/^@article{feehery_Efficient_1997,$/;"	a
fig:matrix	main.tex	/^        \\label{fig:matrix}}$/;"	l
fig:pseudo-derivative	main.tex	/^        \\caption{Illustration of surrogate gradient (pseudo-derivative)\\label{fig:pseudo-deriv/;"	l
fig:results	main.tex	/^    \\caption{Computational savings and sparsity results on synthetic dataset. Mean and std err /;"	l
galan_Parametric_1999	references.bib	/^@article{galan_Parametric_1999,$/;"	a
gale2019state	references.bib	/^@article{gale2019state,$/;"	a
ghosh2019Spatiotemporal	references.bib	/^@misc{ghosh2019Spatiotemporal,$/;"	n
goyal_Recurrent_2019	references.bib	/^@article{goyal_Recurrent_2019,$/;"	a
grid1650	figures/pseudo-derivative.svg	/^       id="grid1650" \/>$/;"	i
gronwall1919note	references.bib	/^@article{gronwall1919note,$/;"	a
gu2020improving	references.bib	/^@inproceedings{gu2020improving,$/;"	j
guide146651	figures/pseudo-derivative.svg	/^       inkscape:color="rgb(228,87,31)" \/>$/;"	i
guide146736	figures/pseudo-derivative.svg	/^       inkscape:color="rgb(228,87,31)" \/>$/;"	i
guide151099	figures/pseudo-derivative.svg	/^       inkscape:locked="false" \/>$/;"	i
guide163145	figures/pseudo-derivative.svg	/^       inkscape:locked="false" \/>$/;"	i
guide1646	figures/pseudo-derivative.svg	/^       inkscape:locked="false" \/>$/;"	i
guide1648	figures/pseudo-derivative.svg	/^       inkscape:locked="false" \/>$/;"	i
guide165310	figures/pseudo-derivative.svg	/^       inkscape:locked="false" \/>$/;"	i
guide165312	figures/pseudo-derivative.svg	/^       inkscape:locked="false" \/>$/;"	i
guide165554	figures/pseudo-derivative.svg	/^       inkscape:locked="false" \/>$/;"	i
guide3636	figures/pseudo-derivative.svg	/^       inkscape:locked="false" \/>$/;"	i
guo_Population_2012	references.bib	/^@article{guo_Population_2012,$/;"	a
haste2020	references.bib	/^@misc{haste2020,$/;"	n
he2020comparing	references.bib	/^@article{he2020comparing,$/;"	a
hochreiter_Long_1997	references.bib	/^@article{hochreiter_Long_1997,$/;"	a
hoefler2021sparsity	references.bib	/^@article{hoefler2021sparsity,$/;"	a
hoefler_Sparsity_2021	references.bib	/^@article{hoefler_Sparsity_2021,$/;"	a
hooker2019compressed	references.bib	/^@article{hooker2019compressed,$/;"	a
hoppner2017dynamic	references.bib	/^@inproceedings{hoppner2017dynamic,$/;"	j
hunter2021sparsities	references.bib	/^@misc{hunter2021sparsities,$/;"	n
hussain_Delay_2014	references.bib	/^@article{hussain_Delay_2014,$/;"	a
inan2017tying	references.bib	/^@inproceedings{inan2017tying,$/;"	j
inkscape	figures/pseudo-derivative.svg	/^   xmlns:dc="http:\/\/purl.org\/dc\/elements\/1.1\/">$/;"	n	uri:http://www.inkscape.org/namespaces/inkscape
innocenti2021temporal	references.bib	/^@inproceedings{innocenti2021temporal,$/;"	j
jaderberg_Decoupled_2016	references.bib	/^@article{jaderberg_Decoupled_2016,$/;"	a
jia2019dissecting	references.bib	/^@article{jia2019dissecting,$/;"	a
jordan_Gated_2019	references.bib	/^@article{jordan_Gated_2019,$/;"	a
jordan_extremely_2018	references.bib	/^@article{jordan_extremely_2018,$/;"	a
kidger_Neural_2020a	references.bib	/^@article{kidger_Neural_2020a,$/;"	a
lamport1998part	references.bib	/^@article{lamport1998part,$/;"	a
laskin_Parallel_2020	references.bib	/^@article{laskin_Parallel_2020,$/;"	a
layer1	figures/pseudo-derivative.svg	/^     transform="translate(-0.17461809,-0.60135857)">$/;"	i
layer2	figures/pseudo-derivative.svg	/^     sodipodi:insensitive="true">$/;"	i
le2015simple	references.bib	/^@misc{le2015simple,$/;"	n
lechner2020learning	references.bib	/^@article{lechner2020learning,$/;"	a
lecun1998gradient	references.bib	/^@article{lecun1998gradient,$/;"	a
legend_1	figures/combined-sparsity-plots.svg	/^	<g id="legend_1">$/;"	i
lei_Simple_2017	references.bib	/^@article{lei_Simple_2017,$/;"	a
li2020deep	references.bib	/^@article{li2020deep,$/;"	a
li2020federated	references.bib	/^@article{li2020federated,$/;"	a
li_Independently_2018	references.bib	/^@article{li_Independently_2018,$/;"	a
lichtsteiner2008128	references.bib	/^@article{lichtsteiner2008128,$/;"	a
line2d_100	figures/combined-sparsity-plots.svg	/^		<g id="line2d_100">$/;"	i
line2d_101	figures/combined-sparsity-plots.svg	/^		<g id="line2d_101">$/;"	i
line2d_102	figures/combined-sparsity-plots.svg	/^		<g id="line2d_102">$/;"	i
line2d_103	figures/combined-sparsity-plots.svg	/^		<g id="line2d_103">$/;"	i
line2d_104	figures/combined-sparsity-plots.svg	/^		<g id="line2d_104">$/;"	i
line2d_105	figures/combined-sparsity-plots.svg	/^		<g id="line2d_105">$/;"	i
line2d_10_00000023986287797542087770000013690430315983508638_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_10_00000023986287797542087770000013690430315983508638_">$/;"	i
line2d_10_00000098921245006299149800000017092363594734122682_	figures/combined-sparsity-plots.svg	/^	<g id="line2d_10_00000098921245006299149800000017092363594734122682_">$/;"	i
line2d_11_00000038390023768077166900000009888489111847761597_	figures/combined-sparsity-plots.svg	/^	<g id="line2d_11_00000038390023768077166900000009888489111847761597_">$/;"	i
line2d_11_00000133515200250720226600000010497292162072010117_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_11_00000133515200250720226600000010497292162072010117_">$/;"	i
line2d_12_00000004514585772558886000000012237754167994492601_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_12_00000004514585772558886000000012237754167994492601_">$/;"	i
line2d_12_00000011000931612377663470000018121312483626447777_	figures/combined-sparsity-plots.svg	/^	<g id="line2d_12_00000011000931612377663470000018121312483626447777_">$/;"	i
line2d_13_00000010312990953954388630000015648365670105892739_	figures/combined-sparsity-plots.svg	/^	<g id="line2d_13_00000010312990953954388630000015648365670105892739_">$/;"	i
line2d_13_00000072983512977009585870000006277545882510671009_	figures/combined-sparsity-plots.svg	/^	<g id="line2d_13_00000072983512977009585870000006277545882510671009_">$/;"	i
line2d_14_00000057847660861173175720000016670367624922062473_	figures/combined-sparsity-plots.svg	/^	<g id="line2d_14_00000057847660861173175720000016670367624922062473_">$/;"	i
line2d_14_00000139978829307368640240000005845811487527601797_	figures/combined-sparsity-plots.svg	/^	<g id="line2d_14_00000139978829307368640240000005845811487527601797_">$/;"	i
line2d_15_00000005228500448001196880000005308025362708510124_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_15_00000005228500448001196880000005308025362708510124_">$/;"	i
line2d_15_00000100365678885761239840000001746603408827227010_	figures/combined-sparsity-plots.svg	/^	<g id="line2d_15_00000100365678885761239840000001746603408827227010_">$/;"	i
line2d_16_00000026123970897236722790000001391138590456816521_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_16_00000026123970897236722790000001391138590456816521_">$/;"	i
line2d_16_00000119113787544839902390000016176367795958603446_	figures/combined-sparsity-plots.svg	/^	<g id="line2d_16_00000119113787544839902390000016176367795958603446_">$/;"	i
line2d_17_00000016043876262989610170000000979883338126251175_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_17_00000016043876262989610170000000979883338126251175_">$/;"	i
line2d_17_00000044884458544560951680000014642214176112625327_	figures/combined-sparsity-plots.svg	/^	<g id="line2d_17_00000044884458544560951680000014642214176112625327_">$/;"	i
line2d_18_00000075873136260618750470000010992318717472498564_	figures/combined-sparsity-plots.svg	/^	<g id="line2d_18_00000075873136260618750470000010992318717472498564_">$/;"	i
line2d_18_00000096742479280216420020000000917305122026706606_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_18_00000096742479280216420020000000917305122026706606_">$/;"	i
line2d_19_00000066517696414685899800000006408374372583824557_	figures/combined-sparsity-plots.svg	/^	<g id="line2d_19_00000066517696414685899800000006408374372583824557_">$/;"	i
line2d_19_00000084531427869462324750000013360323652591226790_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_19_00000084531427869462324750000013360323652591226790_">$/;"	i
line2d_1_00000101801514012270272430000001658068918139294868_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_1_00000101801514012270272430000001658068918139294868_">$/;"	i
line2d_1_00000108996624439804974280000000759485239937773232_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_1_00000108996624439804974280000000759485239937773232_">$/;"	i
line2d_20_00000173153031375221988440000009783337717764556177_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_20_00000173153031375221988440000009783337717764556177_">$/;"	i
line2d_20_00000175311368149654320840000011189204608842767772_	figures/combined-sparsity-plots.svg	/^	<g id="line2d_20_00000175311368149654320840000011189204608842767772_">$/;"	i
line2d_21_00000045583626385235476120000002675111798602140045_	figures/combined-sparsity-plots.svg	/^	<g id="line2d_21_00000045583626385235476120000002675111798602140045_">$/;"	i
line2d_21_00000145764581747210024670000004224209648257140916_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_21_00000145764581747210024670000004224209648257140916_">$/;"	i
line2d_22_00000008107429359071171110000010679079226419946119_	figures/combined-sparsity-plots.svg	/^	<g id="line2d_22_00000008107429359071171110000010679079226419946119_">$/;"	i
line2d_22_00000175291561148639427850000013379690296378949551_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_22_00000175291561148639427850000013379690296378949551_">$/;"	i
line2d_23	figures/combined-sparsity-plots.svg	/^			<g id="line2d_23">$/;"	i
line2d_23_00000036220250781912461940000002483532659094806405_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_23_00000036220250781912461940000002483532659094806405_">$/;"	i
line2d_24	figures/combined-sparsity-plots.svg	/^			<g id="line2d_24">$/;"	i
line2d_24_00000088821498977345497440000001103323842706904507_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_24_00000088821498977345497440000001103323842706904507_">$/;"	i
line2d_25	figures/combined-sparsity-plots.svg	/^			<g id="line2d_25">$/;"	i
line2d_25_00000088816647012729074040000016708407076645090688_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_25_00000088816647012729074040000016708407076645090688_">$/;"	i
line2d_26	figures/combined-sparsity-plots.svg	/^			<g id="line2d_26">$/;"	i
line2d_26_00000057120006498292122430000002007756777303999384_	figures/combined-sparsity-plots.svg	/^	<g id="line2d_26_00000057120006498292122430000002007756777303999384_">$/;"	i
line2d_27	figures/combined-sparsity-plots.svg	/^			<g id="line2d_27">$/;"	i
line2d_27_00000045619020414628384930000009276232666329833630_	figures/combined-sparsity-plots.svg	/^	<g id="line2d_27_00000045619020414628384930000009276232666329833630_">$/;"	i
line2d_28	figures/combined-sparsity-plots.svg	/^			<g id="line2d_28">$/;"	i
line2d_28_00000145039082931743051670000016084490942778406323_	figures/combined-sparsity-plots.svg	/^	<g id="line2d_28_00000145039082931743051670000016084490942778406323_">$/;"	i
line2d_29	figures/combined-sparsity-plots.svg	/^			<g id="line2d_29">$/;"	i
line2d_29_00000181088677633996220940000005196907327317185429_	figures/combined-sparsity-plots.svg	/^	<g id="line2d_29_00000181088677633996220940000005196907327317185429_">$/;"	i
line2d_2_00000138561280315531894000000017311735021480816038_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_2_00000138561280315531894000000017311735021480816038_">$/;"	i
line2d_2_00000147920391300926743700000000871792550781299894_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_2_00000147920391300926743700000000871792550781299894_">$/;"	i
line2d_30	figures/combined-sparsity-plots.svg	/^			<g id="line2d_30">$/;"	i
line2d_30_00000008846015173893359610000005913929785539019955_	figures/combined-sparsity-plots.svg	/^	<g id="line2d_30_00000008846015173893359610000005913929785539019955_">$/;"	i
line2d_31	figures/combined-sparsity-plots.svg	/^			<g id="line2d_31">$/;"	i
line2d_31_00000017493998024128935860000016403444998205097902_	figures/combined-sparsity-plots.svg	/^	<g id="line2d_31_00000017493998024128935860000016403444998205097902_">$/;"	i
line2d_32	figures/combined-sparsity-plots.svg	/^			<g id="line2d_32">$/;"	i
line2d_32_00000042726203717067787840000004005952086340594620_	figures/combined-sparsity-plots.svg	/^	<g id="line2d_32_00000042726203717067787840000004005952086340594620_">$/;"	i
line2d_33	figures/combined-sparsity-plots.svg	/^			<g id="line2d_33">$/;"	i
line2d_33_00000101792974801761324220000011581740261195755395_	figures/combined-sparsity-plots.svg	/^	<g id="line2d_33_00000101792974801761324220000011581740261195755395_">$/;"	i
line2d_34	figures/combined-sparsity-plots.svg	/^	<g id="line2d_34">$/;"	i
line2d_34_00000075126835086585222990000017986621228294926748_	figures/combined-sparsity-plots.svg	/^	<g id="line2d_34_00000075126835086585222990000017986621228294926748_">$/;"	i
line2d_35	figures/combined-sparsity-plots.svg	/^	<g id="line2d_35">$/;"	i
line2d_35_00000155121540972769853200000000613696798862234532_	figures/combined-sparsity-plots.svg	/^	<g id="line2d_35_00000155121540972769853200000000613696798862234532_">$/;"	i
line2d_36	figures/combined-sparsity-plots.svg	/^	<g id="line2d_36">$/;"	i
line2d_36_00000022536005491472538420000001758519789167272579_	figures/combined-sparsity-plots.svg	/^		<g id="line2d_36_00000022536005491472538420000001758519789167272579_">$/;"	i
line2d_36_00000098907054540358713000000003833819080197954750_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_36_00000098907054540358713000000003833819080197954750_">$/;"	i
line2d_37	figures/combined-sparsity-plots.svg	/^	<g id="line2d_37">$/;"	i
line2d_37_00000026158955008037708820000007375799987413061026_	figures/combined-sparsity-plots.svg	/^		<g id="line2d_37_00000026158955008037708820000007375799987413061026_">$/;"	i
line2d_37_00000111884938535347646430000014140611111387535506_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_37_00000111884938535347646430000014140611111387535506_">$/;"	i
line2d_38	figures/combined-sparsity-plots.svg	/^	<g id="line2d_38">$/;"	i
line2d_38_00000016756813069098841280000017224576543250279582_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_38_00000016756813069098841280000017224576543250279582_">$/;"	i
line2d_38_00000085964114056062126560000017458521919499480227_	figures/combined-sparsity-plots.svg	/^		<g id="line2d_38_00000085964114056062126560000017458521919499480227_">$/;"	i
line2d_39	figures/combined-sparsity-plots.svg	/^	<g id="line2d_39">$/;"	i
line2d_39_00000001646452080386476560000008040902811618368897_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_39_00000001646452080386476560000008040902811618368897_">$/;"	i
line2d_39_00000034058312664138042820000016159220025022426814_	figures/combined-sparsity-plots.svg	/^		<g id="line2d_39_00000034058312664138042820000016159220025022426814_">$/;"	i
line2d_3_00000020364081205497947170000006448769302782557065_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_3_00000020364081205497947170000006448769302782557065_">$/;"	i
line2d_3_00000038378856915479652490000002213203055888203930_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_3_00000038378856915479652490000002213203055888203930_">$/;"	i
line2d_40	figures/combined-sparsity-plots.svg	/^	<g id="line2d_40">$/;"	i
line2d_40_00000000218222431821095310000008817216252021247883_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_40_00000000218222431821095310000008817216252021247883_">$/;"	i
line2d_40_00000062150996469646842670000013815870428871476126_	figures/combined-sparsity-plots.svg	/^		<g id="line2d_40_00000062150996469646842670000013815870428871476126_">$/;"	i
line2d_41	figures/combined-sparsity-plots.svg	/^	<g id="line2d_41">$/;"	i
line2d_41_00000069398735944575296430000002239868794154572175_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_41_00000069398735944575296430000002239868794154572175_">$/;"	i
line2d_41_00000151508547178815043330000017028188595031123847_	figures/combined-sparsity-plots.svg	/^		<g id="line2d_41_00000151508547178815043330000017028188595031123847_">$/;"	i
line2d_42	figures/combined-sparsity-plots.svg	/^	<g id="line2d_42">$/;"	i
line2d_42_00000013898462072612106820000007330471852668162714_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_42_00000013898462072612106820000007330471852668162714_">$/;"	i
line2d_42_00000124132512305970610260000011547524566932628415_	figures/combined-sparsity-plots.svg	/^		<g id="line2d_42_00000124132512305970610260000011547524566932628415_">$/;"	i
line2d_43	figures/combined-sparsity-plots.svg	/^	<g id="line2d_43">$/;"	i
line2d_43_00000023267649196428898780000002516257801969669255_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_43_00000023267649196428898780000002516257801969669255_">$/;"	i
line2d_43_00000145767153939749993210000014380201797754323124_	figures/combined-sparsity-plots.svg	/^		<g id="line2d_43_00000145767153939749993210000014380201797754323124_">$/;"	i
line2d_44_00000079445769677023042810000012632387295758757763_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_44_00000079445769677023042810000012632387295758757763_">$/;"	i
line2d_45_00000094585936761280255500000000296976071812419515_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_45_00000094585936761280255500000000296976071812419515_">$/;"	i
line2d_46_00000141445993429946128610000008020454848371524265_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_46_00000141445993429946128610000008020454848371524265_">$/;"	i
line2d_47_00000001654264327076465910000012274089713836910250_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_47_00000001654264327076465910000012274089713836910250_">$/;"	i
line2d_48_00000115484310411117701760000008322155932851450811_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_48_00000115484310411117701760000008322155932851450811_">$/;"	i
line2d_49_00000065789230522077349630000006396097179038469026_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_49_00000065789230522077349630000006396097179038469026_">$/;"	i
line2d_4_00000123430722734348699590000017692815137967744945_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_4_00000123430722734348699590000017692815137967744945_">$/;"	i
line2d_4_00000139278752014535386380000009556572445123358106_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_4_00000139278752014535386380000009556572445123358106_">$/;"	i
line2d_50_00000057852078077948736010000016628805537534962838_	figures/combined-sparsity-plots.svg	/^	<g id="line2d_50_00000057852078077948736010000016628805537534962838_">$/;"	i
line2d_51_00000044878520687493264040000007917675432154165683_	figures/combined-sparsity-plots.svg	/^	<g id="line2d_51_00000044878520687493264040000007917675432154165683_">$/;"	i
line2d_52_00000023280481589720729500000006878391874602962563_	figures/combined-sparsity-plots.svg	/^	<g id="line2d_52_00000023280481589720729500000006878391874602962563_">$/;"	i
line2d_53_00000163054706868757641640000005229040330199649199_	figures/combined-sparsity-plots.svg	/^	<g id="line2d_53_00000163054706868757641640000005229040330199649199_">$/;"	i
line2d_54_00000143617452767804919230000004101009039646861227_	figures/combined-sparsity-plots.svg	/^	<g id="line2d_54_00000143617452767804919230000004101009039646861227_">$/;"	i
line2d_55_00000183211676367833831330000017808594414477985931_	figures/combined-sparsity-plots.svg	/^	<g id="line2d_55_00000183211676367833831330000017808594414477985931_">$/;"	i
line2d_56_00000108293322874051540400000002508685017465698472_	figures/combined-sparsity-plots.svg	/^	<g id="line2d_56_00000108293322874051540400000002508685017465698472_">$/;"	i
line2d_57_00000000194949011136702550000013227390093899126698_	figures/combined-sparsity-plots.svg	/^	<g id="line2d_57_00000000194949011136702550000013227390093899126698_">$/;"	i
line2d_58_00000008110779189021159480000013664338366690147484_	figures/combined-sparsity-plots.svg	/^	<g id="line2d_58_00000008110779189021159480000013664338366690147484_">$/;"	i
line2d_59_00000030486428548712241160000007170101050634847147_	figures/combined-sparsity-plots.svg	/^	<g id="line2d_59_00000030486428548712241160000007170101050634847147_">$/;"	i
line2d_5_00000109012340280603729920000004025833147281673099_	figures/combined-sparsity-plots.svg	/^	<g id="line2d_5_00000109012340280603729920000004025833147281673099_">$/;"	i
line2d_5_00000145040462825541457510000011351044721388186047_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_5_00000145040462825541457510000011351044721388186047_">$/;"	i
line2d_60_00000005954566699516853960000001509455338588326833_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_60_00000005954566699516853960000001509455338588326833_">$/;"	i
line2d_61_00000174592750569418460990000000268140139575335091_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_61_00000174592750569418460990000000268140139575335091_">$/;"	i
line2d_62_00000121266752674357704650000000219893718063393154_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_62_00000121266752674357704650000000219893718063393154_">$/;"	i
line2d_63_00000175295992392063921920000015446883652061709483_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_63_00000175295992392063921920000015446883652061709483_">$/;"	i
line2d_64_00000164482884788680027740000016175055289134015132_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_64_00000164482884788680027740000016175055289134015132_">$/;"	i
line2d_65_00000080198475280987439180000003673882870352674186_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_65_00000080198475280987439180000003673882870352674186_">$/;"	i
line2d_66_00000114063073079266523390000000851390395815278735_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_66_00000114063073079266523390000000851390395815278735_">$/;"	i
line2d_67_00000180340500398534934870000013528116746318276757_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_67_00000180340500398534934870000013528116746318276757_">$/;"	i
line2d_68_00000020399498789918980110000012047022831676391057_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_68_00000020399498789918980110000012047022831676391057_">$/;"	i
line2d_69_00000099627306806680462180000016609383969473663663_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_69_00000099627306806680462180000016609383969473663663_">$/;"	i
line2d_6_00000013876689472239881510000012110068646036744104_	figures/combined-sparsity-plots.svg	/^	<g id="line2d_6_00000013876689472239881510000012110068646036744104_">$/;"	i
line2d_6_00000178888051252964673330000000986991444576182178_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_6_00000178888051252964673330000000986991444576182178_">$/;"	i
line2d_70_00000111892138947312347130000011441768577279238284_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_70_00000111892138947312347130000011441768577279238284_">$/;"	i
line2d_71_00000181774098264130700010000009258867699768404895_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_71_00000181774098264130700010000009258867699768404895_">$/;"	i
line2d_72_00000019637472095804696200000009971827443670950813_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_72_00000019637472095804696200000009971827443670950813_">$/;"	i
line2d_73_00000098920146417406973530000005558094993881966471_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_73_00000098920146417406973530000005558094993881966471_">$/;"	i
line2d_74_00000074437330172586444820000006894971238036529545_	figures/combined-sparsity-plots.svg	/^	<g id="line2d_74_00000074437330172586444820000006894971238036529545_">$/;"	i
line2d_75_00000003067067738841436700000000784809684909920920_	figures/combined-sparsity-plots.svg	/^	<g id="line2d_75_00000003067067738841436700000000784809684909920920_">$/;"	i
line2d_76_00000086664365586151163120000014651501303281668499_	figures/combined-sparsity-plots.svg	/^	<g id="line2d_76_00000086664365586151163120000014651501303281668499_">$/;"	i
line2d_77_00000010991168443999416410000002990692365513227700_	figures/combined-sparsity-plots.svg	/^	<g id="line2d_77_00000010991168443999416410000002990692365513227700_">$/;"	i
line2d_78_00000171688234549305757020000005677003812380083381_	figures/combined-sparsity-plots.svg	/^	<g id="line2d_78_00000171688234549305757020000005677003812380083381_">$/;"	i
line2d_79_00000183230040683680978810000012361629871911960762_	figures/combined-sparsity-plots.svg	/^	<g id="line2d_79_00000183230040683680978810000012361629871911960762_">$/;"	i
line2d_7_00000047036936550323324690000005387938709120033161_	figures/combined-sparsity-plots.svg	/^	<g id="line2d_7_00000047036936550323324690000005387938709120033161_">$/;"	i
line2d_7_00000132786190583600716740000016185653803743344282_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_7_00000132786190583600716740000016185653803743344282_">$/;"	i
line2d_80_00000095313160414029726720000006956596685243645587_	figures/combined-sparsity-plots.svg	/^	<g id="line2d_80_00000095313160414029726720000006956596685243645587_">$/;"	i
line2d_81_00000121260790301182283540000017456025453995096213_	figures/combined-sparsity-plots.svg	/^	<g id="line2d_81_00000121260790301182283540000017456025453995096213_">$/;"	i
line2d_82_00000025422177158775513060000016767625202324595617_	figures/combined-sparsity-plots.svg	/^	<g id="line2d_82_00000025422177158775513060000016767625202324595617_">$/;"	i
line2d_83_00000150081093694933969900000016536153336383120772_	figures/combined-sparsity-plots.svg	/^	<g id="line2d_83_00000150081093694933969900000016536153336383120772_">$/;"	i
line2d_86	figures/combined-sparsity-plots.svg	/^	<g id="line2d_86">$/;"	i
line2d_87	figures/combined-sparsity-plots.svg	/^	<g id="line2d_87">$/;"	i
line2d_88	figures/combined-sparsity-plots.svg	/^	<g id="line2d_88">$/;"	i
line2d_89	figures/combined-sparsity-plots.svg	/^	<g id="line2d_89">$/;"	i
line2d_8_00000006670906528179753530000015422618217010268311_	figures/combined-sparsity-plots.svg	/^	<g id="line2d_8_00000006670906528179753530000015422618217010268311_">$/;"	i
line2d_8_00000010268290832632888930000006323062225370809270_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_8_00000010268290832632888930000006323062225370809270_">$/;"	i
line2d_90	figures/combined-sparsity-plots.svg	/^	<g id="line2d_90">$/;"	i
line2d_91	figures/combined-sparsity-plots.svg	/^	<g id="line2d_91">$/;"	i
line2d_92	figures/combined-sparsity-plots.svg	/^	<g id="line2d_92">$/;"	i
line2d_93	figures/combined-sparsity-plots.svg	/^	<g id="line2d_93">$/;"	i
line2d_94	figures/combined-sparsity-plots.svg	/^	<g id="line2d_94">$/;"	i
line2d_95	figures/combined-sparsity-plots.svg	/^	<g id="line2d_95">$/;"	i
line2d_96	figures/combined-sparsity-plots.svg	/^		<g id="line2d_96">$/;"	i
line2d_97	figures/combined-sparsity-plots.svg	/^		<g id="line2d_97">$/;"	i
line2d_98	figures/combined-sparsity-plots.svg	/^		<g id="line2d_98">$/;"	i
line2d_99	figures/combined-sparsity-plots.svg	/^		<g id="line2d_99">$/;"	i
line2d_9_00000031906075751425278960000004888529032214514343_	figures/combined-sparsity-plots.svg	/^			<g id="line2d_9_00000031906075751425278960000004888529032214514343_">$/;"	i
line2d_9_00000040540137287194867770000004986396792209722515_	figures/combined-sparsity-plots.svg	/^	<g id="line2d_9_00000040540137287194867770000004986396792209722515_">$/;"	i
lisman_Bursts_1997	references.bib	/^@article{lisman_Bursts_1997,$/;"	a
liu2019intrinsically	references.bib	/^@misc{liu2019intrinsically,$/;"	n
liu2021efficient	references.bib	/^@article{liu2021efficient,$/;"	a
liu2021selfish	references.bib	/^@inproceedings{liu2021selfish,$/;"	j
m13807df1ec	figures/combined-sparsity-plots.svg	/^							l0,0v-1.3v0.8V69v0.4v0.3v-0.3v-0.3v0.5v-0.3V69v0.5v-0.7v0.7v-0.3v0.2v-0.6v-0.3V68v1.6V70v/;"	i
m19c53ea899	figures/combined-sparsity-plots.svg	/^							l-0.2-0.5l-0.2-0.4l-0.2-0.5L80,69.3l-0.2,0.3v1.1H79.7z"\/>$/;"	i
m2a8090b4bb	figures/combined-sparsity-plots.svg	/^							l-0.4-1.6l-0.4,1.2l-0.4-0.5l-0.4-0.6h-0.4l-0.4-2.1h-0.4l-0.4-0.8l-0.4,0.4v4.7H518.5z"\/>$/;"	i
m2aa2a98e15_00000065785139656996117270000004580211635980854914_	figures/combined-sparsity-plots.svg	/^							h-0.2l-0.2-2.1H80l-0.2-0.8l-0.2,0.4v4.4H79.4z"\/>$/;"	i
m2b309c9df6	figures/combined-sparsity-plots.svg	/^							l-0.2,0.1l-0.2-0.1l-0.2,0.1h-0.2L536.2,267.9L536.2,267.9z"\/>$/;"	i
m2e4a99abed	figures/combined-sparsity-plots.svg	/^							l-0.1,0.1l-0.1-0.6l-0.1-0.3l-0.1-0.5l-0.1,1.6l-0.1,0.1v0.6H536.3z"\/>$/;"	i
m363143482c	figures/combined-sparsity-plots.svg	/^							l0,0v-1.2v0.8v-0.1v0.4v0.3v-0.4v-0.2v0.5v-0.3v-0.3v0.6v-0.7v0.7v-0.4v0.2v-0.6V69v-0.5v1.6/;"	i
m3a7a4680c0	figures/combined-sparsity-plots.svg	/^							l-0.2-0.6l-0.2,0.6l-0.2-2.1l-0.2,1.8l-0.2-0.7l-0.2-0.5l-0.2,0.3l-0.2-2.6l-0.2,0.4L514,499/;"	i
m3cf8871903	figures/combined-sparsity-plots.svg	/^							v-0.3v-0.3v0.5v-0.3v-0.3v0.5V73v0.7v-0.3v0.2V73v-0.4v-0.5v1.6V74L536.2,71.7L536.2,71.7z"\//;"	i
m3e1d878996	figures/combined-sparsity-plots.svg	/^							v-0.3V70v-0.3v-0.2V70v-0.7V70v-0.3v0.1v-0.5v-0.4v-0.5V70v0.2v1.5H536.2z"\/>$/;"	i
m4635baac39	figures/combined-sparsity-plots.svg	/^							l-0.2,0.2l-0.2-0.4l-0.2,0.4l-0.2-0.4l-0.2-0.3l-0.2,0.6l-0.2-0.1l-0.2,0.2l-0.2,0.1l-0.2-0./;"	i
m46e8eee969	figures/combined-sparsity-plots.svg	/^							H518.6z"\/>$/;"	i
m47ed7e2fed	figures/combined-sparsity-plots.svg	/^							v-0.7v-0.2v0.4v-0.1v-1.2V70v-0.1v0.4v0.3v-0.4V70v0.5v-0.3V70v0.5v-0.7v0.7v-0.3v0.2v-0.6v-/;"	i
m484113e831	figures/combined-sparsity-plots.svg	/^							\/>$/;"	i
m4a2671e94f_00000155845964911015187350000007958264363931696015_	figures/combined-sparsity-plots.svg	/^							l-0.2-0.7l-0.2,0.7l-0.2-2.1l-0.2,1.9l-0.2-0.7l-0.2-0.4l-0.2,0.2l-0.2-2.7l-0.2,0.5l-0.2-0./;"	i
m4c09508fa9	figures/combined-sparsity-plots.svg	/^							l-0.2,0.1l-0.2-0.1l-0.2-0.1h-0.2h-0.2l-0.2-0.1H84h-0.2h-0.2l-0.2,0.1l-0.2,0.1H83l-0.2,0.3/;"	i
m4f4bfd553c	figures/combined-sparsity-plots.svg	/^							\/>$/;"	i
m55df168758_00000100358455311644403170000013668851547832672692_	figures/combined-sparsity-plots.svg	/^							l-0.2-0.6l-0.2,0.1l-0.2-2.3l-0.2,0.1l-0.2-0.7l-0.2,0.1v4.4H79.4z"\/>$/;"	i
m561ec4cbfd	figures/combined-sparsity-plots.svg	/^							l-0.2-0.4l-0.2-0.5l-0.2,1.6l-0.2,0.2L79.7,70.7L79.7,70.7z"\/>$/;"	i
m5698be4520_00000124126690376696383480000015706609943846435483_	figures/combined-sparsity-plots.svg	/^							l-0.2,0.7v4.5H79.4z"\/>$/;"	i
m5745777d33	figures/combined-sparsity-plots.svg	/^							l-0.2-0.3l-0.2,0.4l-0.2-0.2l-0.2-0.1L537,274h-0.2l-0.2,0.1l-0.2,0.1l-0.2-0.2L536.2,284.8L/;"	i
m5875a5107f	figures/combined-sparsity-plots.svg	/^							\/>$/;"	i
m5b8cdd57e3	figures/combined-sparsity-plots.svg	/^							v0.5v-0.7v0.7v-0.3v0.1v-0.5v-0.4L536.2,71.7l0.1,1.7v0.3L536.2,71.7L536.2,71.7z"\/>$/;"	i
m5de0691be6	figures/combined-sparsity-plots.svg	/^							L80,69.5l-0.2,0.4v0.8H79.7z"\/>$/;"	i
m5def0dc4f3	figures/combined-sparsity-plots.svg	/^						<path id="m5def0dc4f3" class="st21" d="M536.2,215.4v3.5"\/>$/;"	i
m5def0dc4f3_00000008870260105559809410000003610590837792169140_	figures/combined-sparsity-plots.svg	/^						<path id="m5def0dc4f3_00000008870260105559809410000003610590837792169140_" class="st21" d=/;"	i
m5def0dc4f3_00000013185083664821546340000014599780224481766046_	figures/combined-sparsity-plots.svg	/^						<path id="m5def0dc4f3_00000013185083664821546340000014599780224481766046_" class="st21" d=/;"	i
m5def0dc4f3_00000015319048082779842640000017908827312639071109_	figures/combined-sparsity-plots.svg	/^						<path id="m5def0dc4f3_00000015319048082779842640000017908827312639071109_" class="st21" d=/;"	i
m5def0dc4f3_00000018211303552182683720000009442649425850088322_	figures/combined-sparsity-plots.svg	/^						<path id="m5def0dc4f3_00000018211303552182683720000009442649425850088322_" class="st21" d=/;"	i
m5def0dc4f3_00000029724183578510664530000012136535567160115895_	figures/combined-sparsity-plots.svg	/^						<path id="m5def0dc4f3_00000029724183578510664530000012136535567160115895_" class="st21" d=/;"	i
m5def0dc4f3_00000029761890556011889390000009033930741595918985_	figures/combined-sparsity-plots.svg	/^						<path id="m5def0dc4f3_00000029761890556011889390000009033930741595918985_" class="st21" d=/;"	i
m5def0dc4f3_00000036933452019451010100000003103083404921676943_	figures/combined-sparsity-plots.svg	/^						<path id="m5def0dc4f3_00000036933452019451010100000003103083404921676943_" class="st21" d=/;"	i
m5def0dc4f3_00000036943008367041367530000016136268543781231547_	figures/combined-sparsity-plots.svg	/^						<path id="m5def0dc4f3_00000036943008367041367530000016136268543781231547_" class="st21" d=/;"	i
m5def0dc4f3_00000043422969469182097290000017698889763379476620_	figures/combined-sparsity-plots.svg	/^					<path id="m5def0dc4f3_00000043422969469182097290000017698889763379476620_" class="st21" d="/;"	i
m5def0dc4f3_00000051384491148145741700000000817675590405827004_	figures/combined-sparsity-plots.svg	/^						<path id="m5def0dc4f3_00000051384491148145741700000000817675590405827004_" class="st21" d=/;"	i
m5def0dc4f3_00000062899290237898845220000001858822527992098435_	figures/combined-sparsity-plots.svg	/^						<path id="m5def0dc4f3_00000062899290237898845220000001858822527992098435_" class="st21" d=/;"	i
m5def0dc4f3_00000065035796104063575290000005890869016066984585_	figures/combined-sparsity-plots.svg	/^						<path id="m5def0dc4f3_00000065035796104063575290000005890869016066984585_" class="st21" d=/;"	i
m5def0dc4f3_00000065792575752625710710000015260166649984231833_	figures/combined-sparsity-plots.svg	/^					<path id="m5def0dc4f3_00000065792575752625710710000015260166649984231833_" class="st21" d="/;"	i
m5def0dc4f3_00000067200697638698471830000007133172875284510857_	figures/combined-sparsity-plots.svg	/^						<path id="m5def0dc4f3_00000067200697638698471830000007133172875284510857_" class="st21" d=/;"	i
m5def0dc4f3_00000072962307405136339470000015928481644238120863_	figures/combined-sparsity-plots.svg	/^						<path id="m5def0dc4f3_00000072962307405136339470000015928481644238120863_" class="st21" d=/;"	i
m5def0dc4f3_00000076579260176716703700000009425493119456196542_	figures/combined-sparsity-plots.svg	/^						<path id="m5def0dc4f3_00000076579260176716703700000009425493119456196542_" class="st21" d=/;"	i
m5def0dc4f3_00000083784731098239807860000016090984461768303538_	figures/combined-sparsity-plots.svg	/^						<path id="m5def0dc4f3_00000083784731098239807860000016090984461768303538_" class="st21" d=/;"	i
m5def0dc4f3_00000091007642878391670820000009635214709344651935_	figures/combined-sparsity-plots.svg	/^					<path id="m5def0dc4f3_00000091007642878391670820000009635214709344651935_" class="st21" d="/;"	i
m5def0dc4f3_00000093875277088902945230000002993491353177364389_	figures/combined-sparsity-plots.svg	/^						<path id="m5def0dc4f3_00000093875277088902945230000002993491353177364389_" class="st21" d=/;"	i
m5def0dc4f3_00000099651762511921240220000001891639115857562007_	figures/combined-sparsity-plots.svg	/^						<path id="m5def0dc4f3_00000099651762511921240220000001891639115857562007_" class="st21" d=/;"	i
m5def0dc4f3_00000103259865923418678910000008985082814250511291_	figures/combined-sparsity-plots.svg	/^						<path id="m5def0dc4f3_00000103259865923418678910000008985082814250511291_" class="st21" d=/;"	i
m5def0dc4f3_00000104686318820966129020000008585678966395749038_	figures/combined-sparsity-plots.svg	/^					<path id="m5def0dc4f3_00000104686318820966129020000008585678966395749038_" class="st21" d="/;"	i
m5def0dc4f3_00000107558355527131417080000017934529636615147683_	figures/combined-sparsity-plots.svg	/^					<path id="m5def0dc4f3_00000107558355527131417080000017934529636615147683_" class="st21" d="/;"	i
m5def0dc4f3_00000111193105996471626470000012652846173324563369_	figures/combined-sparsity-plots.svg	/^						<path id="m5def0dc4f3_00000111193105996471626470000012652846173324563369_" class="st21" d=/;"	i
m5def0dc4f3_00000121995761185109830740000017410427734606251683_	figures/combined-sparsity-plots.svg	/^					<path id="m5def0dc4f3_00000121995761185109830740000017410427734606251683_" class="st21" d="/;"	i
m5def0dc4f3_00000125576159856260011640000012243592302412608673_	figures/combined-sparsity-plots.svg	/^						<path id="m5def0dc4f3_00000125576159856260011640000012243592302412608673_" class="st21" d=/;"	i
m5def0dc4f3_00000134241908956425320250000006411619142567500205_	figures/combined-sparsity-plots.svg	/^						<path id="m5def0dc4f3_00000134241908956425320250000006411619142567500205_" class="st21" d=/;"	i
m5def0dc4f3_00000142157126396720724300000005684479920464638139_	figures/combined-sparsity-plots.svg	/^					<path id="m5def0dc4f3_00000142157126396720724300000005684479920464638139_" class="st21" d="/;"	i
m5def0dc4f3_00000152955217481581430660000013607147570254822539_	figures/combined-sparsity-plots.svg	/^					<path id="m5def0dc4f3_00000152955217481581430660000013607147570254822539_" class="st21" d="/;"	i
m5def0dc4f3_00000160173615539025443330000017025372246693559965_	figures/combined-sparsity-plots.svg	/^						<path id="m5def0dc4f3_00000160173615539025443330000017025372246693559965_" class="st21" d=/;"	i
m65bd77e81c	figures/combined-sparsity-plots.svg	/^							l-0.2,0.4L79.7,70.7L79.7,70.7z"\/>$/;"	i
m68621f90a1	figures/combined-sparsity-plots.svg	/^							L79.7,70.7L79.7,70.7z"\/>$/;"	i
m6c0f888204	figures/combined-sparsity-plots.svg	/^							l-0.2,1.6l-0.2,0.3L79.7,70.7L79.7,70.7z"\/>$/;"	i
m6d284a5b47	figures/combined-sparsity-plots.svg	/^							l-0.2,0.2l-0.2-0.1l-0.2,0.3l-0.2,0.2v11.4H79.7z"\/>$/;"	i
m74c62d0820	figures/combined-sparsity-plots.svg	/^							l-0.2-0.1l-0.2-0.1l-0.2,0.2l-0.2-0.2l-0.2,0.2l-0.2-0.1l-0.2-0.1l-0.2,0.3L537,268h-0.2l-0./;"	i
m7bff4b254c	figures/combined-sparsity-plots.svg	/^							L80.9,69l-0.2,0.1l-0.2-0.5l-0.2-0.4l-0.2-0.5l-0.2,1.6l-0.2,0.2L79.7,70.6L79.7,70.6z"\/>$/;"	i
m8015dd74e0	figures/combined-sparsity-plots.svg	/^						<path id="m8015dd74e0" class="st21" d="M62.4,204.7h-3.5"\/>$/;"	i
m8015dd74e0_00000000931093273163489800000012352789729989289348_	figures/combined-sparsity-plots.svg	/^						<path id="m8015dd74e0_00000000931093273163489800000012352789729989289348_" class="st21" d=/;"	i
m8015dd74e0_00000000932498152566643320000005907681399047594684_	figures/combined-sparsity-plots.svg	/^						<path id="m8015dd74e0_00000000932498152566643320000005907681399047594684_" class="st21" d=/;"	i
m8015dd74e0_00000005949805995673902190000003288752697735765949_	figures/combined-sparsity-plots.svg	/^						<path id="m8015dd74e0_00000005949805995673902190000003288752697735765949_" class="st21" d=/;"	i
m8015dd74e0_00000028294783582533940740000004828707291088380559_	figures/combined-sparsity-plots.svg	/^						<path id="m8015dd74e0_00000028294783582533940740000004828707291088380559_" class="st21" d=/;"	i
m8015dd74e0_00000029012509151118585140000015778328540112644779_	figures/combined-sparsity-plots.svg	/^						<path id="m8015dd74e0_00000029012509151118585140000015778328540112644779_" class="st21" d=/;"	i
m8015dd74e0_00000052066442960383516250000003046180351081532319_	figures/combined-sparsity-plots.svg	/^						<path id="m8015dd74e0_00000052066442960383516250000003046180351081532319_" class="st21" d=/;"	i
m8015dd74e0_00000053508870736976264340000010844800601681222299_	figures/combined-sparsity-plots.svg	/^						<path id="m8015dd74e0_00000053508870736976264340000010844800601681222299_" class="st21" d=/;"	i
m8015dd74e0_00000059282675513453481660000006222629777125077687_	figures/combined-sparsity-plots.svg	/^						<path id="m8015dd74e0_00000059282675513453481660000006222629777125077687_" class="st21" d=/;"	i
m8015dd74e0_00000065793199511658937630000011811544586569023399_	figures/combined-sparsity-plots.svg	/^						<path id="m8015dd74e0_00000065793199511658937630000011811544586569023399_" class="st21" d=/;"	i
m8015dd74e0_00000073680165056241303780000010646455740910208191_	figures/combined-sparsity-plots.svg	/^						<path id="m8015dd74e0_00000073680165056241303780000010646455740910208191_" class="st21" d=/;"	i
m8015dd74e0_00000075131791466724773370000001417202486823493561_	figures/combined-sparsity-plots.svg	/^						<path id="m8015dd74e0_00000075131791466724773370000001417202486823493561_" class="st21" d=/;"	i
m8015dd74e0_00000078029831862456332620000015625651711376161943_	figures/combined-sparsity-plots.svg	/^						<path id="m8015dd74e0_00000078029831862456332620000015625651711376161943_" class="st21" d=/;"	i
m8015dd74e0_00000080198344978156014170000012978319367595397512_	figures/combined-sparsity-plots.svg	/^						<path id="m8015dd74e0_00000080198344978156014170000012978319367595397512_" class="st21" d=/;"	i
m8015dd74e0_00000113349995808961770710000017813192221230786193_	figures/combined-sparsity-plots.svg	/^						<path id="m8015dd74e0_00000113349995808961770710000017813192221230786193_" class="st21" d=/;"	i
m8015dd74e0_00000118389383800591071550000016756603990287482792_	figures/combined-sparsity-plots.svg	/^						<path id="m8015dd74e0_00000118389383800591071550000016756603990287482792_" class="st21" d=/;"	i
m8015dd74e0_00000121962047681193164270000010124399901121875852_	figures/combined-sparsity-plots.svg	/^						<path id="m8015dd74e0_00000121962047681193164270000010124399901121875852_" class="st21" d=/;"	i
m8015dd74e0_00000132790605403298266100000009918808190348712858_	figures/combined-sparsity-plots.svg	/^						<path id="m8015dd74e0_00000132790605403298266100000009918808190348712858_" class="st21" d=/;"	i
m8015dd74e0_00000145019346254463515750000011512797689692732824_	figures/combined-sparsity-plots.svg	/^						<path id="m8015dd74e0_00000145019346254463515750000011512797689692732824_" class="st21" d=/;"	i
m8015dd74e0_00000152236519602441752770000003485315440308189622_	figures/combined-sparsity-plots.svg	/^						<path id="m8015dd74e0_00000152236519602441752770000003485315440308189622_" class="st21" d=/;"	i
m80cdd7f65b	figures/combined-sparsity-plots.svg	/^							l-0.2,0.1l-0.2,0.3h-0.2l-0.2,0.2l-0.2,0.2v11.4H79.7z"\/>$/;"	i
m8126682fca_00000000223476045706802560000015455290717417112711_	figures/combined-sparsity-plots.svg	/^							l-0.2-0.6l-0.2,0.7C79.4,500.2,79.4,504.5,79.4,504.5z"\/>$/;"	i
m83f73f7393	figures/combined-sparsity-plots.svg	/^							h-0.2h-0.2H541h-0.2h-0.2h-0.2h-0.2H540h-0.2h-0.2h-0.2h-0.2H539h-0.2h-0.2h-0.2h-0.2H538h-0/;"	i
m8e803df09d	figures/combined-sparsity-plots.svg	/^							h-0.2h-0.2V258H536.2z"\/>$/;"	i
m8f87f6be4d	figures/combined-sparsity-plots.svg	/^							h-0.2l-0.2,0.1l-0.2-0.2v9H536.2z"\/>$/;"	i
m9344c1bcae	figures/combined-sparsity-plots.svg	/^							h-0.2l-0.2,0.2l-0.2,0.2V281H79.7z"\/>$/;"	i
m9347df166d	figures/combined-sparsity-plots.svg	/^							L518.5,504.1z"\/>$/;"	i
m952489e659	figures/combined-sparsity-plots.svg	/^							l-0.2,1.9l-0.2-0.8l-0.2-0.5l-0.2,0.1l-0.2-2.4l-0.2,0.2l-0.2-0.9l-0.2,0.7L518.4,504L518.4,/;"	i
m9645942640_00000085221871379598246360000013466415674172831130_	figures/combined-sparsity-plots.svg	/^						<path id="m9645942640_00000085221871379598246360000013466415674172831130_" class="st21" d=/;"	i
m9645942640_00000094585418090507190310000002887285633877522048_	figures/combined-sparsity-plots.svg	/^						<path id="m9645942640_00000094585418090507190310000002887285633877522048_" class="st21" d=/;"	i
m9645942640_00000109736606678948971490000007886178978915076738_	figures/combined-sparsity-plots.svg	/^						<path id="m9645942640_00000109736606678948971490000007886178978915076738_" class="st21" d=/;"	i
m9645942640_00000159469797743307850680000010706990788706651028_	figures/combined-sparsity-plots.svg	/^						<path id="m9645942640_00000159469797743307850680000010706990788706651028_" class="st21" d=/;"	i
m9931b7658f	figures/combined-sparsity-plots.svg	/^							l-0.5-2.4l-0.5,0.1l-0.5-1H521v4.7H518.7z"\/>$/;"	i
m9a6e787ceb_00000177445375497810464750000011749650616476519332_	figures/combined-sparsity-plots.svg	/^							C79.4,501,79.4,504.7,79.4,504.7z"\/>$/;"	i
m9f9714f9ef	figures/combined-sparsity-plots.svg	/^							l-0.2-0.5l-0.2,1.6l-0.2,0.3L79.7,70.6L79.7,70.6z"\/>$/;"	i
ma552581d60_00000016059843750172364030000008439503000296982691_	figures/combined-sparsity-plots.svg	/^						<path id="ma552581d60_00000016059843750172364030000008439503000296982691_" class="st21" d=/;"	i
ma552581d60_00000021828777026436760860000005544415205204282013_	figures/combined-sparsity-plots.svg	/^						<path id="ma552581d60_00000021828777026436760860000005544415205204282013_" class="st21" d=/;"	i
ma552581d60_00000085222233836425995130000001526662363467881919_	figures/combined-sparsity-plots.svg	/^						<path id="ma552581d60_00000085222233836425995130000001526662363467881919_" class="st21" d=/;"	i
ma552581d60_00000101792063330227225540000007564157314743851421_	figures/combined-sparsity-plots.svg	/^						<path id="ma552581d60_00000101792063330227225540000007564157314743851421_" class="st21" d=/;"	i
ma552581d60_00000124877939811824053910000017814028329751422081_	figures/combined-sparsity-plots.svg	/^						<path id="ma552581d60_00000124877939811824053910000017814028329751422081_" class="st21" d=/;"	i
ma552581d60_00000136403216243101548240000016145693205573512349_	figures/combined-sparsity-plots.svg	/^						<path id="ma552581d60_00000136403216243101548240000016145693205573512349_" class="st21" d=/;"	i
ma552581d60_00000181087649075806453940000002024905692972339868_	figures/combined-sparsity-plots.svg	/^						<path id="ma552581d60_00000181087649075806453940000002024905692972339868_" class="st21" d=/;"	i
ma5a4ea88c7_00000095325536599658550430000006667878953347470772_	figures/combined-sparsity-plots.svg	/^							l-0.2-0.5l-0.2,0.3l-1.4-2l-0.2,0.4l-0.2-0.9l-0.2,0.9C79.4,500.4,79.4,504.5,79.4,504.5z"\//;"	i
ma5b66f02b9	figures/combined-sparsity-plots.svg	/^							v0.7v-0.3v0.1v-0.5V69v-0.5v1.6v0.2v1.3H536.2z"\/>$/;"	i
maaa356109f_00000000187689340005213570000004840962673256997293_	figures/combined-sparsity-plots.svg	/^						<path id="maaa356109f_00000000187689340005213570000004840962673256997293_" class="st21" d=/;"	i
maaa356109f_00000002376703126915349390000014040624189270053762_	figures/combined-sparsity-plots.svg	/^						<path id="maaa356109f_00000002376703126915349390000014040624189270053762_" class="st21" d=/;"	i
maaa356109f_00000014628798526996815510000007358581342646741139_	figures/combined-sparsity-plots.svg	/^						<path id="maaa356109f_00000014628798526996815510000007358581342646741139_" class="st21" d=/;"	i
maaa356109f_00000056389061499784329820000002776810850895198865_	figures/combined-sparsity-plots.svg	/^						<path id="maaa356109f_00000056389061499784329820000002776810850895198865_" class="st21" d=/;"	i
maaa356109f_00000070824531293730052870000000472433356478060187_	figures/combined-sparsity-plots.svg	/^						<path id="maaa356109f_00000070824531293730052870000000472433356478060187_" class="st21" d=/;"	i
maaa356109f_00000129890030629787462830000017199924128927632302_	figures/combined-sparsity-plots.svg	/^						<path id="maaa356109f_00000129890030629787462830000017199924128927632302_" class="st21" d=/;"	i
maaa356109f_00000166666319588492797160000003330359079370367644_	figures/combined-sparsity-plots.svg	/^						<path id="maaa356109f_00000166666319588492797160000003330359079370367644_" class="st21" d=/;"	i
maaa356109f_00000181082647161791053370000006811531720499587513_	figures/combined-sparsity-plots.svg	/^						<path id="maaa356109f_00000181082647161791053370000006811531720499587513_" class="st21" d=/;"	i
maass1997networks	references.bib	/^@article{maass1997networks,$/;"	a
maass_Dynamic_1999	references.bib	/^@article{maass_Dynamic_1999,$/;"	a
maass_Model_2000	references.bib	/^@article{maass_Model_2000,$/;"	a
madc630dca7_00000024702553115505819230000004335717570573946254_	figures/combined-sparsity-plots.svg	/^						<path id="madc630dca7_00000024702553115505819230000004335717570573946254_" class="st21" d=/;"	i
madc630dca7_00000050659570149810790790000001644986861248676025_	figures/combined-sparsity-plots.svg	/^						<path id="madc630dca7_00000050659570149810790790000001644986861248676025_" class="st21" d=/;"	i
madc630dca7_00000088811339307848779400000016670310339710178697_	figures/combined-sparsity-plots.svg	/^						<path id="madc630dca7_00000088811339307848779400000016670310339710178697_" class="st21" d=/;"	i
madc630dca7_00000129904975160714267980000004463747790232065202_	figures/combined-sparsity-plots.svg	/^						<path id="madc630dca7_00000129904975160714267980000004463747790232065202_" class="st21" d=/;"	i
maly_Numerical_1996	references.bib	/^@article{maly_Numerical_1996,$/;"	a
marschall2020unified	references.bib	/^@article{marschall2020unified,$/;"	a
matplotlib.axis_1_00000045617760261074719580000011688372093688654773_	figures/combined-sparsity-plots.svg	/^	<g id="matplotlib.axis_1_00000045617760261074719580000011688372093688654773_">$/;"	i
matplotlib.axis_1_00000151513079703427368780000008394203640186897306_	figures/combined-sparsity-plots.svg	/^	<g id="matplotlib.axis_1_00000151513079703427368780000008394203640186897306_">$/;"	i
matplotlib.axis_2_00000006673029024178704320000004810978620561129139_	figures/combined-sparsity-plots.svg	/^	<g id="matplotlib.axis_2_00000006673029024178704320000004810978620561129139_">$/;"	i
matplotlib.axis_2_00000159453305834857522230000009771635608145318273_	figures/combined-sparsity-plots.svg	/^	<g id="matplotlib.axis_2_00000159453305834857522230000009771635608145318273_">$/;"	i
matplotlib.axis_3	figures/combined-sparsity-plots.svg	/^	<g id="matplotlib.axis_3">$/;"	i
matplotlib.axis_3_00000031188877303510865810000015304312226003624630_	figures/combined-sparsity-plots.svg	/^	<g id="matplotlib.axis_3_00000031188877303510865810000015304312226003624630_">$/;"	i
matplotlib.axis_4	figures/combined-sparsity-plots.svg	/^	<g id="matplotlib.axis_4">$/;"	i
matplotlib.axis_4_00000157299319282779849380000006197261979796089247_	figures/combined-sparsity-plots.svg	/^	<g id="matplotlib.axis_4_00000157299319282779849380000006197261979796089247_">$/;"	i
matplotlib.axis_5_00000134938204106806830620000013416262867024322195_	figures/combined-sparsity-plots.svg	/^<g id="matplotlib.axis_5_00000134938204106806830620000013416262867024322195_">$/;"	i
matplotlib.axis_5_00000161618562996711682880000015888119101887273888_	figures/combined-sparsity-plots.svg	/^	<g id="matplotlib.axis_5_00000161618562996711682880000015888119101887273888_">$/;"	i
matplotlib.axis_6_00000155833622813073201450000014455422093746527408_	figures/combined-sparsity-plots.svg	/^	<g id="matplotlib.axis_6_00000155833622813073201450000014455422093746527408_">$/;"	i
matplotlib.axis_7_00000072247231141641172580000003015681539874505867_	figures/combined-sparsity-plots.svg	/^	<g id="matplotlib.axis_7_00000072247231141641172580000003015681539874505867_">$/;"	i
matplotlib.axis_8_00000013909224877458621370000005315568150834135215_	figures/combined-sparsity-plots.svg	/^	<g id="matplotlib.axis_8_00000013909224877458621370000005315568150834135215_">$/;"	i
mazzia_EfficientCapsNet_2021	references.bib	/^@article{mazzia_EfficientCapsNet_2021,$/;"	a
mb667d0581f	figures/combined-sparsity-plots.svg	/^							v-0.2v0.5v-0.7v0.7V70l0,0v-0.5v-0.4v-0.5v1.6v0.3v1.1H536.2z"\/>$/;"	i
mbeef9c9c50	figures/combined-sparsity-plots.svg	/^							l-0.2-0.3l-0.2-0.5L80,69.7l-0.2,0.1v0.8H79.7z"\/>$/;"	i
mc922f3b2a6_00000060031506191791902680000007556704778509757614_	figures/combined-sparsity-plots.svg	/^							l-0.2,0.3l-0.2-1.1l-0.2,0.8l-0.2-0.3l-0.2-0.5l-0.2,0.1l-0.2-2.1l-0.2,0.2l-0.2-0.4l-0.2,0./;"	i
mca02cb2f21_00000183243911940964262420000017084704285714883212_	figures/combined-sparsity-plots.svg	/^							l-0.2-0.6l-0.2,0.1l-0.2-2.4l-0.2,0.1l-0.2-1h-0.2L79.4,504.2L79.4,504.2z"\/>$/;"	i
mca98eb8487	figures/combined-sparsity-plots.svg	/^							l-0.4,0.1l-0.4-2.1l-0.4,0.2l-0.4-0.4l-0.4,0.2v3.3H518.6z"\/>$/;"	i
mce1a5b8f95	figures/combined-sparsity-plots.svg	/^							l-0.2-0.3V295H536.2z"\/>$/;"	i
md5934e744c	figures/combined-sparsity-plots.svg	/^							h-0.2H539h-0.2h-0.2l-0.2-0.1h-0.2H538h-0.2h-0.2l-0.2,0.1h-0.2l-0.2,0.1h-0.2v2.9H536.2z"\//;"	i
md6b1875940	figures/combined-sparsity-plots.svg	/^							l-0.2,0.1l-0.2-0.1l-0.2-0.1H82l-0.2-0.1h-0.2h-0.2h-0.2H81l-0.2,0.1l-0.2,0.1h-0.2l-0.2,0.3/;"	i
mdd90a137d3	figures/combined-sparsity-plots.svg	/^							v-0.6v0.6v-0.3l0,0v-0.5v-0.3v-0.5v1.6V71v0.7H536.2z"\/>$/;"	i
mead2020we	references.bib	/^@article{mead2020we,$/;"	a
meb6341b9b3	figures/combined-sparsity-plots.svg	/^							l-0.2,0.1l-0.2,0.1H81l-0.2,0.2l-0.2,0.3h-0.2l-0.2,0.3l-0.2,0.2v10.7H79.7z"\/>$/;"	i
med212bdbfa	figures/combined-sparsity-plots.svg	/^							l-0.2-0.1l-0.2-0.1h-0.2h-0.2l-0.2-0.1l-0.2,0.1H81h-0.2l-0.2,0.1l-0.2,0.1h-0.2l-0.2,0.2l-0/;"	i
menick2020practicala	references.bib	/^@inproceedings{menick2020practicala,$/;"	j
menick_Practical_2020	references.bib	/^@inproceedings{menick_Practical_2020,$/;"	j
merity_Regularizing_2017	references.bib	/^@article{merity_Regularizing_2017,$/;"	a
merity_Single_2019	references.bib	/^@article{merity_Single_2019,$/;"	a
metadata143462	figures/pseudo-derivative.svg	/^     id="metadata143462">$/;"	i
mf0fde266b6	figures/combined-sparsity-plots.svg	/^							\/>$/;"	i
mf23151f34d	figures/combined-sparsity-plots.svg	/^							l-0.2,0.2l-0.2-0.1h-0.2H82l-0.2,0.1h-0.2l-0.2,0.1h-0.2H81l-0.2,0.2l-0.2,0.2h-0.2l-0.2,0.2/;"	i
mfbb94d438a	figures/combined-sparsity-plots.svg	/^							h-0.2v6.3H536.2z"\/>$/;"	i
mfc0814b2f7	figures/combined-sparsity-plots.svg	/^							l-0.2,0.2l-0.2,0.1l-0.2,0.2l-0.2,0.2v10.9H79.7z"\/>$/;"	i
mfc1e645a43_00000128474376657066934830000009004097364825370540_	figures/combined-sparsity-plots.svg	/^							l-0.2-2.3l-0.2,0.1l-0.2-0.9l-0.2,0.6v4.3H79.4z"\/>$/;"	i
mfd2f771708	figures/combined-sparsity-plots.svg	/^							h-0.2H82h-0.2h-0.2h-0.2h-0.2H81l-0.2,0.1l-0.2,0.2l-0.2-0.1l-0.2,0.3l-0.2,0.2v10.3H79.7z"\//;"	i
mnih_Recurrent_2014	references.bib	/^@incollection{mnih_Recurrent_2014,$/;"	I
mostafa_Supervised_2018	references.bib	/^@article{mostafa_Supervised_2018,$/;"	a
narang2017exploring	references.bib	/^@misc{narang2017exploring,$/;"	n
neil_Delta_2017	references.bib	/^@inproceedings{neil_Delta_2017,$/;"	j
neil_Phased_2016	references.bib	/^@article{neil_Phased_2016,$/;"	a
ns3e2cd9b30101	figures/combined-sparsity-plots.svg	/^	 viewBox="0 0 928 657" style="enable-background:new 0 0 928 657;" xml:space="preserve">$/;"	n	uri:http://www.w3.org/2000/svg
nse618eb570101	figures/pseudo-derivative.svg	/^   xmlns:dc="http:\/\/purl.org\/dc\/elements\/1.1\/">$/;"	n	uri:http://www.w3.org/2000/svg
nvidia-2-4	references.bib	/^@misc{nvidia-2-4,$/;"	n
oord_Pixel_2016	references.bib	/^@article{oord_Pixel_2016,$/;"	a
ostraubenchmarking	references.bib	/^@article{ostraubenchmarking,$/;"	a
patch_10_00000168815152893751345520000006765394761862482068_	figures/combined-sparsity-plots.svg	/^	<g id="patch_10_00000168815152893751345520000006765394761862482068_">$/;"	i
patch_11_00000044856672496058375010000014429425074914685347_	figures/combined-sparsity-plots.svg	/^	<g id="patch_11_00000044856672496058375010000014429425074914685347_">$/;"	i
patch_12_00000054230672997460131410000004521728404820312221_	figures/combined-sparsity-plots.svg	/^	<g id="patch_12_00000054230672997460131410000004521728404820312221_">$/;"	i
patch_13_00000078728630341152388610000013313778229207310497_	figures/combined-sparsity-plots.svg	/^	<g id="patch_13_00000078728630341152388610000013313778229207310497_">$/;"	i
patch_14	figures/combined-sparsity-plots.svg	/^		<g id="patch_14">$/;"	i
patch_2_00000090978973447733739000000005364042209492194189_	figures/combined-sparsity-plots.svg	/^	<g id="patch_2_00000090978973447733739000000005364042209492194189_">$/;"	i
patch_2_00000159459648235149272480000013805719130748496831_	figures/combined-sparsity-plots.svg	/^	<g id="patch_2_00000159459648235149272480000013805719130748496831_">$/;"	i
patch_3_00000011005841439911315690000012930866142980482490_	figures/combined-sparsity-plots.svg	/^	<g id="patch_3_00000011005841439911315690000012930866142980482490_">$/;"	i
patch_3_00000044137625169309984870000005714331714860195985_	figures/combined-sparsity-plots.svg	/^	<g id="patch_3_00000044137625169309984870000005714331714860195985_">$/;"	i
patch_4_00000053520517696397605910000017208814097764520094_	figures/combined-sparsity-plots.svg	/^	<g id="patch_4_00000053520517696397605910000017208814097764520094_">$/;"	i
patch_4_00000098903603983431674380000010059745292619883938_	figures/combined-sparsity-plots.svg	/^	<g id="patch_4_00000098903603983431674380000010059745292619883938_">$/;"	i
patch_5	figures/combined-sparsity-plots.svg	/^	<g id="patch_5">$/;"	i
patch_5_00000091727298459224528350000018144922608232504707_	figures/combined-sparsity-plots.svg	/^	<g id="patch_5_00000091727298459224528350000018144922608232504707_">$/;"	i
patch_6	figures/combined-sparsity-plots.svg	/^	<g id="patch_6">$/;"	i
patch_6_00000176759145425845747570000005526178996771384215_	figures/combined-sparsity-plots.svg	/^	<g id="patch_6_00000176759145425845747570000005526178996771384215_">$/;"	i
patch_7	figures/combined-sparsity-plots.svg	/^	<g id="patch_7">$/;"	i
patch_7_00000147188597241473394080000003334635069798142608_	figures/combined-sparsity-plots.svg	/^	<g id="patch_7_00000147188597241473394080000003334635069798142608_">$/;"	i
patch_8_00000159459803216050946340000009745620771150395030_	figures/combined-sparsity-plots.svg	/^	<g id="patch_8_00000159459803216050946340000009745620771150395030_">$/;"	i
patch_9_00000085968862334469806060000012803792224422568625_	figures/combined-sparsity-plots.svg	/^	<g id="patch_9_00000085968862334469806060000012803792224422568625_">$/;"	i
path12009	figures/pseudo-derivative.svg	/^       id="path12009" \/>$/;"	i
path12009-0	figures/pseudo-derivative.svg	/^       id="path12009-0" \/>$/;"	i
path1424	figures/pseudo-derivative.svg	/^       sodipodi:nodetypes="ccccc" \/>$/;"	i
path1424-1	figures/pseudo-derivative.svg	/^       sodipodi:nodetypes="cccc" \/>$/;"	i
path1424-1-1	figures/pseudo-derivative.svg	/^       sodipodi:nodetypes="cccc" \/>$/;"	i
path1424-8	figures/pseudo-derivative.svg	/^       sodipodi:nodetypes="ccccc" \/>$/;"	i
path144021-6-5-0-03-23	figures/pseudo-derivative.svg	/^       r="3.5395234" \/>$/;"	i
path144021-6-5-0-03-23-0	figures/pseudo-derivative.svg	/^       r="3.5395234" \/>$/;"	i
path144021-6-5-0-03-3	figures/pseudo-derivative.svg	/^       r="3.5395234" \/>$/;"	i
path144021-6-5-0-03-3-3	figures/pseudo-derivative.svg	/^       r="3.5395234" \/>$/;"	i
path144021-6-5-0-03-3-3-5	figures/pseudo-derivative.svg	/^       r="3.5395234" \/>$/;"	i
path144021-6-5-0-03-3-7	figures/pseudo-derivative.svg	/^       r="3.5395234" \/>$/;"	i
path144021-6-5-0-03-3-80	figures/pseudo-derivative.svg	/^       r="3.5395234" \/>$/;"	i
path144021-6-5-0-03-3-80-0	figures/pseudo-derivative.svg	/^       r="3.5395234" \/>$/;"	i
path144021-6-5-0-03-3-80-0-5	figures/pseudo-derivative.svg	/^       r="3.5395234" \/>$/;"	i
path144021-6-5-0-03-3-80-9	figures/pseudo-derivative.svg	/^       r="3.5395234" \/>$/;"	i
path144021-6-5-0-03-4	figures/pseudo-derivative.svg	/^       r="3.5395234" \/>$/;"	i
path144021-6-5-0-03-4-2	figures/pseudo-derivative.svg	/^       r="3.5395234" \/>$/;"	i
path144021-6-5-0-03-4-2-0	figures/pseudo-derivative.svg	/^       r="3.5395234" \/>$/;"	i
path144021-6-5-0-03-4-2-2	figures/pseudo-derivative.svg	/^       r="3.5395234" \/>$/;"	i
path144021-6-5-0-03-4-2-2-8	figures/pseudo-derivative.svg	/^       r="3.5395234" \/>$/;"	i
path144021-6-5-0-03-4-8	figures/pseudo-derivative.svg	/^       r="3.5395234" \/>$/;"	i
path145772-2-3-2-0-8-3	figures/pseudo-derivative.svg	/^       inkscape:connector-curvature="0" \/>$/;"	i
path145772-2-3-2-0-8-3-8	figures/pseudo-derivative.svg	/^       inkscape:connector-curvature="0" \/>$/;"	i
path145772-2-3-2-0-8-3-8-2	figures/pseudo-derivative.svg	/^       inkscape:connector-curvature="0" \/>$/;"	i
path145772-2-3-2-0-8-3-8-5	figures/pseudo-derivative.svg	/^       inkscape:connector-curvature="0" \/>$/;"	i
path145772-2-3-2-0-8-3-8-5-2	figures/pseudo-derivative.svg	/^       inkscape:connector-curvature="0" \/>$/;"	i
path145772-2-3-2-0-8-3-8-5-4	figures/pseudo-derivative.svg	/^       inkscape:connector-curvature="0" \/>$/;"	i
path145772-2-3-2-0-8-3-8-5-4-0	figures/pseudo-derivative.svg	/^       inkscape:connector-curvature="0" \/>$/;"	i
path145772-2-3-2-0-8-3-81	figures/pseudo-derivative.svg	/^       inkscape:connector-curvature="0" \/>$/;"	i
path145772-2-3-2-0-8-8-1	figures/pseudo-derivative.svg	/^       inkscape:connector-curvature="0" \/>$/;"	i
path145772-2-3-2-0-8-8-1-3	figures/pseudo-derivative.svg	/^       inkscape:connector-curvature="0" \/>$/;"	i
path145772-2-3-2-0-8-8-1-6	figures/pseudo-derivative.svg	/^       inkscape:connector-curvature="0" \/>$/;"	i
path145772-2-3-2-0-8-8-1-6-2	figures/pseudo-derivative.svg	/^       inkscape:connector-curvature="0" \/>$/;"	i
path145772-2-3-2-0-8-8-1-6-2-1	figures/pseudo-derivative.svg	/^       inkscape:connector-curvature="0" \/>$/;"	i
path145772-2-3-2-0-8-8-1-6-2-1-8	figures/pseudo-derivative.svg	/^       inkscape:connector-curvature="0" \/>$/;"	i
path145772-2-3-2-0-8-8-1-6-2-2	figures/pseudo-derivative.svg	/^       inkscape:connector-curvature="0" \/>$/;"	i
path145772-2-3-2-0-8-8-1-6-5	figures/pseudo-derivative.svg	/^       inkscape:connector-curvature="0" \/>$/;"	i
path1461	figures/pseudo-derivative.svg	/^       inkscape:connector-curvature="0" \/>$/;"	i
path1461-1	figures/pseudo-derivative.svg	/^       inkscape:connector-curvature="0" \/>$/;"	i
path1461-3	figures/pseudo-derivative.svg	/^       inkscape:connector-curvature="0" \/>$/;"	i
path1461-3-7	figures/pseudo-derivative.svg	/^       inkscape:connector-curvature="0" \/>$/;"	i
path1461-5	figures/pseudo-derivative.svg	/^       inkscape:connector-curvature="0" \/>$/;"	i
path1461-5-4	figures/pseudo-derivative.svg	/^       inkscape:export-ydpi="299" \/>$/;"	i
path1461-5-6	figures/pseudo-derivative.svg	/^       inkscape:connector-curvature="0" \/>$/;"	i
path1461-5-6-1	figures/pseudo-derivative.svg	/^       inkscape:connector-curvature="0" \/>$/;"	i
path148205-5-6	figures/pseudo-derivative.svg	/^       inkscape:connector-curvature="0" \/>$/;"	i
path148205-5-6-5	figures/pseudo-derivative.svg	/^       inkscape:connector-curvature="0" \/>$/;"	i
path148205-5-6-7	figures/pseudo-derivative.svg	/^       inkscape:connector-curvature="0" \/>$/;"	i
path148205-5-6-7-3	figures/pseudo-derivative.svg	/^       inkscape:connector-curvature="0" \/>$/;"	i
path148205-5-6-7-3-8	figures/pseudo-derivative.svg	/^       inkscape:connector-curvature="0" \/>$/;"	i
path148205-5-6-7-3-9	figures/pseudo-derivative.svg	/^       inkscape:connector-curvature="0" \/>$/;"	i
path148205-5-6-7-3-9-9	figures/pseudo-derivative.svg	/^       inkscape:connector-curvature="0" \/>$/;"	i
path148205-5-6-7-7	figures/pseudo-derivative.svg	/^       inkscape:connector-curvature="0" \/>$/;"	i
path148205-5-6-9	figures/pseudo-derivative.svg	/^       inkscape:connector-curvature="0" \/>$/;"	i
path148205-5-6-9-6	figures/pseudo-derivative.svg	/^       inkscape:connector-curvature="0" \/>$/;"	i
path148205-5-6-9-6-9	figures/pseudo-derivative.svg	/^       inkscape:connector-curvature="0" \/>$/;"	i
path148205-5-6-9-6-9-0	figures/pseudo-derivative.svg	/^       inkscape:connector-curvature="0" \/>$/;"	i
path148205-5-6-9-6-9-0-0	figures/pseudo-derivative.svg	/^       inkscape:connector-curvature="0" \/>$/;"	i
path148205-5-6-9-6-9-0-0-0	figures/pseudo-derivative.svg	/^       inkscape:connector-curvature="0" \/>$/;"	i
path148205-5-6-9-6-9-0-5	figures/pseudo-derivative.svg	/^       inkscape:connector-curvature="0" \/>$/;"	i
path148205-5-6-9-6-9-05	figures/pseudo-derivative.svg	/^       inkscape:connector-curvature="0" \/>$/;"	i
path148205-5-6-9-9	figures/pseudo-derivative.svg	/^       inkscape:connector-curvature="0" \/>$/;"	i
path148205-5-6-9-9-0	figures/pseudo-derivative.svg	/^       inkscape:connector-curvature="0" \/>$/;"	i
path148205-9	figures/pseudo-derivative.svg	/^       inkscape:connector-curvature="0" \/>$/;"	i
path148205-9-6	figures/pseudo-derivative.svg	/^       inkscape:connector-curvature="0" \/>$/;"	i
path148205-9-9	figures/pseudo-derivative.svg	/^       inkscape:connector-curvature="0" \/>$/;"	i
path148205-9-9-3	figures/pseudo-derivative.svg	/^       inkscape:connector-curvature="0" \/>$/;"	i
path148205-9-9-5	figures/pseudo-derivative.svg	/^       sodipodi:nodetypes="cc" \/>$/;"	i
path148205-9-9-5-6	figures/pseudo-derivative.svg	/^       sodipodi:nodetypes="cc" \/>$/;"	i
path1524	figures/pseudo-derivative.svg	/^         sodipodi:nodetypes="ccscscccscsscccscscccscssc" \/>$/;"	i
path1531	figures/pseudo-derivative.svg	/^       inkscape:connector-curvature="0" \/>$/;"	i
path1531-4	figures/pseudo-derivative.svg	/^       inkscape:connector-curvature="0" \/>$/;"	i
path155664-0-2-1-2-2	figures/pseudo-derivative.svg	/^       inkscape:transform-center-y="-28.549742" \/>$/;"	i
path155664-0-2-1-2-8-0	figures/pseudo-derivative.svg	/^       inkscape:transform-center-y="36.105224" \/>$/;"	i
path155664-0-2-1-2-8-0-1	figures/pseudo-derivative.svg	/^       inkscape:transform-center-y="36.105224" \/>$/;"	i
path155664-0-2-1-2-8-0-1-4	figures/pseudo-derivative.svg	/^       inkscape:transform-center-y="36.105224" \/>$/;"	i
path155664-0-2-1-22-5	figures/pseudo-derivative.svg	/^       sodipodi:nodetypes="cc" \/>$/;"	i
path155664-0-2-1-22-5-5	figures/pseudo-derivative.svg	/^       sodipodi:nodetypes="cc" \/>$/;"	i
path155664-0-2-1-22-5-5-4	figures/pseudo-derivative.svg	/^       sodipodi:nodetypes="cc" \/>$/;"	i
path155664-0-2-1-22-5-5-4-2-3	figures/pseudo-derivative.svg	/^       sodipodi:nodetypes="cc" \/>$/;"	i
path155664-0-2-1-22-5-5-7-5	figures/pseudo-derivative.svg	/^       sodipodi:nodetypes="cc" \/>$/;"	i
path155664-0-2-1-22-5-7	figures/pseudo-derivative.svg	/^       sodipodi:nodetypes="cc" \/>$/;"	i
path155664-0-2-1-22-5-7-6	figures/pseudo-derivative.svg	/^       sodipodi:nodetypes="cc" \/>$/;"	i
path155664-0-2-1-28-0-6	figures/pseudo-derivative.svg	/^       sodipodi:nodetypes="cc" \/>$/;"	i
path155664-0-2-1-28-0-6-2	figures/pseudo-derivative.svg	/^       sodipodi:nodetypes="cc" \/>$/;"	i
path155664-0-2-1-28-0-6-2-8	figures/pseudo-derivative.svg	/^       sodipodi:nodetypes="cc" \/>$/;"	i
path155664-0-2-1-28-0-6-9	figures/pseudo-derivative.svg	/^       sodipodi:nodetypes="cc" \/>$/;"	i
path155664-0-2-1-28-0-6-9-3-4	figures/pseudo-derivative.svg	/^       sodipodi:nodetypes="cc" \/>$/;"	i
path155664-0-2-1-28-0-6-9-9	figures/pseudo-derivative.svg	/^       sodipodi:nodetypes="cc" \/>$/;"	i
path155664-0-2-1-28-0-6-9-9-9-9	figures/pseudo-derivative.svg	/^       sodipodi:nodetypes="cc" \/>$/;"	i
path155664-0-2-1-28-5	figures/pseudo-derivative.svg	/^       inkscape:transform-center-y="11.484327" \/>$/;"	i
path155664-0-2-4-2	figures/pseudo-derivative.svg	/^       inkscape:transform-center-y="5.0384266" \/>$/;"	i
path155664-0-2-4-7-0	figures/pseudo-derivative.svg	/^       sodipodi:nodetypes="cc" \/>$/;"	i
path155664-0-2-4-7-0-3	figures/pseudo-derivative.svg	/^       sodipodi:nodetypes="cc" \/>$/;"	i
path155664-0-2-4-7-0-3-0	figures/pseudo-derivative.svg	/^       sodipodi:nodetypes="cc" \/>$/;"	i
path155664-0-2-4-7-0-9	figures/pseudo-derivative.svg	/^       sodipodi:nodetypes="cc" \/>$/;"	i
path155664-0-2-4-7-0-9-1-6	figures/pseudo-derivative.svg	/^       sodipodi:nodetypes="cc" \/>$/;"	i
path155664-0-2-4-7-0-9-9	figures/pseudo-derivative.svg	/^       sodipodi:nodetypes="cc" \/>$/;"	i
path155664-0-2-4-7-0-9-9-2-7	figures/pseudo-derivative.svg	/^       sodipodi:nodetypes="cc" \/>$/;"	i
path155664-0-2-5-8	figures/pseudo-derivative.svg	/^       sodipodi:nodetypes="cc" \/>$/;"	i
path155664-0-2-5-8-1	figures/pseudo-derivative.svg	/^       sodipodi:nodetypes="cc" \/>$/;"	i
path155664-0-2-5-8-1-3-7	figures/pseudo-derivative.svg	/^       sodipodi:nodetypes="cc" \/>$/;"	i
path155664-0-2-5-8-1-4	figures/pseudo-derivative.svg	/^       sodipodi:nodetypes="cc" \/>$/;"	i
path155664-0-2-5-8-1-4-0-6	figures/pseudo-derivative.svg	/^       sodipodi:nodetypes="cc" \/>$/;"	i
path155664-0-2-5-8-3	figures/pseudo-derivative.svg	/^       sodipodi:nodetypes="cc" \/>$/;"	i
path155664-0-2-5-8-3-0	figures/pseudo-derivative.svg	/^       sodipodi:nodetypes="cc" \/>$/;"	i
path155664-0-2-9-2	figures/pseudo-derivative.svg	/^       inkscape:transform-center-y="-13.430046" \/>$/;"	i
path155664-0-2-9-6-1	figures/pseudo-derivative.svg	/^       inkscape:transform-center-y="17.201766" \/>$/;"	i
path155664-0-2-9-6-1-8	figures/pseudo-derivative.svg	/^       inkscape:transform-center-y="17.201766" \/>$/;"	i
path155664-0-2-9-6-1-8-5	figures/pseudo-derivative.svg	/^       inkscape:transform-center-y="17.201766" \/>$/;"	i
path155664-0-8	figures/pseudo-derivative.svg	/^       sodipodi:nodetypes="cc" \/>$/;"	i
path155664-0-9-5	figures/pseudo-derivative.svg	/^       sodipodi:nodetypes="cc" \/>$/;"	i
path155664-0-9-5-3	figures/pseudo-derivative.svg	/^       sodipodi:nodetypes="cc" \/>$/;"	i
path155664-0-9-5-3-7	figures/pseudo-derivative.svg	/^       sodipodi:nodetypes="cc" \/>$/;"	i
path155664-1-0	figures/pseudo-derivative.svg	/^       sodipodi:nodetypes="cc" \/>$/;"	i
path155664-1-0-0	figures/pseudo-derivative.svg	/^       sodipodi:nodetypes="cc" \/>$/;"	i
path155664-1-0-0-5	figures/pseudo-derivative.svg	/^       sodipodi:nodetypes="cc" \/>$/;"	i
path155664-7	figures/pseudo-derivative.svg	/^       sodipodi:nodetypes="cc" \/>$/;"	i
path61560	figures/pseudo-derivative.svg	/^         transform="scale(0.6) rotate(180) translate(0,0)" \/>$/;"	i
path61560-0	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-2	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-0	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-0-0	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-0-08	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-0-4	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-0-4-0	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-0-4-4	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-0-4-48	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-0-4-48-2	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-0-4-48-3	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-0-4-48-3-1	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-0-4-7	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-0-4-8	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-0-43	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-0-43-1	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-0-43-5	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-0-43-6	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-0-43-7	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-0-43-7-6	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-0-43-74	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-0-45	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-3	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-3-0	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-3-4	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-3-7	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-3-7-6	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-3-7-6-8	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-3-7-6-8-1	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-3-7-6-8-1-9	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-3-7-6-8-1-9-1	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-3-7-6-8-18	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-3-7-6-8-18-7	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-3-7-6-8-2	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-3-7-6-8-2-7	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-3-7-6-8-2-7-7	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-3-7-6-9	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-3-7-6-9-9	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-3-8	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-3-9	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-5	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-5-2	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-5-3	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-5-9	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-5-9-1	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-6	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-6-2	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-6-6	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-6-8	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-6-8-2	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-6-8-6	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-6-8-6-4	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-6-9	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-6-93	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-7	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-5-8	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-57	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-57-8	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-57-8-8	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-57-8-8-7	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-57-8-8-74	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-57-8-8-74-2	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-57-8-8-74-5	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-57-8-8-74-6	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-57-8-8-74-6-0	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-57-8-8-74-6-4	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-57-8-8-74-6-9	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-57-8-8-74-63	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-57-8-8-74-63-0	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-57-8-8-74-63-0-5	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-57-8-8-74-63-0-6	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-57-8-8-74-63-5	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-57-8-8-74-63-6	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-57-8-8-74-63-68	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-57-8-8-74-63-9	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-57-8-8-74-63-9-2	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-57-8-8-74-63-9-3	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-57-8-8-74-63-9-7	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-57-8-8-74-63-9-78	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-57-8-8-74-63-9-78-3	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-57-8-8-74-63-9-78-5	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-57-8-8-74-63-9-78-7	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-57-8-8-74-63-9-78-7-5	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-57-8-8-74-63-9-78-7-8	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-57-8-8-74-63-9-78-7-8-2	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-57-8-8-74-63-9-78-7-83	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-57-8-8-74-63-9-8	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-57-8-8-74-7	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-57-8-8-74-72	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-57-8-8-74-72-0	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-57-8-8-74-72-09	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-57-8-8-74-72-9	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-57-8-8-74-8	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-57-8-8-74-8-0	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-57-8-8-74-8-5	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-57-8-8-74-83	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-57-8-8-74-9	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-57-8-8-74-9-3	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-57-8-8-74-9-3-2	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-57-8-8-74-9-3-2-6	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-57-8-8-74-9-3-2-6-5	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-57-8-8-74-9-3-2-8	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-57-8-8-74-9-3-2-83	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-57-8-8-74-9-3-4	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-57-8-8-74-9-3-6	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-57-8-8-74-9-4	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-57-8-8-74-9-6	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-57-8-8-74-9-64	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-57-8-8-74-9-8	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-6	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-6-6	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-6-6-8	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-2	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-2-0	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-2-0-0	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-2-0-0-0	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-2-0-0-2	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-2-0-2	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-2-0-5	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-2-0-7	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-2-0-9	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-2-2	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-2-24	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-2-7	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-2-7-1	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-2-7-1-1	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-2-9	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-4	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-5	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-5-2	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-5-4	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-5-4-5	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-5-4-55	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-5-4-55-0	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-5-4-55-0-0	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-5-4-55-0-0-4	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-5-4-55-0-6	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-5-4-55-7	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-5-4-8	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-5-8	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-5-8-1	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-5-8-2	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-5-8-20	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-5-8-28	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-5-8-4	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-5-8-4-0	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-5-8-4-7	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-5-8-4-7-7	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-5-8-5	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-5-8-5-1	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-5-8-5-5	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-5-8-5-55	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-5-8-54	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-5-8-54-2	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-5-8-54-9	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-5-8-54-9-2	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-5-8-54-9-2-8	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-5-8-54-9-3	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-5-8-8	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-5-9	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-5-91	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-5-91-9	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-57	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-57-2	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-57-8	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-8-7-4-7-9-9	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-88	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-88-0	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-88-2	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-88-3	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-88-3-0	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-88-3-0-1	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-88-3-0-7	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-88-3-0-9	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-88-3-2	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-88-3-5	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-88-3-55	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-88-34	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-9	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-9-7	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
path61560-9-7-0	figures/pseudo-derivative.svg	/^         transform="scale(-0.6)" \/>$/;"	i
perez-nieves_Sparse_2021	references.bib	/^@article{perez-nieves_Sparse_2021,$/;"	a
petrovici_Pattern_2017	references.bib	/^@inproceedings{petrovici_Pattern_2017,$/;"	j
pontryagin1962mathematical	references.bib	/^@book{pontryagin1962mathematical,$/;"	b
proposition	main.tex	/^\\newtheorem{proposition}{Proposition}$/;"	t
pytorch	references.bib	/^@incollection{pytorch,$/;"	I
ramesh2022hierarchical	references.bib	/^@article{ramesh2022hierarchical,$/;"	a
ramesh_ZeroShot_2021	references.bib	/^@article{ramesh_ZeroShot_2021,$/;"	a
rdf	figures/pseudo-derivative.svg	/^   xmlns:dc="http:\/\/purl.org\/dc\/elements\/1.1\/">$/;"	n	uri:http://www.w3.org/1999/02/22-rdf-syntax-ns#
rect145758-0-1-9-0	figures/pseudo-derivative.svg	/^       ry="0" \/>$/;"	i
rect145758-0-1-9-0-3	figures/pseudo-derivative.svg	/^       ry="0" \/>$/;"	i
rect145758-0-1-9-0-3-9	figures/pseudo-derivative.svg	/^       ry="0" \/>$/;"	i
rect145758-0-1-9-0-3-9-5	figures/pseudo-derivative.svg	/^       transform="scale(-1,1)" \/>$/;"	i
rect145758-0-1-9-0-6	figures/pseudo-derivative.svg	/^       ry="0" \/>$/;"	i
rect145758-0-1-9-0-6-6	figures/pseudo-derivative.svg	/^       ry="0" \/>$/;"	i
rect145758-0-1-9-0-6-6-8	figures/pseudo-derivative.svg	/^       ry="0" \/>$/;"	i
rect145758-0-1-9-0-6-7	figures/pseudo-derivative.svg	/^       ry="0" \/>$/;"	i
rect145758-0-1-9-0-9	figures/pseudo-derivative.svg	/^       ry="0" \/>$/;"	i
rect145758-0-1-9-1	figures/pseudo-derivative.svg	/^       ry="0" \/>$/;"	i
rect145758-0-1-9-1-1	figures/pseudo-derivative.svg	/^       ry="0" \/>$/;"	i
rect145758-0-1-9-1-1-3	figures/pseudo-derivative.svg	/^       ry="0" \/>$/;"	i
rect145758-0-1-9-1-1-7	figures/pseudo-derivative.svg	/^       ry="0" \/>$/;"	i
rect145758-0-1-9-1-1-7-4	figures/pseudo-derivative.svg	/^       ry="0" \/>$/;"	i
rect145758-0-1-9-1-2	figures/pseudo-derivative.svg	/^       ry="0" \/>$/;"	i
rect145758-0-1-9-4	figures/pseudo-derivative.svg	/^       ry="0" \/>$/;"	i
rect145758-0-1-9-4-9	figures/pseudo-derivative.svg	/^       ry="0" \/>$/;"	i
rect191940-5-8	figures/pseudo-derivative.svg	/^       y="107.13273" \/>$/;"	i
rect191940-5-8-3	figures/pseudo-derivative.svg	/^       y="107.13273" \/>$/;"	i
rect191940-7	figures/pseudo-derivative.svg	/^       y="82.972511" \/>$/;"	i
rect191940-7-2	figures/pseudo-derivative.svg	/^       y="82.972511" \/>$/;"	i
rect33189	figures/pseudo-derivative.svg	/^       y="0.60135907" \/>$/;"	i
roy2019towards	references.bib	/^@article{roy2019towards,$/;"	a
rozenwasser_sensitivity_2019	references.bib	/^@book{rozenwasser_sensitivity_2019,$/;"	b
rusch2021coupled	references.bib	/^@article{rusch2021coupled,$/;"	a
sabour_Dynamic_2017	references.bib	/^@inproceedings{sabour_Dynamic_2017,$/;"	j
salaj_Spike_2021	references.bib	/^@article{salaj_Spike_2021,$/;"	a
schaefer2022aegnn	references.bib	/^@article{schaefer2022aegnn,$/;"	a
schafer2006recurrent	references.bib	/^@inproceedings{schafer2006recurrent,$/;"	j
schuman2017survey	references.bib	/^@article{schuman2017survey,$/;"	a
sec:discussion	main.tex	/^\\section{Discussion}\\label{sec:discussion}$/;"	l
sec:introduction	main.tex	/^\\label{sec:introduction}$/;"	l
serban_sensitivity_2019	references.bib	/^@article{serban_sensitivity_2019,$/;"	a
shazeer_Outrageously_2017	references.bib	/^@article{shazeer_Outrageously_2017,$/;"	a
shrestha_Robust_2017a	references.bib	/^@article{shrestha_Robust_2017a,$/;"	a
siegelmann_Computational_1995	references.bib	/^@article{siegelmann_Computational_1995,$/;"	a
sodipodi	figures/pseudo-derivative.svg	/^   xmlns:dc="http:\/\/purl.org\/dc\/elements\/1.1\/">$/;"	n	uri:http://sodipodi.sourceforge.net/DTD/sodipodi-0.dtd
subramoney2022egru	references.bib	/^@misc{subramoney2022egru,$/;"	n
svg	figures/pseudo-derivative.svg	/^   xmlns:dc="http:\/\/purl.org\/dc\/elements\/1.1\/">$/;"	n	uri:http://www.w3.org/2000/svg
svg143465	figures/pseudo-derivative.svg	/^   xmlns:dc="http:\/\/purl.org\/dc\/elements\/1.1\/">$/;"	i
tab:cost-comparison	main.tex	/^\\label{tab:cost-comparison}$/;"	l
text10558	figures/pseudo-derivative.svg	/^       id="text10558"><tspan$/;"	i
text145762-2	figures/pseudo-derivative.svg	/^       id="text145762-2"><tspan$/;"	i
text145762-2-4	figures/pseudo-derivative.svg	/^       id="text145762-2-4"><tspan$/;"	i
text145762-2-8	figures/pseudo-derivative.svg	/^       id="text145762-2-8"><tspan$/;"	i
text145762-2-8-0	figures/pseudo-derivative.svg	/^       id="text145762-2-8-0"><tspan$/;"	i
text145762-2-8-8	figures/pseudo-derivative.svg	/^       id="text145762-2-8-8"><tspan$/;"	i
text145762-2-8-8-2	figures/pseudo-derivative.svg	/^       id="text145762-2-8-8-2"><tspan$/;"	i
text145762-2-8-8-9	figures/pseudo-derivative.svg	/^       id="text145762-2-8-8-9"><tspan$/;"	i
text145762-2-8-8-9-9	figures/pseudo-derivative.svg	/^       id="text145762-2-8-8-9-9"><tspan$/;"	i
text145762-3-0	figures/pseudo-derivative.svg	/^       id="text145762-3-0"><tspan$/;"	i
text145762-3-0-0	figures/pseudo-derivative.svg	/^       id="text145762-3-0-0"><tspan$/;"	i
text145762-3-0-4	figures/pseudo-derivative.svg	/^       id="text145762-3-0-4"><tspan$/;"	i
text145762-3-0-4-4	figures/pseudo-derivative.svg	/^       id="text145762-3-0-4-4"><tspan$/;"	i
text145762-3-0-4-4-5	figures/pseudo-derivative.svg	/^       id="text145762-3-0-4-4-5"><tspan$/;"	i
text145762-3-0-4-4-5-3	figures/pseudo-derivative.svg	/^       id="text145762-3-0-4-4-5-3"><tspan$/;"	i
text145762-3-0-4-4-6	figures/pseudo-derivative.svg	/^       id="text145762-3-0-4-4-6"><tspan$/;"	i
text145762-3-0-4-9	figures/pseudo-derivative.svg	/^       id="text145762-3-0-4-9"><tspan$/;"	i
text145762-3-7-5	figures/pseudo-derivative.svg	/^       id="text145762-3-7-5"><tspan$/;"	i
text145762-3-7-5-3	figures/pseudo-derivative.svg	/^       id="text145762-3-7-5-3"><tspan$/;"	i
text145762-3-7-5-6	figures/pseudo-derivative.svg	/^       id="text145762-3-7-5-6"><tspan$/;"	i
text145762-3-7-5-6-8	figures/pseudo-derivative.svg	/^       id="text145762-3-7-5-6-8"><tspan$/;"	i
text145762-3-7-5-6-9	figures/pseudo-derivative.svg	/^       id="text145762-3-7-5-6-9"><tspan$/;"	i
text145762-3-7-5-6-9-2	figures/pseudo-derivative.svg	/^       id="text145762-3-7-5-6-9-2"><tspan$/;"	i
text145762-3-7-5-6-9-2-0	figures/pseudo-derivative.svg	/^       id="text145762-3-7-5-6-9-2-0"><tspan$/;"	i
text145762-3-7-5-6-9-9	figures/pseudo-derivative.svg	/^       id="text145762-3-7-5-6-9-9"><tspan$/;"	i
text145762-5-7	figures/pseudo-derivative.svg	/^       id="text145762-5-7"><tspan$/;"	i
text145762-5-7-1	figures/pseudo-derivative.svg	/^       id="text145762-5-7-1"><tspan$/;"	i
text145762-5-7-8	figures/pseudo-derivative.svg	/^       id="text145762-5-7-8"><tspan$/;"	i
text145762-5-7-8-0	figures/pseudo-derivative.svg	/^       id="text145762-5-7-8-0"><tspan$/;"	i
text145762-5-7-8-0-3	figures/pseudo-derivative.svg	/^       id="text145762-5-7-8-0-3"><tspan$/;"	i
text145762-5-7-8-0-4	figures/pseudo-derivative.svg	/^       id="text145762-5-7-8-0-4"><tspan$/;"	i
text145762-5-7-8-0-4-7	figures/pseudo-derivative.svg	/^       id="text145762-5-7-8-0-4-7"><tspan$/;"	i
text145762-5-7-8-1	figures/pseudo-derivative.svg	/^       id="text145762-5-7-8-1"><tspan$/;"	i
text1459	figures/pseudo-derivative.svg	/^       id="text1459"><tspan$/;"	i
text1459-5	figures/pseudo-derivative.svg	/^       id="text1459-5"><tspan$/;"	i
text1459-6	figures/pseudo-derivative.svg	/^       id="text1459-6"><tspan$/;"	i
text1459-6-8	figures/pseudo-derivative.svg	/^       id="text1459-6-8"><tspan$/;"	i
text1516	figures/pseudo-derivative.svg	/^       id="text1516"><tspan$/;"	i
text1516-5	figures/pseudo-derivative.svg	/^       id="text1516-5"><tspan$/;"	i
text1516-7	figures/pseudo-derivative.svg	/^       id="text1516-7"><tspan$/;"	i
text1516-7-8	figures/pseudo-derivative.svg	/^       id="text1516-7-8"><tspan$/;"	i
text1522	figures/pseudo-derivative.svg	/^       transform="matrix(1.1959062,0,0,1.1959062,41.005211,93.898133)">$/;"	i
text1529	figures/pseudo-derivative.svg	/^       id="text1529"><tspan$/;"	i
text164186	figures/pseudo-derivative.svg	/^       id="text164186"><tspan$/;"	i
text164186-2	figures/pseudo-derivative.svg	/^       id="text164186-2"><tspan$/;"	i
text164186-2-7	figures/pseudo-derivative.svg	/^       id="text164186-2-7"><tspan$/;"	i
text164186-5	figures/pseudo-derivative.svg	/^       id="text164186-5"><tspan$/;"	i
text165558	figures/pseudo-derivative.svg	/^       id="text165558"><tspan$/;"	i
text165558-3	figures/pseudo-derivative.svg	/^       id="text165558-3"><tspan$/;"	i
text1659	figures/pseudo-derivative.svg	/^       id="text1659"><tspan$/;"	i
text1659-0	figures/pseudo-derivative.svg	/^       id="text1659-0"><tspan$/;"	i
text1659-0-1	figures/pseudo-derivative.svg	/^       id="text1659-0-1"><tspan$/;"	i
text1659-0-1-5	figures/pseudo-derivative.svg	/^       id="text1659-0-1-5"><tspan$/;"	i
text1659-0-1-5-3	figures/pseudo-derivative.svg	/^       id="text1659-0-1-5-3"><tspan$/;"	i
text1659-0-1-5-7	figures/pseudo-derivative.svg	/^       id="text1659-0-1-5-7"><tspan$/;"	i
text1659-0-1-5-7-6	figures/pseudo-derivative.svg	/^       id="text1659-0-1-5-7-6"><tspan$/;"	i
text1659-0-1-5-7-6-3	figures/pseudo-derivative.svg	/^       id="text1659-0-1-5-7-6-3"><tspan$/;"	i
text1659-0-1-5-7-6-9	figures/pseudo-derivative.svg	/^       id="text1659-0-1-5-7-6-9"><tspan$/;"	i
text1659-0-1-5-7-6-9-2	figures/pseudo-derivative.svg	/^       id="text1659-0-1-5-7-6-9-2"><tspan$/;"	i
text1659-0-1-5-7-8	figures/pseudo-derivative.svg	/^       id="text1659-0-1-5-7-8"><tspan$/;"	i
text1659-0-1-59	figures/pseudo-derivative.svg	/^       id="text1659-0-1-59"><tspan$/;"	i
text1659-0-1-59-3	figures/pseudo-derivative.svg	/^       id="text1659-0-1-59-3"><tspan$/;"	i
text1659-0-1-59-9	figures/pseudo-derivative.svg	/^       id="text1659-0-1-59-9"><tspan$/;"	i
text1659-0-1-59-9-5	figures/pseudo-derivative.svg	/^       id="text1659-0-1-59-9-5"><tspan$/;"	i
text1659-0-1-59-9-8	figures/pseudo-derivative.svg	/^       id="text1659-0-1-59-9-8"><tspan$/;"	i
text1659-0-1-59-9-8-0	figures/pseudo-derivative.svg	/^       id="text1659-0-1-59-9-8-0"><tspan$/;"	i
text1659-0-1-9	figures/pseudo-derivative.svg	/^       id="text1659-0-1-9"><tspan$/;"	i
text1659-0-2	figures/pseudo-derivative.svg	/^       id="text1659-0-2"><tspan$/;"	i
text1659-0-2-0	figures/pseudo-derivative.svg	/^       id="text1659-0-2-0"><tspan$/;"	i
text1659-0-2-0-5	figures/pseudo-derivative.svg	/^       id="text1659-0-2-0-5"><tspan$/;"	i
text1659-0-2-0-5-1	figures/pseudo-derivative.svg	/^       id="text1659-0-2-0-5-1"><tspan$/;"	i
text1659-0-2-0-57	figures/pseudo-derivative.svg	/^       id="text1659-0-2-0-57"><tspan$/;"	i
text1659-0-2-7	figures/pseudo-derivative.svg	/^       id="text1659-0-2-7"><tspan$/;"	i
text1659-0-6	figures/pseudo-derivative.svg	/^       id="text1659-0-6"><tspan$/;"	i
text1659-04	figures/pseudo-derivative.svg	/^       id="text1659-04"><tspan$/;"	i
text1659-04-3	figures/pseudo-derivative.svg	/^       id="text1659-04-3"><tspan$/;"	i
text1659-04-3-0	figures/pseudo-derivative.svg	/^       id="text1659-04-3-0"><tspan$/;"	i
text1659-04-3-0-5	figures/pseudo-derivative.svg	/^       id="text1659-04-3-0-5"><tspan$/;"	i
text1659-04-3-8	figures/pseudo-derivative.svg	/^       id="text1659-04-3-8"><tspan$/;"	i
text1659-04-4	figures/pseudo-derivative.svg	/^       id="text1659-04-4"><tspan$/;"	i
text1659-7	figures/pseudo-derivative.svg	/^       id="text1659-7"><tspan$/;"	i
text1663	figures/pseudo-derivative.svg	/^       transform="scale(0.5607879,1.7832054)"><tspan$/;"	i
text1663-3	figures/pseudo-derivative.svg	/^       transform="scale(0.56078789,1.7832054)"><tspan$/;"	i
text1663-3-5	figures/pseudo-derivative.svg	/^       transform="scale(0.56078789,1.7832054)"><tspan$/;"	i
text1663-3-5-7	figures/pseudo-derivative.svg	/^       transform="scale(0.56078789,1.7832054)"><tspan$/;"	i
text1663-3-5-9	figures/pseudo-derivative.svg	/^       transform="scale(0.56078789,1.7832054)"><tspan$/;"	i
text1663-3-5-9-1	figures/pseudo-derivative.svg	/^       transform="scale(0.56078789,1.7832054)"><tspan$/;"	i
text1663-3-5-9-1-4	figures/pseudo-derivative.svg	/^       transform="scale(0.56078789,1.7832054)"><tspan$/;"	i
text1663-3-5-9-1-4-0	figures/pseudo-derivative.svg	/^       transform="scale(0.56078789,1.7832054)"><tspan$/;"	i
text1663-3-5-9-1-4-9	figures/pseudo-derivative.svg	/^       transform="scale(0.56078789,1.7832054)"><tspan$/;"	i
text1663-3-5-9-1-4-9-9	figures/pseudo-derivative.svg	/^       transform="scale(0.56078789,1.7832054)"><tspan$/;"	i
text1663-3-5-9-1-41	figures/pseudo-derivative.svg	/^       transform="scale(0.56078789,1.7832054)"><tspan$/;"	i
text1663-3-5-9-7	figures/pseudo-derivative.svg	/^       transform="scale(0.56078789,1.7832054)"><tspan$/;"	i
text1663-3-5-90	figures/pseudo-derivative.svg	/^       transform="scale(0.56078789,1.7832054)"><tspan$/;"	i
text1663-3-5-90-3	figures/pseudo-derivative.svg	/^       transform="scale(0.56078789,1.7832054)"><tspan$/;"	i
text1663-3-5-90-3-0	figures/pseudo-derivative.svg	/^       transform="scale(0.56078789,1.7832054)"><tspan$/;"	i
text1663-3-5-90-3-8	figures/pseudo-derivative.svg	/^       transform="scale(0.56078789,1.7832054)"><tspan$/;"	i
text1663-3-5-90-3-8-5	figures/pseudo-derivative.svg	/^       transform="scale(0.56078789,1.7832054)"><tspan$/;"	i
text1663-3-5-90-37	figures/pseudo-derivative.svg	/^       transform="scale(0.56078789,1.7832054)"><tspan$/;"	i
text1663-3-6	figures/pseudo-derivative.svg	/^       transform="scale(0.56078789,1.7832054)"><tspan$/;"	i
text1663-3-6-9	figures/pseudo-derivative.svg	/^       transform="scale(0.56078789,1.7832054)"><tspan$/;"	i
text1663-3-6-9-2	figures/pseudo-derivative.svg	/^       transform="scale(0.56078789,1.7832054)"><tspan$/;"	i
text1663-3-6-9-2-1	figures/pseudo-derivative.svg	/^       transform="scale(0.56078789,1.7832054)"><tspan$/;"	i
text1663-3-6-9-3	figures/pseudo-derivative.svg	/^       transform="scale(0.56078789,1.7832054)"><tspan$/;"	i
text1663-3-6-97	figures/pseudo-derivative.svg	/^       transform="scale(0.56078789,1.7832054)"><tspan$/;"	i
text1663-3-66	figures/pseudo-derivative.svg	/^       transform="scale(0.56078789,1.7832054)"><tspan$/;"	i
text1663-6	figures/pseudo-derivative.svg	/^       transform="scale(-0.5607879,1.7832054)"><tspan$/;"	i
text1663-6-0	figures/pseudo-derivative.svg	/^       transform="scale(-0.56078789,1.7832054)"><tspan$/;"	i
text1663-6-0-0	figures/pseudo-derivative.svg	/^       transform="scale(-0.56078789,1.7832054)"><tspan$/;"	i
text1663-6-0-0-5	figures/pseudo-derivative.svg	/^       transform="scale(-0.56078789,1.7832054)"><tspan$/;"	i
text1663-6-0-0-9	figures/pseudo-derivative.svg	/^       transform="scale(-0.56078789,1.7832054)"><tspan$/;"	i
text1663-6-0-0-9-0	figures/pseudo-derivative.svg	/^       transform="scale(-0.56078789,1.7832054)"><tspan$/;"	i
text1663-6-0-0-9-0-0	figures/pseudo-derivative.svg	/^       transform="scale(-0.56078789,1.7832054)"><tspan$/;"	i
text1663-6-0-0-9-3	figures/pseudo-derivative.svg	/^       transform="scale(-0.56078789,1.7832054)"><tspan$/;"	i
text1663-6-0-2	figures/pseudo-derivative.svg	/^       transform="scale(-0.56078789,1.7832054)"><tspan$/;"	i
text1663-6-0-7	figures/pseudo-derivative.svg	/^       transform="scale(-0.56078789,1.7832054)"><tspan$/;"	i
text1663-6-0-7-1	figures/pseudo-derivative.svg	/^       transform="scale(-0.56078789,1.7832054)"><tspan$/;"	i
text1663-6-0-7-1-0	figures/pseudo-derivative.svg	/^       transform="scale(-0.56078789,1.7832054)"><tspan$/;"	i
text1663-6-0-7-1-0-4	figures/pseudo-derivative.svg	/^       transform="scale(-0.56078789,1.7832054)"><tspan$/;"	i
text1663-6-0-7-1-0-4-6	figures/pseudo-derivative.svg	/^       transform="scale(-0.56078789,1.7832054)"><tspan$/;"	i
text1663-6-0-7-1-0-7	figures/pseudo-derivative.svg	/^       transform="scale(-0.56078789,1.7832054)"><tspan$/;"	i
text1663-6-0-7-1-3	figures/pseudo-derivative.svg	/^       transform="scale(-0.56078789,1.7832054)"><tspan$/;"	i
text1663-6-0-7-10	figures/pseudo-derivative.svg	/^       transform="scale(-0.56078789,1.7832054)"><tspan$/;"	i
text1663-6-0-7-7	figures/pseudo-derivative.svg	/^       transform="scale(-0.56078789,1.7832054)"><tspan$/;"	i
text1663-6-0-7-7-6	figures/pseudo-derivative.svg	/^       transform="scale(-0.56078789,1.7832054)"><tspan$/;"	i
text1663-6-0-7-7-9	figures/pseudo-derivative.svg	/^       transform="scale(-0.56078789,1.7832054)"><tspan$/;"	i
text1663-6-0-7-7-9-0	figures/pseudo-derivative.svg	/^       transform="scale(-0.56078789,1.7832054)"><tspan$/;"	i
text1663-6-0-7-7-9-0-0	figures/pseudo-derivative.svg	/^       transform="scale(-0.56078789,1.7832054)"><tspan$/;"	i
text1663-6-0-7-7-9-0-2	figures/pseudo-derivative.svg	/^       transform="scale(-0.56078789,1.7832054)"><tspan$/;"	i
text1663-6-0-7-7-9-0-2-4	figures/pseudo-derivative.svg	/^       transform="scale(-0.56078789,1.7832054)"><tspan$/;"	i
text1663-6-0-7-7-9-09	figures/pseudo-derivative.svg	/^       transform="scale(-0.56078789,1.7832054)"><tspan$/;"	i
text1663-6-2	figures/pseudo-derivative.svg	/^       transform="scale(-0.56078789,1.7832054)"><tspan$/;"	i
text1663-6-2-0	figures/pseudo-derivative.svg	/^       transform="scale(-0.56078789,1.7832054)"><tspan$/;"	i
text1663-6-2-3	figures/pseudo-derivative.svg	/^       transform="scale(-0.56078789,1.7832054)"><tspan$/;"	i
text1663-6-2-3-2	figures/pseudo-derivative.svg	/^       transform="scale(-0.56078789,1.7832054)"><tspan$/;"	i
text1663-6-2-3-2-1	figures/pseudo-derivative.svg	/^       transform="scale(-0.56078789,1.7832054)"><tspan$/;"	i
text1663-6-2-3-7	figures/pseudo-derivative.svg	/^       transform="scale(-0.56078789,1.7832054)"><tspan$/;"	i
text1663-6-8	figures/pseudo-derivative.svg	/^       transform="scale(-0.56078789,1.7832054)"><tspan$/;"	i
text1663-7	figures/pseudo-derivative.svg	/^       transform="scale(0.56078789,1.7832054)"><tspan$/;"	i
text1663-7-1	figures/pseudo-derivative.svg	/^       transform="scale(0.56078789,1.7832054)"><tspan$/;"	i
text1663-7-1-0	figures/pseudo-derivative.svg	/^       transform="scale(0.56078789,1.7832054)"><tspan$/;"	i
text1663-7-1-2	figures/pseudo-derivative.svg	/^       transform="scale(0.56078789,1.7832054)"><tspan$/;"	i
text1663-7-1-2-7	figures/pseudo-derivative.svg	/^       transform="scale(0.56078789,1.7832054)"><tspan$/;"	i
text1663-7-7	figures/pseudo-derivative.svg	/^       transform="scale(0.56078789,1.7832054)"><tspan$/;"	i
text1663-8	figures/pseudo-derivative.svg	/^       transform="scale(0.56078789,1.7832054)"><tspan$/;"	i
text191995	figures/pseudo-derivative.svg	/^       transform="rotate(-90)"><tspan$/;"	i
text191995-2	figures/pseudo-derivative.svg	/^       transform="rotate(-90)"><tspan$/;"	i
text25941	figures/pseudo-derivative.svg	/^       id="text25941"><tspan$/;"	i
text25941-8	figures/pseudo-derivative.svg	/^       id="text25941-8"><tspan$/;"	i
text_10_00000025402117890948562680000005723937169633012632_	figures/combined-sparsity-plots.svg	/^			<g id="text_10_00000025402117890948562680000005723937169633012632_">$/;"	i
text_10_00000180330667493432485500000005503855278462567614_	figures/combined-sparsity-plots.svg	/^			<g id="text_10_00000180330667493432485500000005503855278462567614_">$/;"	i
text_11_00000080197790398159468820000017035393406401484987_	figures/combined-sparsity-plots.svg	/^			<g id="text_11_00000080197790398159468820000017035393406401484987_">$/;"	i
text_11_00000165923986562226979020000010325471850067988896_	figures/combined-sparsity-plots.svg	/^			<g id="text_11_00000165923986562226979020000010325471850067988896_">$/;"	i
text_12_00000158715632489751165800000016066571304419404934_	figures/combined-sparsity-plots.svg	/^			<g id="text_12_00000158715632489751165800000016066571304419404934_">$/;"	i
text_12_00000162320029448203993040000001997987319563512706_	figures/combined-sparsity-plots.svg	/^			<g id="text_12_00000162320029448203993040000001997987319563512706_">$/;"	i
text_13_00000037675726172968515550000003773553248303942826_	figures/combined-sparsity-plots.svg	/^		<g id="text_13_00000037675726172968515550000003773553248303942826_">$/;"	i
text_13_00000132785077193799557870000004767648747120669115_	figures/combined-sparsity-plots.svg	/^			<g id="text_13_00000132785077193799557870000004767648747120669115_">$/;"	i
text_14_00000001629335892175702310000005526006266770534030_	figures/combined-sparsity-plots.svg	/^		<g id="text_14_00000001629335892175702310000005526006266770534030_">$/;"	i
text_14_00000067204567052406663270000002212402676969702050_	figures/combined-sparsity-plots.svg	/^			<g id="text_14_00000067204567052406663270000002212402676969702050_">$/;"	i
text_15	figures/combined-sparsity-plots.svg	/^			<g id="text_15">$/;"	i
text_15_00000032629081542659933900000013956714345102382012_	figures/combined-sparsity-plots.svg	/^			<g id="text_15_00000032629081542659933900000013956714345102382012_">$/;"	i
text_16	figures/combined-sparsity-plots.svg	/^			<g id="text_16">$/;"	i
text_16_00000181066601506672730600000000598311736325626025_	figures/combined-sparsity-plots.svg	/^			<g id="text_16_00000181066601506672730600000000598311736325626025_">$/;"	i
text_17	figures/combined-sparsity-plots.svg	/^			<g id="text_17">$/;"	i
text_17_00000168088240593715386140000015853086148467946115_	figures/combined-sparsity-plots.svg	/^			<g id="text_17_00000168088240593715386140000015853086148467946115_">$/;"	i
text_18	figures/combined-sparsity-plots.svg	/^			<g id="text_18">$/;"	i
text_18_00000110448788903474022620000016978831529279226275_	figures/combined-sparsity-plots.svg	/^		<g id="text_18_00000110448788903474022620000016978831529279226275_">$/;"	i
text_19	figures/combined-sparsity-plots.svg	/^			<g id="text_19">$/;"	i
text_19_00000169535087335356266610000013822879693198544294_	figures/combined-sparsity-plots.svg	/^		<g id="text_19_00000169535087335356266610000013822879693198544294_">$/;"	i
text_19_00000183947446145216529410000016098858282362771086_	figures/combined-sparsity-plots.svg	/^			<g id="text_19_00000183947446145216529410000016098858282362771086_">$/;"	i
text_1_00000092414747648365814740000016506081165565497505_	figures/combined-sparsity-plots.svg	/^			<g id="text_1_00000092414747648365814740000016506081165565497505_">$/;"	i
text_1_00000119119403136701310370000001993366918420618148_	figures/combined-sparsity-plots.svg	/^			<g id="text_1_00000119119403136701310370000001993366918420618148_">$/;"	i
text_20	figures/combined-sparsity-plots.svg	/^			<g id="text_20">$/;"	i
text_20_00000152972524620636547500000004335014914891595187_	figures/combined-sparsity-plots.svg	/^		<g id="text_20_00000152972524620636547500000004335014914891595187_">$/;"	i
text_20_00000154416079392604530910000005231702381403834001_	figures/combined-sparsity-plots.svg	/^			<g id="text_20_00000154416079392604530910000005231702381403834001_">$/;"	i
text_21	figures/combined-sparsity-plots.svg	/^			<g id="text_21">$/;"	i
text_21_00000024689792024197521140000010306816963301315497_	figures/combined-sparsity-plots.svg	/^		<g id="text_21_00000024689792024197521140000010306816963301315497_">$/;"	i
text_21_00000103223846221067951700000014015179323786576295_	figures/combined-sparsity-plots.svg	/^			<g id="text_21_00000103223846221067951700000014015179323786576295_">$/;"	i
text_22	figures/combined-sparsity-plots.svg	/^		<g id="text_22">$/;"	i
text_22_00000134212571260532666880000009150390799729241217_	figures/combined-sparsity-plots.svg	/^			<g id="text_22_00000134212571260532666880000009150390799729241217_">$/;"	i
text_22_00000155140715784544818590000018226491267688960926_	figures/combined-sparsity-plots.svg	/^		<g id="text_22_00000155140715784544818590000018226491267688960926_">$/;"	i
text_23	figures/combined-sparsity-plots.svg	/^			<g id="text_23">$/;"	i
text_23_00000044138503665666246220000004364669438944298628_	figures/combined-sparsity-plots.svg	/^		<g id="text_23_00000044138503665666246220000004364669438944298628_">$/;"	i
text_23_00000177479659490516836140000007118109041399548861_	figures/combined-sparsity-plots.svg	/^			<g id="text_23_00000177479659490516836140000007118109041399548861_">$/;"	i
text_24	figures/combined-sparsity-plots.svg	/^			<g id="text_24">$/;"	i
text_24_00000027604567429209531490000011934432267621795225_	figures/combined-sparsity-plots.svg	/^			<g id="text_24_00000027604567429209531490000011934432267621795225_">$/;"	i
text_24_00000073720554199412671450000013869710962683295664_	figures/combined-sparsity-plots.svg	/^		<g id="text_24_00000073720554199412671450000013869710962683295664_">$/;"	i
text_25	figures/combined-sparsity-plots.svg	/^			<g id="text_25">$/;"	i
text_25_00000045613653218304610210000017387475358415618433_	figures/combined-sparsity-plots.svg	/^		<g id="text_25_00000045613653218304610210000017387475358415618433_">$/;"	i
text_25_00000132085751319827194110000002130517002005188759_	figures/combined-sparsity-plots.svg	/^			<g id="text_25_00000132085751319827194110000002130517002005188759_">$/;"	i
text_26	figures/combined-sparsity-plots.svg	/^			<g id="text_26">$/;"	i
text_26_00000070821319036162804240000003914152815214829757_	figures/combined-sparsity-plots.svg	/^		<g id="text_26_00000070821319036162804240000003914152815214829757_">$/;"	i
text_26_00000180326899863942948390000007401075450340245942_	figures/combined-sparsity-plots.svg	/^			<g id="text_26_00000180326899863942948390000007401075450340245942_">$/;"	i
text_27	figures/combined-sparsity-plots.svg	/^		<g id="text_27">$/;"	i
text_27_00000070080126532949194710000001867763334055949478_	figures/combined-sparsity-plots.svg	/^		<g id="text_27_00000070080126532949194710000001867763334055949478_">$/;"	i
text_27_00000128447578931503780070000010529672081964054711_	figures/combined-sparsity-plots.svg	/^	<g id="text_27_00000128447578931503780070000010529672081964054711_">$/;"	i
text_28_00000007410538782728982100000007785440459939103134_	figures/combined-sparsity-plots.svg	/^			<g id="text_28_00000007410538782728982100000007785440459939103134_">$/;"	i
text_29_00000156572759810012081750000007464286959655511177_	figures/combined-sparsity-plots.svg	/^			<g id="text_29_00000156572759810012081750000007464286959655511177_">$/;"	i
text_2_00000002382458366851567030000000301929933619281300_	figures/combined-sparsity-plots.svg	/^			<g id="text_2_00000002382458366851567030000000301929933619281300_">$/;"	i
text_2_00000113334200143191587410000005498731272354828730_	figures/combined-sparsity-plots.svg	/^			<g id="text_2_00000113334200143191587410000005498731272354828730_">$/;"	i
text_30_00000031929153437433001080000000384819521312291481_	figures/combined-sparsity-plots.svg	/^			<g id="text_30_00000031929153437433001080000000384819521312291481_">$/;"	i
text_31_00000070808094651178458110000003953857543840927362_	figures/combined-sparsity-plots.svg	/^			<g id="text_31_00000070808094651178458110000003953857543840927362_">$/;"	i
text_32_00000157285848208332482990000004365530690259378871_	figures/combined-sparsity-plots.svg	/^			<g id="text_32_00000157285848208332482990000004365530690259378871_">$/;"	i
text_33_00000067216603810993455650000002358665358994987439_	figures/combined-sparsity-plots.svg	/^			<g id="text_33_00000067216603810993455650000002358665358994987439_">$/;"	i
text_34_00000027603565215904919900000002961089822761051798_	figures/combined-sparsity-plots.svg	/^		<g id="text_34_00000027603565215904919900000002961089822761051798_">$/;"	i
text_35_00000155843462136076761550000010686802651558860974_	figures/combined-sparsity-plots.svg	/^			<g id="text_35_00000155843462136076761550000010686802651558860974_">$/;"	i
text_36_00000160167378759725314590000011007792414989805211_	figures/combined-sparsity-plots.svg	/^			<g id="text_36_00000160167378759725314590000011007792414989805211_">$/;"	i
text_37_00000066485008482809313640000018095271403786674336_	figures/combined-sparsity-plots.svg	/^			<g id="text_37_00000066485008482809313640000018095271403786674336_">$/;"	i
text_38_00000170255148722584969650000006516463150896614317_	figures/combined-sparsity-plots.svg	/^			<g id="text_38_00000170255148722584969650000006516463150896614317_">$/;"	i
text_39_00000145027009092328815200000018201490978496679813_	figures/combined-sparsity-plots.svg	/^			<g id="text_39_00000145027009092328815200000018201490978496679813_">$/;"	i
text_3_00000018223942945820580450000005613645354920143790_	figures/combined-sparsity-plots.svg	/^			<g id="text_3_00000018223942945820580450000005613645354920143790_">$/;"	i
text_3_00000115488024852450825830000010805682515787848839_	figures/combined-sparsity-plots.svg	/^			<g id="text_3_00000115488024852450825830000010805682515787848839_">$/;"	i
text_40_00000057108161885342076150000007132293284347846331_	figures/combined-sparsity-plots.svg	/^			<g id="text_40_00000057108161885342076150000007132293284347846331_">$/;"	i
text_41_00000053542255114590846550000009654816261654820269_	figures/combined-sparsity-plots.svg	/^			<g id="text_41_00000053542255114590846550000009654816261654820269_">$/;"	i
text_42_00000063610867326660569640000008776659414389156769_	figures/combined-sparsity-plots.svg	/^			<g id="text_42_00000063610867326660569640000008776659414389156769_">$/;"	i
text_43_00000049204980007984972390000012337313940556078748_	figures/combined-sparsity-plots.svg	/^		<g id="text_43_00000049204980007984972390000012337313940556078748_">$/;"	i
text_44_00000113327662911109987750000008024892099359319680_	figures/combined-sparsity-plots.svg	/^			<g id="text_44_00000113327662911109987750000008024892099359319680_">$/;"	i
text_45_00000115472426987091456340000011381355942919281823_	figures/combined-sparsity-plots.svg	/^			<g id="text_45_00000115472426987091456340000011381355942919281823_">$/;"	i
text_46_00000020377819863751022480000004586821131730651791_	figures/combined-sparsity-plots.svg	/^			<g id="text_46_00000020377819863751022480000004586821131730651791_">$/;"	i
text_47_00000044864715959257228670000009242017271997812385_	figures/combined-sparsity-plots.svg	/^			<g id="text_47_00000044864715959257228670000009242017271997812385_">$/;"	i
text_48_00000171709672083968962690000015735304379918266300_	figures/combined-sparsity-plots.svg	/^			<g id="text_48_00000171709672083968962690000015735304379918266300_">$/;"	i
text_49_00000146486168825228627850000016512957243996582819_	figures/combined-sparsity-plots.svg	/^			<g id="text_49_00000146486168825228627850000016512957243996582819_">$/;"	i
text_4_00000065780387806992849970000008079730070071101584_	figures/combined-sparsity-plots.svg	/^			<g id="text_4_00000065780387806992849970000008079730070071101584_">$/;"	i
text_4_00000121975277180662488900000012524063917012571022_	figures/combined-sparsity-plots.svg	/^			<g id="text_4_00000121975277180662488900000012524063917012571022_">$/;"	i
text_50_00000047772415184666112070000010232800488308049310_	figures/combined-sparsity-plots.svg	/^		<g id="text_50_00000047772415184666112070000010232800488308049310_">$/;"	i
text_53	figures/combined-sparsity-plots.svg	/^		<g id="text_53">$/;"	i
text_54	figures/combined-sparsity-plots.svg	/^		<g id="text_54">$/;"	i
text_55	figures/combined-sparsity-plots.svg	/^		<g id="text_55">$/;"	i
text_56	figures/combined-sparsity-plots.svg	/^		<g id="text_56">$/;"	i
text_57	figures/combined-sparsity-plots.svg	/^		<g id="text_57">$/;"	i
text_58	figures/combined-sparsity-plots.svg	/^		<g id="text_58">$/;"	i
text_59	figures/combined-sparsity-plots.svg	/^		<g id="text_59">$/;"	i
text_5_00000044173807405333991080000007180978024077757870_	figures/combined-sparsity-plots.svg	/^		<g id="text_5_00000044173807405333991080000007180978024077757870_">$/;"	i
text_5_00000139268407338375356650000004471050463646537112_	figures/combined-sparsity-plots.svg	/^			<g id="text_5_00000139268407338375356650000004471050463646537112_">$/;"	i
text_60	figures/combined-sparsity-plots.svg	/^		<g id="text_60">$/;"	i
text_61	figures/combined-sparsity-plots.svg	/^		<g id="text_61">$/;"	i
text_62	figures/combined-sparsity-plots.svg	/^		<g id="text_62">$/;"	i
text_6_00000000206163287254062910000000900956833705026479_	figures/combined-sparsity-plots.svg	/^			<g id="text_6_00000000206163287254062910000000900956833705026479_">$/;"	i
text_6_00000084523399376215113440000004094775638278198146_	figures/combined-sparsity-plots.svg	/^			<g id="text_6_00000084523399376215113440000004094775638278198146_">$/;"	i
text_7_00000031929941623377118760000005371074811816118698_	figures/combined-sparsity-plots.svg	/^			<g id="text_7_00000031929941623377118760000005371074811816118698_">$/;"	i
text_7_00000164505442676616378940000017819940082488382398_	figures/combined-sparsity-plots.svg	/^			<g id="text_7_00000164505442676616378940000017819940082488382398_">$/;"	i
text_8_00000057848414566772355600000014037198949325874091_	figures/combined-sparsity-plots.svg	/^			<g id="text_8_00000057848414566772355600000014037198949325874091_">$/;"	i
text_8_00000065763884583428273710000011779441288747410339_	figures/combined-sparsity-plots.svg	/^			<g id="text_8_00000065763884583428273710000011779441288747410339_">$/;"	i
text_9_00000120559035599947794560000011152670116694110101_	figures/combined-sparsity-plots.svg	/^		<g id="text_9_00000120559035599947794560000011152670116694110101_">$/;"	i
text_9_00000137132818588276083490000006101139055382328497_	figures/combined-sparsity-plots.svg	/^			<g id="text_9_00000137132818588276083490000006101139055382328497_">$/;"	i
theorem	main.tex	/^\\newtheorem{theorem}{Theorem}$/;"	t
tspan10556	figures/pseudo-derivative.svg	/^         y="72.778641">event<\/tspan><tspan$/;"	i
tspan10560	figures/pseudo-derivative.svg	/^         id="tspan10560">generation<\/tspan><\/text>$/;"	i
tspan10700	figures/pseudo-derivative.svg	/^   id="tspan10700">H<\/tspan><\/tspan><tspan$/;"	i
tspan10700-2	figures/pseudo-derivative.svg	/^   id="tspan10700-2">H<\/tspan><\/tspan><tspan$/;"	i
tspan1457	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">+ε<\/tspan><\/text>$/;"	i
tspan1457-2	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">-ε<\/tspan><\/text>$/;"	i
tspan1457-2-3	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">-ε<\/tspan><\/text>$/;"	i
tspan1457-4	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">+ε<\/tspan><\/text>$/;"	i
tspan145760-0-8	figures/pseudo-derivative.svg	/^         style="font-size:2.11667px;stroke-width:0.264583"><tspan$/;"	i
tspan145760-0-8-2	figures/pseudo-derivative.svg	/^         style="font-size:2.11667px;stroke-width:0.264583"><tspan$/;"	i
tspan145760-0-8-9	figures/pseudo-derivative.svg	/^         style="font-size:2.11667px;stroke-width:0.264583"><tspan$/;"	i
tspan145760-0-8-9-0	figures/pseudo-derivative.svg	/^         style="font-size:2.11667px;stroke-width:0.264583"><tspan$/;"	i
tspan145760-0-8-9-6	figures/pseudo-derivative.svg	/^         style="font-size:2.11667px;stroke-width:0.264583"><tspan$/;"	i
tspan145760-0-8-9-6-4	figures/pseudo-derivative.svg	/^         style="font-size:2.11667px;stroke-width:0.264583"><tspan$/;"	i
tspan145760-0-8-9-6-8	figures/pseudo-derivative.svg	/^         style="font-size:2.11667px;stroke-width:0.264583"><tspan$/;"	i
tspan145760-0-8-9-6-8-1	figures/pseudo-derivative.svg	/^         style="font-size:2.11667px;stroke-width:0.264583"><tspan$/;"	i
tspan145760-1-3-0	figures/pseudo-derivative.svg	/^         style="font-size:2.11667px;stroke-width:0.264583"><tspan$/;"	i
tspan145760-1-3-0-1	figures/pseudo-derivative.svg	/^         style="font-size:2.11667px;stroke-width:0.264583"><tspan$/;"	i
tspan145760-1-3-0-4	figures/pseudo-derivative.svg	/^         style="font-size:2.11667px;stroke-width:0.264583"><tspan$/;"	i
tspan145760-1-3-0-4-0	figures/pseudo-derivative.svg	/^         style="font-size:2.11667px;stroke-width:0.264583"><tspan$/;"	i
tspan145760-1-3-0-4-0-7	figures/pseudo-derivative.svg	/^         style="font-size:2.11667px;stroke-width:0.264583"><tspan$/;"	i
tspan145760-1-3-0-4-0-9	figures/pseudo-derivative.svg	/^         style="font-size:2.11667px;stroke-width:0.264583"><tspan$/;"	i
tspan145760-1-3-0-4-0-9-2	figures/pseudo-derivative.svg	/^         style="font-size:2.11667px;stroke-width:0.264583"><tspan$/;"	i
tspan145760-1-3-0-4-8	figures/pseudo-derivative.svg	/^         style="font-size:2.11667px;stroke-width:0.264583"><tspan$/;"	i
tspan145760-1-6	figures/pseudo-derivative.svg	/^         style="font-size:2.11667px;stroke-width:0.264583"><tspan$/;"	i
tspan145760-1-6-1	figures/pseudo-derivative.svg	/^         style="font-size:2.11667px;stroke-width:0.264583"><tspan$/;"	i
tspan145760-1-6-92	figures/pseudo-derivative.svg	/^         style="font-size:2.11667px;stroke-width:0.264583"><tspan$/;"	i
tspan145760-1-6-92-7	figures/pseudo-derivative.svg	/^         style="font-size:2.11667px;stroke-width:0.264583"><tspan$/;"	i
tspan145760-1-6-92-7-3	figures/pseudo-derivative.svg	/^         style="font-size:2.11667px;stroke-width:0.264583"><tspan$/;"	i
tspan145760-1-6-92-7-8	figures/pseudo-derivative.svg	/^         style="font-size:2.11667px;stroke-width:0.264583"><tspan$/;"	i
tspan145760-1-6-92-7-8-2	figures/pseudo-derivative.svg	/^         style="font-size:2.11667px;stroke-width:0.264583"><tspan$/;"	i
tspan145760-1-6-92-9	figures/pseudo-derivative.svg	/^         style="font-size:2.11667px;stroke-width:0.264583"><tspan$/;"	i
tspan145760-2	figures/pseudo-derivative.svg	/^         style="font-size:2.11667px;stroke-width:0.264583"><tspan$/;"	i
tspan145760-2-4	figures/pseudo-derivative.svg	/^         style="font-size:2.11667px;stroke-width:0.264583"><tspan$/;"	i
tspan145760-2-4-2	figures/pseudo-derivative.svg	/^         style="font-size:2.11667px;stroke-width:0.264583"><tspan$/;"	i
tspan145760-2-4-6	figures/pseudo-derivative.svg	/^         style="font-size:2.11667px;stroke-width:0.264583"><tspan$/;"	i
tspan145760-2-4-6-1	figures/pseudo-derivative.svg	/^         style="font-size:2.11667px;stroke-width:0.264583"><tspan$/;"	i
tspan145760-2-4-6-1-7	figures/pseudo-derivative.svg	/^         style="font-size:2.11667px;stroke-width:0.264583"><tspan$/;"	i
tspan145760-2-4-6-7	figures/pseudo-derivative.svg	/^         style="font-size:2.11667px;stroke-width:0.264583"><tspan$/;"	i
tspan145760-2-9	figures/pseudo-derivative.svg	/^         style="font-size:2.11667px;stroke-width:0.264583"><tspan$/;"	i
tspan146581-0-0	figures/pseudo-derivative.svg	/^   id="tspan146581-0-0">y<\/tspan><tspan$/;"	i
tspan146581-0-0-0	figures/pseudo-derivative.svg	/^   id="tspan146581-0-0-0">y<\/tspan><tspan$/;"	i
tspan146581-0-0-2	figures/pseudo-derivative.svg	/^   id="tspan146581-0-0-2">y<\/tspan><tspan$/;"	i
tspan146581-0-0-2-2	figures/pseudo-derivative.svg	/^   id="tspan146581-0-0-2-2">y<\/tspan><tspan$/;"	i
tspan146581-0-0-2-2-0	figures/pseudo-derivative.svg	/^   id="tspan146581-0-0-2-2-0">y<\/tspan><tspan$/;"	i
tspan146581-0-0-2-2-0-2	figures/pseudo-derivative.svg	/^   id="tspan146581-0-0-2-2-0-2">y<\/tspan><tspan$/;"	i
tspan146581-0-0-2-2-4	figures/pseudo-derivative.svg	/^   id="tspan146581-0-0-2-2-4">y<\/tspan><tspan$/;"	i
tspan146581-0-0-2-3	figures/pseudo-derivative.svg	/^   id="tspan146581-0-0-2-3">y<\/tspan><tspan$/;"	i
tspan146581-3	figures/pseudo-derivative.svg	/^   id="tspan146581-3">y<\/tspan><tspan$/;"	i
tspan146581-3-0	figures/pseudo-derivative.svg	/^   id="tspan146581-3-0">y<\/tspan><tspan$/;"	i
tspan146581-3-3	figures/pseudo-derivative.svg	/^   id="tspan146581-3-3">y<\/tspan><tspan$/;"	i
tspan146581-3-3-2	figures/pseudo-derivative.svg	/^   id="tspan146581-3-3-2">y<\/tspan><tspan$/;"	i
tspan146581-3-3-2-0	figures/pseudo-derivative.svg	/^   id="tspan146581-3-3-2-0">y<\/tspan><tspan$/;"	i
tspan146581-3-3-2-0-9	figures/pseudo-derivative.svg	/^   id="tspan146581-3-3-2-0-9">y<\/tspan><tspan$/;"	i
tspan146581-3-3-2-03	figures/pseudo-derivative.svg	/^   id="tspan146581-3-3-2-03">y<\/tspan><tspan$/;"	i
tspan146581-3-3-9	figures/pseudo-derivative.svg	/^   id="tspan146581-3-3-9">y<\/tspan><tspan$/;"	i
tspan146589-2-0	figures/pseudo-derivative.svg	/^   id="tspan146589-2-0">c<\/tspan><tspan$/;"	i
tspan146589-2-0-1	figures/pseudo-derivative.svg	/^   id="tspan146589-2-0-1">c<\/tspan><tspan$/;"	i
tspan146589-2-0-9	figures/pseudo-derivative.svg	/^   id="tspan146589-2-0-9">c<\/tspan><tspan$/;"	i
tspan146589-2-0-9-6	figures/pseudo-derivative.svg	/^   id="tspan146589-2-0-9-6">c<\/tspan><tspan$/;"	i
tspan146589-2-0-9-8	figures/pseudo-derivative.svg	/^   id="tspan146589-2-0-9-8">c<\/tspan><tspan$/;"	i
tspan146589-2-0-9-8-2	figures/pseudo-derivative.svg	/^   id="tspan146589-2-0-9-8-2">c<\/tspan><tspan$/;"	i
tspan146589-2-0-9-8-6	figures/pseudo-derivative.svg	/^   id="tspan146589-2-0-9-8-6">c<\/tspan><tspan$/;"	i
tspan146589-2-0-9-8-6-1	figures/pseudo-derivative.svg	/^   id="tspan146589-2-0-9-8-6-1">c<\/tspan><tspan$/;"	i
tspan146589-9	figures/pseudo-derivative.svg	/^   id="tspan146589-9">c<\/tspan><tspan$/;"	i
tspan146589-9-0	figures/pseudo-derivative.svg	/^   id="tspan146589-9-0">c<\/tspan><tspan$/;"	i
tspan146589-9-0-2	figures/pseudo-derivative.svg	/^   id="tspan146589-9-0-2">c<\/tspan><tspan$/;"	i
tspan146589-9-0-2-6	figures/pseudo-derivative.svg	/^   id="tspan146589-9-0-2-6">c<\/tspan><tspan$/;"	i
tspan146589-9-0-2-7	figures/pseudo-derivative.svg	/^   id="tspan146589-9-0-2-7">c<\/tspan><tspan$/;"	i
tspan146589-9-0-2-7-4	figures/pseudo-derivative.svg	/^   id="tspan146589-9-0-2-7-4">c<\/tspan><tspan$/;"	i
tspan146589-9-0-4	figures/pseudo-derivative.svg	/^   id="tspan146589-9-0-4">c<\/tspan><tspan$/;"	i
tspan146589-9-9	figures/pseudo-derivative.svg	/^   id="tspan146589-9-9">c<\/tspan><tspan$/;"	i
tspan146591-1-5	figures/pseudo-derivative.svg	/^   id="tspan146591-1-5">j<\/tspan>   <\/tspan><\/text>$/;"	i
tspan146591-1-5-5	figures/pseudo-derivative.svg	/^   id="tspan146591-1-5-5">j<\/tspan>   <\/tspan><\/text>$/;"	i
tspan146591-1-5-5-0	figures/pseudo-derivative.svg	/^   id="tspan146591-1-5-5-0">j<\/tspan>   <\/tspan><\/text>$/;"	i
tspan146591-1-5-5-1	figures/pseudo-derivative.svg	/^   id="tspan146591-1-5-5-1">j<\/tspan>   <\/tspan><\/text>$/;"	i
tspan146591-1-5-5-1-1	figures/pseudo-derivative.svg	/^   id="tspan146591-1-5-5-1-1">j<\/tspan>   <\/tspan><\/text>$/;"	i
tspan146591-1-5-5-1-1-7	figures/pseudo-derivative.svg	/^   id="tspan146591-1-5-5-1-1-7">j<\/tspan>   <\/tspan><\/text>$/;"	i
tspan146591-1-5-5-1-5	figures/pseudo-derivative.svg	/^   id="tspan146591-1-5-5-1-5">j<\/tspan>   <\/tspan><\/text>$/;"	i
tspan146591-1-5-9	figures/pseudo-derivative.svg	/^   id="tspan146591-1-5-9">j<\/tspan>   <\/tspan><\/text>$/;"	i
tspan146591-6	figures/pseudo-derivative.svg	/^   id="tspan146591-6">i<\/tspan>   <\/tspan><\/text>$/;"	i
tspan146591-6-6	figures/pseudo-derivative.svg	/^   id="tspan146591-6-6">i<\/tspan>   <\/tspan><\/text>$/;"	i
tspan146591-6-6-4	figures/pseudo-derivative.svg	/^   id="tspan146591-6-6-4">i<\/tspan>   <\/tspan><\/text>$/;"	i
tspan146591-6-6-4-0	figures/pseudo-derivative.svg	/^   id="tspan146591-6-6-4-0">i<\/tspan>   <\/tspan><\/text>$/;"	i
tspan146591-6-6-4-0-3	figures/pseudo-derivative.svg	/^   id="tspan146591-6-6-4-0-3">i<\/tspan>   <\/tspan><\/text>$/;"	i
tspan146591-6-6-4-3	figures/pseudo-derivative.svg	/^   id="tspan146591-6-6-4-3">i<\/tspan>   <\/tspan><\/text>$/;"	i
tspan146591-6-6-5	figures/pseudo-derivative.svg	/^   id="tspan146591-6-6-5">i<\/tspan>   <\/tspan><\/text>$/;"	i
tspan146591-6-62	figures/pseudo-derivative.svg	/^   id="tspan146591-6-62">i<\/tspan>   <\/tspan><\/text>$/;"	i
tspan146599-2	figures/pseudo-derivative.svg	/^   style="font-style:normal;font-variant:normal;font-weight:normal;font-stretch:normal;font-size/;"	i
tspan146599-2-1	figures/pseudo-derivative.svg	/^   style="font-style:normal;font-variant:normal;font-weight:normal;font-stretch:normal;font-size/;"	i
tspan146599-2-1-0	figures/pseudo-derivative.svg	/^   style="font-style:normal;font-variant:normal;font-weight:normal;font-stretch:normal;font-size/;"	i
tspan146599-2-1-8	figures/pseudo-derivative.svg	/^   style="font-style:normal;font-variant:normal;font-weight:normal;font-stretch:normal;font-size/;"	i
tspan146599-2-1-8-4	figures/pseudo-derivative.svg	/^   style="font-style:normal;font-variant:normal;font-weight:normal;font-stretch:normal;font-size/;"	i
tspan146599-2-1-8-7	figures/pseudo-derivative.svg	/^   style="font-style:normal;font-variant:normal;font-weight:normal;font-stretch:normal;font-size/;"	i
tspan146599-2-1-8-7-9	figures/pseudo-derivative.svg	/^   style="font-style:normal;font-variant:normal;font-weight:normal;font-stretch:normal;font-size/;"	i
tspan146599-2-2	figures/pseudo-derivative.svg	/^   style="font-style:normal;font-variant:normal;font-weight:normal;font-stretch:normal;font-size/;"	i
tspan146599-5-6	figures/pseudo-derivative.svg	/^   style="font-style:normal;font-variant:normal;font-weight:normal;font-stretch:normal;font-size/;"	i
tspan146599-5-6-6	figures/pseudo-derivative.svg	/^   style="font-style:normal;font-variant:normal;font-weight:normal;font-stretch:normal;font-size/;"	i
tspan146599-5-6-6-7	figures/pseudo-derivative.svg	/^   style="font-style:normal;font-variant:normal;font-weight:normal;font-stretch:normal;font-size/;"	i
tspan146599-5-6-6-9	figures/pseudo-derivative.svg	/^   style="font-style:normal;font-variant:normal;font-weight:normal;font-stretch:normal;font-size/;"	i
tspan146599-5-6-6-9-3	figures/pseudo-derivative.svg	/^   style="font-style:normal;font-variant:normal;font-weight:normal;font-stretch:normal;font-size/;"	i
tspan146599-5-6-6-9-4	figures/pseudo-derivative.svg	/^   style="font-style:normal;font-variant:normal;font-weight:normal;font-stretch:normal;font-size/;"	i
tspan146599-5-6-6-9-4-2	figures/pseudo-derivative.svg	/^   style="font-style:normal;font-variant:normal;font-weight:normal;font-stretch:normal;font-size/;"	i
tspan146599-5-6-7	figures/pseudo-derivative.svg	/^   style="font-style:normal;font-variant:normal;font-weight:normal;font-stretch:normal;font-size/;"	i
tspan15046	figures/pseudo-derivative.svg	/^   id="tspan15046">c<\/tspan>)<\/tspan><\/text>$/;"	i
tspan15046-7	figures/pseudo-derivative.svg	/^   id="tspan15046-7">c<\/tspan>)<\/tspan><\/text>$/;"	i
tspan1514	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">d<tspan$/;"	i
tspan1514-2	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">d<tspan$/;"	i
tspan1518	figures/pseudo-derivative.svg	/^         id="tspan1518">d<tspan$/;"	i
tspan1518-4	figures/pseudo-derivative.svg	/^         id="tspan1518-4"><tspan$/;"	i
tspan1518-4-7	figures/pseudo-derivative.svg	/^         id="tspan1518-4-7"><tspan$/;"	i
tspan1518-6	figures/pseudo-derivative.svg	/^         id="tspan1518-6">d<tspan$/;"	i
tspan1527	figures/pseudo-derivative.svg	/^         style="stroke-width:0.26458332" \/><\/text>$/;"	i
tspan164184	figures/pseudo-derivative.svg	/^         style="font-style:normal;font-variant:normal;font-weight:bold;font-stretch:normal;font-/;"	i
tspan164184-3	figures/pseudo-derivative.svg	/^         style="font-style:normal;font-variant:normal;font-weight:bold;font-stretch:normal;font-/;"	i
tspan164184-3-5	figures/pseudo-derivative.svg	/^         style="font-style:normal;font-variant:normal;font-weight:bold;font-stretch:normal;font-/;"	i
tspan164184-4	figures/pseudo-derivative.svg	/^         style="font-style:normal;font-variant:normal;font-weight:bold;font-stretch:normal;font-/;"	i
tspan165556	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">time<\/tspan><\/text>$/;"	i
tspan165556-9	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">time<\/tspan><\/text>$/;"	i
tspan1657	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">0<\/tspan><\/text>$/;"	i
tspan1657-4	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">0<\/tspan><\/text>$/;"	i
tspan1657-6	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">0<\/tspan><\/text>$/;"	i
tspan1657-6-0	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">0<\/tspan><\/text>$/;"	i
tspan1657-6-2	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">1<\/tspan><\/text>$/;"	i
tspan1657-6-2-3	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">2<\/tspan><\/text>$/;"	i
tspan1657-6-2-3-1	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">2<\/tspan><\/text>$/;"	i
tspan1657-6-2-3-5	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">3<\/tspan><\/text>$/;"	i
tspan1657-6-2-3-5-1	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">3<\/tspan><\/text>$/;"	i
tspan1657-6-2-5	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">1<\/tspan><\/text>$/;"	i
tspan1657-6-5	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">0<\/tspan><\/text>$/;"	i
tspan1657-6-5-4	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">1<\/tspan><\/text>$/;"	i
tspan1657-6-5-4-3	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">2<\/tspan><\/text>$/;"	i
tspan1657-6-5-4-3-1	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">2<\/tspan><\/text>$/;"	i
tspan1657-6-5-4-3-3	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">3<\/tspan><\/text>$/;"	i
tspan1657-6-5-4-3-3-8	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">3<\/tspan><\/text>$/;"	i
tspan1657-6-5-4-8	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">1<\/tspan><\/text>$/;"	i
tspan1657-6-5-6	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">0<\/tspan><\/text>$/;"	i
tspan1657-6-5-6-1	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">1<\/tspan><\/text>$/;"	i
tspan1657-6-5-6-1-6	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">2<\/tspan><\/text>$/;"	i
tspan1657-6-5-6-1-6-1	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">3<\/tspan><\/text>$/;"	i
tspan1657-6-5-6-1-6-1-1	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">3<\/tspan><\/text>$/;"	i
tspan1657-6-5-6-1-6-5	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">2<\/tspan><\/text>$/;"	i
tspan1657-6-5-6-1-7	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">1<\/tspan><\/text>$/;"	i
tspan1657-6-5-6-7	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">0<\/tspan><\/text>$/;"	i
tspan1657-6-5-60	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">0<\/tspan><\/text>$/;"	i
tspan1657-8	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">1<\/tspan><\/text>$/;"	i
tspan1657-8-1	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">2<\/tspan><\/text>$/;"	i
tspan1657-8-1-4	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">3<\/tspan><\/text>$/;"	i
tspan1657-8-1-4-1	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">3<\/tspan><\/text>$/;"	i
tspan1657-8-1-9	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">2<\/tspan><\/text>$/;"	i
tspan1657-8-6	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">1<\/tspan><\/text>$/;"	i
tspan1661	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-1	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-1-2	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-1-6	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-1-6-6	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-1-6-6-1	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-1-6-6-4	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-1-6-6-4-4	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-1-6-6-4-7	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-1-6-6-4-7-4	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-1-6-6-4-7-4-4	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-1-6-6-4-7-4-5	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-1-6-6-4-7-4-5-8	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-1-6-6-4-7-8	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-1-6-6-7	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-1-6-6-7-5	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-1-6-6-7-5-0	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-1-6-6-7-5-0-6	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-1-6-6-7-5-6	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-1-6-6-7-7	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-1-6-61	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-1-6-61-3	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-1-6-61-6	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-1-6-61-6-2	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-1-6-61-6-2-4	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-1-6-61-6-8	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-1-6-8	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-1-7	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-1-7-4	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-1-7-4-0	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-1-7-4-0-7	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-1-7-4-6	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-1-7-9	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-17	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-17-0	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-17-0-2	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-17-0-2-4	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-17-0-24	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-17-6	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-2	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-2-1	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-2-1-1	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-2-1-1-3	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-2-1-1-9	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-2-1-1-9-7	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-2-1-8	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-2-4	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-2-4-0	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-2-4-3	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-2-4-3-2	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-2-4-3-5	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-2-4-3-5-0	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-2-4-3-5-0-6	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-2-4-3-5-0-6-6	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-2-4-3-5-0-8	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-2-4-3-5-9	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-2-4-9	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-2-4-9-8	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-2-4-9-8-0	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-2-4-9-8-0-1	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-2-4-9-8-8	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-2-4-9-9	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-2-46	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan1661-5	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">&lt;<\/tspan><\/text>$/;"	i
tspan17260	figures/pseudo-derivative.svg	/^   id="tspan17260">c<\/tspan><\/tspan><\/text>$/;"	i
tspan17260-6	figures/pseudo-derivative.svg	/^   id="tspan17260-6">c<\/tspan><\/tspan><\/text>$/;"	i
tspan191993	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">unit i<\/tspan><\/text>$/;"	i
tspan191993-2	figures/pseudo-derivative.svg	/^         style="stroke-width:0.264583">unit j<\/tspan><\/text>$/;"	i
tspan25939	figures/pseudo-derivative.svg	/^         y="72.954216">A<\/tspan><\/text>$/;"	i
tspan25939-6	figures/pseudo-derivative.svg	/^         y="72.954216">B<\/tspan><\/text>$/;"	i
tspan8958	figures/pseudo-derivative.svg	/^   id="tspan8958">H<\/tspan>(<tspan$/;"	i
tspan8958-8	figures/pseudo-derivative.svg	/^   id="tspan8958-8">H<\/tspan>(<tspan$/;"	i
vaswani2017attention	references.bib	/^@article{vaswani2017attention,$/;"	a
wandb	references.bib	/^@misc{wandb,$/;"	n
whittlestone2019ethical	references.bib	/^@article{whittlestone2019ethical,$/;"	a
williams_Learning_1989	references.bib	/^@article{williams_Learning_1989,$/;"	a
wunderlich_Eventbased_2021	references.bib	/^@article{wunderlich_Eventbased_2021,$/;"	a
xlink	figures/combined-sparsity-plots.svg	/^	 viewBox="0 0 928 657" style="enable-background:new 0 0 928 657;" xml:space="preserve">$/;"	n	uri:http://www.w3.org/1999/xlink
xtick_10	figures/combined-sparsity-plots.svg	/^		<g id="xtick_10">$/;"	i
xtick_10_00000112607381513015924200000016625273075885906860_	figures/combined-sparsity-plots.svg	/^		<g id="xtick_10_00000112607381513015924200000016625273075885906860_">$/;"	i
xtick_11	figures/combined-sparsity-plots.svg	/^		<g id="xtick_11">$/;"	i
xtick_11_00000001638188400179335760000012488174280967667085_	figures/combined-sparsity-plots.svg	/^		<g id="xtick_11_00000001638188400179335760000012488174280967667085_">$/;"	i
xtick_12	figures/combined-sparsity-plots.svg	/^		<g id="xtick_12">$/;"	i
xtick_12_00000164508672172072919660000010389887049171759505_	figures/combined-sparsity-plots.svg	/^		<g id="xtick_12_00000164508672172072919660000010389887049171759505_">$/;"	i
xtick_13	figures/combined-sparsity-plots.svg	/^		<g id="xtick_13">$/;"	i
xtick_13_00000008149019143772297260000015427895114929264039_	figures/combined-sparsity-plots.svg	/^		<g id="xtick_13_00000008149019143772297260000015427895114929264039_">$/;"	i
xtick_14	figures/combined-sparsity-plots.svg	/^		<g id="xtick_14">$/;"	i
xtick_14_00000068662282232751212540000003120545066452351380_	figures/combined-sparsity-plots.svg	/^		<g id="xtick_14_00000068662282232751212540000003120545066452351380_">$/;"	i
xtick_15	figures/combined-sparsity-plots.svg	/^		<g id="xtick_15">$/;"	i
xtick_15_00000127015079237389561970000017845044381709150360_	figures/combined-sparsity-plots.svg	/^		<g id="xtick_15_00000127015079237389561970000017845044381709150360_">$/;"	i
xtick_16_00000173136248783722550650000006578262842468763283_	figures/combined-sparsity-plots.svg	/^	<g id="xtick_16_00000173136248783722550650000006578262842468763283_">$/;"	i
xtick_16_00000174601081005644518280000018182228020997921470_	figures/combined-sparsity-plots.svg	/^		<g id="xtick_16_00000174601081005644518280000018182228020997921470_">$/;"	i
xtick_17_00000065057984818596949060000004532359424642153902_	figures/combined-sparsity-plots.svg	/^		<g id="xtick_17_00000065057984818596949060000004532359424642153902_">$/;"	i
xtick_17_00000117643447945388393630000015476401681405607068_	figures/combined-sparsity-plots.svg	/^	<g id="xtick_17_00000117643447945388393630000015476401681405607068_">$/;"	i
xtick_18_00000001638255462024832810000015483257157413598857_	figures/combined-sparsity-plots.svg	/^	<g id="xtick_18_00000001638255462024832810000015483257157413598857_">$/;"	i
xtick_18_00000100340219822686179260000001958699281737525676_	figures/combined-sparsity-plots.svg	/^		<g id="xtick_18_00000100340219822686179260000001958699281737525676_">$/;"	i
xtick_19_00000003819224002289059750000017457189188243229583_	figures/combined-sparsity-plots.svg	/^		<g id="xtick_19_00000003819224002289059750000017457189188243229583_">$/;"	i
xtick_19_00000170980330403207116320000008862084579467804549_	figures/combined-sparsity-plots.svg	/^	<g id="xtick_19_00000170980330403207116320000008862084579467804549_">$/;"	i
xtick_1_00000165955813006903263570000002515869651008763540_	figures/combined-sparsity-plots.svg	/^		<g id="xtick_1_00000165955813006903263570000002515869651008763540_">$/;"	i
xtick_1_00000175324084781621234990000009532149734338875550_	figures/combined-sparsity-plots.svg	/^		<g id="xtick_1_00000175324084781621234990000009532149734338875550_">$/;"	i
xtick_20_00000005234882233710409860000016238183083451064766_	figures/combined-sparsity-plots.svg	/^	<g id="xtick_20_00000005234882233710409860000016238183083451064766_">$/;"	i
xtick_20_00000005266061986211219900000007290943084209019836_	figures/combined-sparsity-plots.svg	/^		<g id="xtick_20_00000005266061986211219900000007290943084209019836_">$/;"	i
xtick_21_00000036212385179323801300000012173476084102470075_	figures/combined-sparsity-plots.svg	/^	<g id="xtick_21_00000036212385179323801300000012173476084102470075_">$/;"	i
xtick_21_00000129172745773531377480000010393185124597837988_	figures/combined-sparsity-plots.svg	/^		<g id="xtick_21_00000129172745773531377480000010393185124597837988_">$/;"	i
xtick_22_00000054265682545319634130000008181939882789305738_	figures/combined-sparsity-plots.svg	/^	<g id="xtick_22_00000054265682545319634130000008181939882789305738_">$/;"	i
xtick_22_00000066480515257990590050000008428120853326288558_	figures/combined-sparsity-plots.svg	/^		<g id="xtick_22_00000066480515257990590050000008428120853326288558_">$/;"	i
xtick_23_00000089552620002672105040000003818287083298668464_	figures/combined-sparsity-plots.svg	/^		<g id="xtick_23_00000089552620002672105040000003818287083298668464_">$/;"	i
xtick_23_00000128447164313318958440000012362271432307132055_	figures/combined-sparsity-plots.svg	/^	<g id="xtick_23_00000128447164313318958440000012362271432307132055_">$/;"	i
xtick_24_00000075120857246795403940000016997530660746425001_	figures/combined-sparsity-plots.svg	/^		<g id="xtick_24_00000075120857246795403940000016997530660746425001_">$/;"	i
xtick_25_00000150095700916395943580000004536858055336038794_	figures/combined-sparsity-plots.svg	/^		<g id="xtick_25_00000150095700916395943580000004536858055336038794_">$/;"	i
xtick_26_00000121257922822453060800000008671528364323006626_	figures/combined-sparsity-plots.svg	/^		<g id="xtick_26_00000121257922822453060800000008671528364323006626_">$/;"	i
xtick_27_00000134947145689242845200000014811967379307058577_	figures/combined-sparsity-plots.svg	/^		<g id="xtick_27_00000134947145689242845200000014811967379307058577_">$/;"	i
xtick_28_00000137112433047558938930000014654578589642369669_	figures/combined-sparsity-plots.svg	/^		<g id="xtick_28_00000137112433047558938930000014654578589642369669_">$/;"	i
xtick_29_00000093176567392711574790000011842851478599350185_	figures/combined-sparsity-plots.svg	/^		<g id="xtick_29_00000093176567392711574790000011842851478599350185_">$/;"	i
xtick_2_00000081630784594171572330000013667767465793825962_	figures/combined-sparsity-plots.svg	/^		<g id="xtick_2_00000081630784594171572330000013667767465793825962_">$/;"	i
xtick_2_00000127752688352877692370000015351089781021949111_	figures/combined-sparsity-plots.svg	/^		<g id="xtick_2_00000127752688352877692370000015351089781021949111_">$/;"	i
xtick_30_00000057106215769965276940000011292792480535357096_	figures/combined-sparsity-plots.svg	/^		<g id="xtick_30_00000057106215769965276940000011292792480535357096_">$/;"	i
xtick_31_00000066475402149329144380000003321719560107431847_	figures/combined-sparsity-plots.svg	/^		<g id="xtick_31_00000066475402149329144380000003321719560107431847_">$/;"	i
xtick_3_00000042704830540653314250000017109593431482574752_	figures/combined-sparsity-plots.svg	/^		<g id="xtick_3_00000042704830540653314250000017109593431482574752_">$/;"	i
xtick_3_00000178922996452552161940000000060671518573061025_	figures/combined-sparsity-plots.svg	/^		<g id="xtick_3_00000178922996452552161940000000060671518573061025_">$/;"	i
xtick_4_00000024704198957054626930000003076379489862033823_	figures/combined-sparsity-plots.svg	/^		<g id="xtick_4_00000024704198957054626930000003076379489862033823_">$/;"	i
xtick_4_00000029022095025222832810000016716706648002868138_	figures/combined-sparsity-plots.svg	/^		<g id="xtick_4_00000029022095025222832810000016716706648002868138_">$/;"	i
xtick_5_00000031909512317834601820000004980640803968874170_	figures/combined-sparsity-plots.svg	/^		<g id="xtick_5_00000031909512317834601820000004980640803968874170_">$/;"	i
xtick_5_00000139999270612554289280000014752610119640208297_	figures/combined-sparsity-plots.svg	/^		<g id="xtick_5_00000139999270612554289280000014752610119640208297_">$/;"	i
xtick_6_00000163049612003642359650000011112919028868083109_	figures/combined-sparsity-plots.svg	/^		<g id="xtick_6_00000163049612003642359650000011112919028868083109_">$/;"	i
xtick_6_00000178172965790109778170000012423822514764612794_	figures/combined-sparsity-plots.svg	/^		<g id="xtick_6_00000178172965790109778170000012423822514764612794_">$/;"	i
xtick_7_00000039116877873852480250000009854783842541477051_	figures/combined-sparsity-plots.svg	/^		<g id="xtick_7_00000039116877873852480250000009854783842541477051_">$/;"	i
xtick_7_00000060723790412188280760000007973874288914467771_	figures/combined-sparsity-plots.svg	/^		<g id="xtick_7_00000060723790412188280760000007973874288914467771_">$/;"	i
xtick_8_00000080170307460808959210000001396073886192879523_	figures/combined-sparsity-plots.svg	/^		<g id="xtick_8_00000080170307460808959210000001396073886192879523_">$/;"	i
xtick_8_00000137852928697147844540000008466733686668050842_	figures/combined-sparsity-plots.svg	/^		<g id="xtick_8_00000137852928697147844540000008466733686668050842_">$/;"	i
xtick_9	figures/combined-sparsity-plots.svg	/^		<g id="xtick_9">$/;"	i
xtick_9_00000154388425697989148270000011268937070366124705_	figures/combined-sparsity-plots.svg	/^		<g id="xtick_9_00000154388425697989148270000011268937070366124705_">$/;"	i
xu_Show_2015	references.bib	/^@inproceedings{xu_Show_2015,$/;"	j
yan2022distributed	references.bib	/^@article{yan2022distributed,$/;"	a
yang2014proof	references.bib	/^@inproceedings{yang2014proof,$/;"	j
yang2018breaking	references.bib	/^@inproceedings{$/;"	j
ytick_10_00000154385007864786002050000011304060705745732773_	figures/combined-sparsity-plots.svg	/^		<g id="ytick_10_00000154385007864786002050000011304060705745732773_">$/;"	i
ytick_11_00000100372743687989403770000009504176885624770711_	figures/combined-sparsity-plots.svg	/^		<g id="ytick_11_00000100372743687989403770000009504176885624770711_">$/;"	i
ytick_12_00000034770932173049495370000011697908285590682785_	figures/combined-sparsity-plots.svg	/^		<g id="ytick_12_00000034770932173049495370000011697908285590682785_">$/;"	i
ytick_13_00000135680978119887750770000009320571038522258843_	figures/combined-sparsity-plots.svg	/^		<g id="ytick_13_00000135680978119887750770000009320571038522258843_">$/;"	i
ytick_14_00000116199325115948586930000009559891510517415085_	figures/combined-sparsity-plots.svg	/^		<g id="ytick_14_00000116199325115948586930000009559891510517415085_">$/;"	i
ytick_15_00000023258973957027206940000005318582919992356276_	figures/combined-sparsity-plots.svg	/^		<g id="ytick_15_00000023258973957027206940000005318582919992356276_">$/;"	i
ytick_16_00000019658412053294652240000007993441035387813802_	figures/combined-sparsity-plots.svg	/^		<g id="ytick_16_00000019658412053294652240000007993441035387813802_">$/;"	i
ytick_17_00000039840461728629059020000005069417320528560533_	figures/combined-sparsity-plots.svg	/^		<g id="ytick_17_00000039840461728629059020000005069417320528560533_">$/;"	i
ytick_18_00000024697683179216231130000000190938858803369118_	figures/combined-sparsity-plots.svg	/^		<g id="ytick_18_00000024697683179216231130000000190938858803369118_">$/;"	i
ytick_19_00000042718210548030407470000012100530959842585986_	figures/combined-sparsity-plots.svg	/^		<g id="ytick_19_00000042718210548030407470000012100530959842585986_">$/;"	i
ytick_1_00000082346874156855856600000009938573668925529519_	figures/combined-sparsity-plots.svg	/^		<g id="ytick_1_00000082346874156855856600000009938573668925529519_">$/;"	i
ytick_1_00000122695174667746243150000008977853002055578270_	figures/combined-sparsity-plots.svg	/^		<g id="ytick_1_00000122695174667746243150000008977853002055578270_">$/;"	i
ytick_20_00000121987337064667647270000017725763402620617643_	figures/combined-sparsity-plots.svg	/^		<g id="ytick_20_00000121987337064667647270000017725763402620617643_">$/;"	i
ytick_2_00000078007394527819089880000012647463734617034168_	figures/combined-sparsity-plots.svg	/^		<g id="ytick_2_00000078007394527819089880000012647463734617034168_">$/;"	i
ytick_2_00000150077197381473495100000011359301485229481114_	figures/combined-sparsity-plots.svg	/^		<g id="ytick_2_00000150077197381473495100000011359301485229481114_">$/;"	i
ytick_3_00000096042810914542452620000014105641028361335703_	figures/combined-sparsity-plots.svg	/^		<g id="ytick_3_00000096042810914542452620000014105641028361335703_">$/;"	i
ytick_3_00000168099591248981377020000007511642254076469890_	figures/combined-sparsity-plots.svg	/^		<g id="ytick_3_00000168099591248981377020000007511642254076469890_">$/;"	i
ytick_4_00000068647024613667299730000014625677110723166394_	figures/combined-sparsity-plots.svg	/^		<g id="ytick_4_00000068647024613667299730000014625677110723166394_">$/;"	i
ytick_4_00000179627327337110106800000005675694854664208265_	figures/combined-sparsity-plots.svg	/^		<g id="ytick_4_00000179627327337110106800000005675694854664208265_">$/;"	i
ytick_5	figures/combined-sparsity-plots.svg	/^		<g id="ytick_5">$/;"	i
ytick_5_00000166642226413415866480000001512473184791681717_	figures/combined-sparsity-plots.svg	/^		<g id="ytick_5_00000166642226413415866480000001512473184791681717_">$/;"	i
ytick_6	figures/combined-sparsity-plots.svg	/^		<g id="ytick_6">$/;"	i
ytick_6_00000122710138539113842500000000641848803940616324_	figures/combined-sparsity-plots.svg	/^		<g id="ytick_6_00000122710138539113842500000000641848803940616324_">$/;"	i
ytick_7	figures/combined-sparsity-plots.svg	/^		<g id="ytick_7">$/;"	i
ytick_7_00000127020930661129915410000008858777881387892411_	figures/combined-sparsity-plots.svg	/^		<g id="ytick_7_00000127020930661129915410000008858777881387892411_">$/;"	i
ytick_8	figures/combined-sparsity-plots.svg	/^		<g id="ytick_8">$/;"	i
ytick_8_00000038383337807207256420000016005727609430291622_	figures/combined-sparsity-plots.svg	/^		<g id="ytick_8_00000038383337807207256420000016005727609430291622_">$/;"	i
ytick_9_00000088135139410960457910000001855916187242721698_	figures/combined-sparsity-plots.svg	/^		<g id="ytick_9_00000088135139410960457910000001855916187242721698_">$/;"	i
zenke_SuperSpike_2018	references.bib	/^@article{zenke_SuperSpike_2018,$/;"	a
zoneout2016	references.bib	/^@misc{zoneout2016,$/;"	n

